Bayesian Emulation of Grey-Box Multi-Model Ensembles Exploiting Known Interior Structure

Computer models are widely used to study complex real world physical systems. However, there are major limitations to their direct use including: their complex structure; large numbers of inputs and outputs; and long evaluation times. Bayesian emulators are an effective means of addressing these challenges providing fast and efficient statistical approximation for computer model outputs. It is commonly assumed that computer models behave like a ``black-box'' function with no knowledge of the output prior to its evaluation. This ensures that emulators are generalisable but potentially limits their accuracy compared with exploiting such knowledge of constrained or structured output behaviour. We assume a ``grey-box'' computer model and develop a methodological toolkit for its analysis. This includes: multi-model ensemble subsampling to identifying a representative model subset to reduce computational expense; constructing a targeted Bayesian design for optimisation or decision support; a ``divide-and-conquer'' approach to emulating sums of outputs; structured emulators exploiting known constrained and structured behaviour of constituent outputs through splitting the parameter space and imposing truncations; emulation of sums of time series outputs; and emulation of multi-model ensemble outputs. Combining these methods establishes a hierarchical emulation framework which achieves greater physical interpretability and more accurate emulator predictions. This research is motivated by and applied to the commercially important TNO OLYMPUS Well Control Optimisation Challenge from the petroleum industry which we re-express as a decision support under uncertainty problem. We thus encourage users to examine their ``black-box'' simulators to achieve superior emulator accuracy.

==> Abstract/Abstract-V1.tex <==
\abstract{
	Computer models are widely used to study complex real world physical systems. However, there are major limitations to their direct use including: their complex structure; large numbers of inputs and outputs; and long evaluation times. Bayesian emulators are an effective means of addressing these challenges providing fast and efficient statistical approximation for computer model outputs. It is commonly assumed that computer models behave like a ``black-box'' function with no knowledge of the output prior to its evaluation. This ensures that emulators are generalisable but potentially limits their accuracy compared with exploiting such knowledge of constrained or structured output behaviour. We assume a ``grey-box'' computer model and establish a hierarchical emulation framework encompassing structured emulators which exploit known constrained and structured behaviour of constituent computer model outputs. This achieves greater physical interpretability and more accurate emulator predictions. This research is motivated by and applied to the commercially important TNO OLYMPUS Well Control Optimisation Challenge from the petroleum industry. We re-express this as a decision support under uncertainty problem. First, we reduce the computational expense of the analysis by identifying a representative subset of models using an efficient multi-model ensemble subsampling technique. Next we apply our hierarchical emulation methodology to the expected Net Present Value utility function with well control decision parameters as inputs.
	%The hierarchical emulation framework is adaptable to handle other known constrained or structured forms of computer model outputs, and we encourage users to examine their ``black-box'' simulators to achieve superior emulator accuracy.
	\\
	\textbf{Keywords:} Computer models; Bayesian emulation; Bayes linear; Known simulator behaviour; Multi-model ensembles; Decision support under uncertainty.
}

%Target maximum word count: 250.

==> Appendices/Extended-Results-Targeted-Bayesian-Design-Methodology.tex <==
\subsection{Targeted Bayesian Design Methodology} \label{subsec:Extended-Results-Targeted-Bayesian-Design-Methodology}

We employ a targeted Bayesian design algorithm in \cref{subsec:Bayesian-Design.tex} to efficiently sample from the decision parameter space by incorporating prior reservoir engineering knowledge. This entails imposing: operational range constraints on the decision parameter control rates (as is standard within the computer modelling literature); and a difference constraint on time consecutive controls to avoid unphysical large temporal variation which is poor engineering practice. Consequently, the decision parameters are not mutually independent. After splitting the decision parameters into independent subgroups by well, $\boldd_{jk} \in \Djk$, the difference constraint stipulates that $\lvert \djkti - \djktiminusone \rvert \leq \Delta_i, \ i = 2, \ldots, \Djk$, where $\Djk$ is the number of control intervals for well $jk$. The decision parameter space is no longer a hypercube, thus motivating the need for a Bayesian design informed by this prior information.

Our targeted Bayesian design algorithm involves a re-parameterisation and sampling the sum of the parameters and their time consecutive differences. First assume each $\djkti \in [0, 1]$. Define $t = \sum_{i = 1}^{\Djk} \djkti \in [0, \Djk]$ to be the sum of the parameters and $\pardiffi = \frac{\djkti - \djktiminusone}{\sqrt{2}}$ for $i = 2, \dots, \Djk$, to be the scaled differences where the scaling by $\frac{1}{\sqrt{2}}$ is required due to the rotation of the parameter space in this alternative parametrisation. The new parameters are mutually orthogonal with $t \in [0, \Djk]$ and $\lvert \pardiffi \rvert \leq \Delta_i^\prime = \frac{\Delta_i}{\sqrt{2}}$. This re-parametrisation is the represented by linear transformation $(t, \pardiffvec)^\Transpose = L \boldd_{jk} $ in \cref{eq:Sampling-Parameter-Sum-Differences-Matrix-Equation} where $L$ is the transformation matrix. Sampling in the re-parametrised space automatically satisfies the difference constraints with a sample for $\boldd_{jk}$ obtained via $\boldd_{jk} = L^{-1} (t, \pardiffvec)^\Transpose$. The range constraints, $\djkti \in [0, 1]$, must also then be verified.
\begin{align} \label{eq:Sampling-Parameter-Sum-Differences-Matrix-Equation}
	\begin{pmatrix}
		t \\
		\pardiff_2 \\
		\pardiff_3 \\
		\pardiff_4 \\
		\vdots \\
		\pardiff_{\Djk}
	\end{pmatrix}
	=
	\begin{pmatrix}
		1 & 1 & 1 & 1 & \cdots & 1 & 1\\
		\sfrac{-1}{\sqrt{2}} & \sfrac{1}{\sqrt{2}} & 0 & 0 & \cdots & 0 & 0\\
		0 & \sfrac{-1}{\sqrt{2}} & \sfrac{1}{\sqrt{2}} & 0 & \cdots & 0 & 0\\
		0 & 0 & \sfrac{-1}{\sqrt{2}} & \sfrac{1}{\sqrt{2}} & \cdots & 0 & 0\\
		\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
		0 & 0 & 0 & 0 & \cdots & \sfrac{-1}{\sqrt{2}} & \sfrac{1}{\sqrt{2}}
	\end{pmatrix}
	\begin{pmatrix}
		d_{jk, 1} \\
		d_{jk, 2} \\
		d_{jk, 3} \\
		d_{jk, 4} \\
		\vdots \\
		d_{jk, \Djk}
	\end{pmatrix}
\end{align}
%
In order to ensure good exploration along the $t$-direction, thought to be important by reservoir engineers, we propose preserving an initial sample of the parameter sums, and then uniformly resample $\pardiffvec$ until both constraint types are satisfied. There is freedom to choose the sampling distribution of $t$ with probability density function, $f_T(t)$, dependent on the analysis. We use a truncated normal distribution with other examples being: uniform; mixture of uniforms; and transformed beta distributions. Orthogonal projection of the samples onto the line $d_{jk, 1} = d_{jk, 2} = \cdots = d_{jk, \Djk}$ will approximately follow the specified distribution. 

The process of generating a sample of size $n$ for an independent subgroup of parameters is described in the rejection style \cref{alg:Sampling-of-Parameter-Sum-and-Differences-preserving-Parameter-Sum-Sampling-Distribution-adjust-Difference-Sampling-Range} yielding matrix $B$ in which each column is a sampled vector of decision parameters. If $t$ is close to 0 or $\Djk$ the rejection step can be computationally time consuming with the efficiency improved by sampling the differences conditional on $t$. This algorithm may be applied separately to each independent subgroup of decision parameters for improved efficiency before combing to obtain a design over the full decision parameter space. Design optimisation may be performed using standard design selection criteria, for example, minimax or maximin design \cite{2003:Santner:The-Design-and-Analysis-of-Computer-Experiments}, both for the designs by subgroup and the full design by combining using random permutations. Further discussion of the targeted Bayesian design method is presented in \cite[Sec.~4.3]{2022:Owen:PhD-Thesis}.

%\begin{algorithm}
%\caption{Build tree}
%\label{alg:buildtree}
%\begin{algorithmic}
%\STATE{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
%\WHILE{$\#P > 1$}
%\STATE{Choose $C^\prime\in\mathcal{C}_p(P)$ with $C^\prime := \operatorname{argmin}_{C\in\mathcal{C}_p(P)} \varrho(C)$}
%\STATE{Find an optimal partition tree $T_{C^\prime}$ }
%\STATE{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
%\STATE{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus} \mathcal{L}(T_{C^\prime})\}$}
%\ENDWHILE
%\RETURN $T$
%\end{algorithmic}
%\end{algorithm}





\begin{algorithm}%[!t]%[!th]
	\caption{Sampling of parameter sums and differences preserving the initial sum of parameters sample.}
	\label{alg:Sampling-of-Parameter-Sum-and-Differences-preserving-Parameter-Sum-Sampling-Distribution-adjust-Difference-Sampling-Range}    % H argument forces algorithm to remain in place.
	\begin{algorithmic}
		\STATE{Let $\mathbf{t}$ be a vector of $n$ samples of $t \sim f_T(t)$}
		\STATE{Let $B$ be an empty matrix of $\Djk$ rows}
		\STATE{Define $dimension(\cdot)$ to be a function to obtain the length of a vector}
		\WHILE{$dimension(\mathbf{t}) > 0$}
			\FORALL{t in $\mathbf{t}$}
				\STATE{Set $\epsilon_i = \min\{t, \Djk - t, \Delta_i^\prime\}$}
				\STATE{Generate $\pardiffi \mid t \sim \mathcal{U}[- \epsilon_i, \epsilon_i]$, for $i = 2, \dots, \Djk$}
			\ENDFOR
			\STATE{Row bind $\mathbf{t}, \pardiffvec_2, \dots, \pardiffvec_{\Djk}$ to form matrix $B_{r, \mathrm{prop}}$}
			\STATE{Compute $B_{\mathrm{prop}} = L^{-1} B_{r, \mathrm{prop}}$}
			\FORALL{Column in $B_{\mathrm{prop}}$}
				\IF{Range \textit{conditions} of parameter vector are satisfied}
					\STATE{Join \textit{Column} to $B$}
					\STATE{Remove corresponding $t$ from $\mathbf{t}$}
				\ELSE
					\STATE{Discard \textit{Column}}
				\ENDIF
			\ENDFOR
		\ENDWHILE
		\RETURN{Matrix $B$ of columns of sampled parameter vectors}
	\end{algorithmic}
\end{algorithm}

%%% Original Version of Algorithm %%%
%\begin{algorithm}[!t]%[!th]
%	\caption{Sampling of parameter sums and differences preserving the initial sum of parameters sample.}
%	\label{alg:Sampling-of-Parameter-Sum-and-Differences-preserving-Parameter-Sum-Sampling-Distribution-adjust-Difference-Sampling-Range}    % H argument forces algorithm to remain in place.
%	\SetAlgoLined    % Prints vertical lines between bloc start-end keywords as begin,end.
%	\KwResult{Matrix $B$ of columns of sampled parameter vectors}    % Result of the algorithm.
%	Let $\mathbf{t}$ be a vector of $n$ samples of $t \sim f_T(t)$\;
%	Let $B$ be an empty matrix of $\Djk$ rows\;
%	Define $dimension(\cdot)$ to be a function to obtain the length of a vector\;
%	\While{$dimension(\mathbf{t}) > 0$}{
%		\ForEach{t in $\mathbf{t}$}{
%			Set $\epsilon_i = \min\{t, \Djk - t, \Delta_i^\prime\}$\;
%			Generate $\pardiffi \mid t \sim \mathcal{U}[- \epsilon_i, \epsilon_i]$, for $i = 2, \dots, \Djk$\;
%		}
%		Row bind $\mathbf{t}, \pardiffvec_2, \dots, \pardiffvec_{\Djk}$ to form matrix $B_{r, \mathrm{prop}}$\;
%		Compute $B_{\mathrm{prop}} = L^{-1} B_{r, \mathrm{prop}}$\;
%		\ForEach{Column in $B_{\mathrm{prop}}$}{
%			\eIf{Range \textit{conditions} of parameter vector are satisfied}{
%				Join \textit{Column} to $B$\;
%				Remove corresponding $t$ from $\mathbf{t}$\;
%			}{
%				Discard \textit{Column}\;
%			}
%		}
%	}
%\end{algorithm}

==> Appendices/Structured-Emulation-with-Two-Sided-Truncation.tex <==
\section{Structured Emulation with Two-Sided Truncation} \label{sec:Structured-Emulation-with-Two-Sided-Truncation}

In this appendix we present an alternative variant of structured emulation exploiting the known simulator behaviour from \cref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents} which uses a two-sided truncation, as presented in \cite[Sec.~3.3.2]{2022:Owen:PhD-Thesis}. It is unnecessary for the application to the \TNOChallengeWC{} in \cref{sec:Results}, but is utilised in another application described in \cite[Sec.~5.4.1 \& 5.8.1]{2022:Owen:PhD-Thesis}. In addition, we detail the truncated normal distribution equations used in both methodologies.

Estimation of the change points and extrapolation cut-offs remains as described in \cref{subsubsec:Structured-Emulation-Change-Points,subsubsec:Structured-Emulation-Extrapolation-Cut-Offs} respectively, as does the physical maximum constraint discussed in \ref{subsubsec:Structured-Emulation-Methodology}. A lower truncation, denoted by $a_i$, may also be imposed, for example, to represent the constraint that the WOPT and WWIT NPV constituents within a control interval must be non-negative ($a_i = 0$). Both constraints are utilised alongside the preliminary Bayes linear emulator in a modified classification step:
\begin{enumerate*}
	\item \textbf{Slope Region:} If $\dcp < \extrapco{jk}{t_i}$ \textbf{or} for the preliminary emulator \lword{$\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} > \dcp \cdot \Delta t_i$}, then collapse the emulator such that for the structured emulator $\E_{\boldFi^\prime}[\fid] = \dcp \cdot \Delta t_i$ with fixed maximum absolute errors of size $\delta_i$.% This corresponds to when the output is strongly believed to be in the slope region.
	
%	\item \textbf{Uncertain Region around Change Point:} As for the upper truncation version above, if for the preliminary emulator $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i < \E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]}$, \textbf{or} if the additional criterion of $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} <  a_i$ \textbf{whilst} $\E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i$, a truncated GP emulator is evaluated. The mean and variance are determined by \cref{eq:Truncated-normal-distribution-mean,eq:Truncated-normal-distribution-variance} respectively and are computed as for the upper truncation version above noting the change in the lower truncation bound $a_i$ and hence $\alpha_i$. This form of emulation is used in the uncertain region around the true location of the change point.
	\item \textbf{Intermediate Region:} As for the upper truncation version, if the preliminary emulator satisfies $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i < \E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]}$, \textbf{or} if the additional criterion of $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} <  a_i$ \textbf{whilst} $\E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i$, a truncated GP emulator is evaluated. The mean and variance are determined by \cref{eq:Truncated-normal-distribution-mean,eq:Truncated-normal-distribution-variance} respectively.% This form of emulation is used in the uncertain region around the true location of the change point.
	
	\item \textbf{Plateau Region:} In all other cases where $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \geq a_i$ \textbf{and} $\E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i$, use the preliminary emulator .% This corresponds to when the output is strongly believed to be in the plateau region.
\end{enumerate*}

The structured emulation methodology utilises a truncated Gaussian process (truncated GP) emulator for which the mean and variance are determined by \cref{eq:Truncated-normal-distribution-mean,eq:Truncated-normal-distribution-variance} respectively \cite{1994:Johnson:Continuous-Univariate-Distributions-Vol-1}, where $\phi(\cdot)$ and $\Phi(\cdot)$ represent the probability density and cumulative distribution functions respectively of a standard normal distribution. These are computed assuming a preliminary Gaussian process emulator with posterior mean and variance, abbreviated to $\mu_i$ and $\sigma_i^2$ respectively, equal to the computed adjusted expectation and variance, and truncation bounds $a_i$ and $b_i = \dcp \cdot \Delta t_i$, with $\alpha_i = \frac{a_i - \mu_i}{\sigma_i}$, and $\beta_i = \frac{b_i - \mu_i}{\sigma_i}$. This form of emulation is used in the intermediate uncertain region around the change point true location.
\begin{align}
	\E_{\boldFi^\prime}[\fid \mid a_i < \fid < b_i] &{} = \mu_i + \sigma \dfrac{\phi(\alpha_i) - \phi(\beta_i)}{\Phi(\beta_i) - \Phi(\alpha_i)} \label{eq:Truncated-normal-distribution-mean} \\
	%
	\Var_{\boldFi^\prime}[\fid \mid a_i < \fid < b_i] &{} = \sigma_i^2 \left[ 1 + \dfrac{\alpha_i \phi(\alpha_i) - \beta_i \phi(\beta_i)}{\Phi(\beta_i) - \Phi(\alpha_i)} - \left( \dfrac{\phi(\alpha_i) - \phi(\beta_i)}{\Phi(\beta_i) - \Phi(\alpha_i)} \right)^2 \right] \label{eq:Truncated-normal-distribution-variance}
\end{align}



%%% Notes %%%
%Add discussion of structured emulation with two-sided truncation. This builds on the methodology in \cref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents} and is an alternative to \cref{subsubsec:Structured-Emulation-Methodology}.
%
%Include the truncated normal distribution equations.

==> Bayesian-Emulation/Bayesian-Emulation-V1.tex <==
\section{Bayesian Emulation} \label{sec:Bayesian-Emulation}

An emulator is a stochastic belief specification for a deterministic or stochastic function that provides a fast and efficient statistical approximation, yielding predictions for as yet unevaluated parameter settings, along with a corresponding statement of the associated uncertainty \cite{2001:Craig:Bayesian-Forecasting-Using-Computer-Simulators,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments}. They are frequently employed for computationally expensive simulators across a range of scientific and industrial applications to perform tasks including: calibration \cite{2001:Kennedy:Bayesian-calibration-of-computer-models,2008:Higdon:Computer-Model-Calibration-Using-High-Dimensional-Output}; history matching \cite{1996:Craig:Bayes-linear-strategies-matching-hydrocarbon-reservoir-history,1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2019:Edwards:Revisiting-Antarctic-ice-loss-due-to-marine-ice-cliff-instability}; uncertainty quantifications \cite{1998:O'Hagan:Uncertainty-Analysis-and-other-Inference-Tools-for-Complex-Computer-Codes}; sensitivity analyses \cite{2004:Oakley-and-O'Hagan:Probabilistic-sensitivity-analysis-of-complex-models-a-Bayesian-approach,2023:Kennedy:Multilevel-emulation-for-stochastic-computer-models-with-application-to-large-offshore-wind-farms}; and decision support \cite{2009:Oakley:Decision-Theoretic-Sensitivity-Analysis-for-Complex-Computer-Models,2012:Williamson:Fast-linked-analyses-for-scenario-based-hierarchies}.

For a computer model $\fd$ the $i$\textsuperscript{th} univariate output is denoted by the function $\fid$, where $\boldd \in \Omega \subset \mathcal{R}^D$ is a vector of (decision) parameters in space $\Omega$. We employ Bayesian emulators of the general form in \cref{eq:Bayes-linear-emulator-structure-in-decision-parameters-univariate-output} \cite{1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2018:Vernon:Bayesian-uncertainty-analysis-systems-biology}.
\begin{align} \label{eq:Bayes-linear-emulator-structure-in-decision-parameters-univariate-output} %\label{eq:Bayes-linear-emulator-structure-in-model-parameters-univariate-output}
	\fid &{} = \boldg_i(\boldd_{A_i})^\Transpose \boldbeta_i + u_i(\boldd_{A_i}) + w_i(\boldd) \nonumber \\
	&{} = \sum_{j = 1}^{p} \beta_{ij}g_{ij}(\boldd_{A_i}) + u_i(\boldd_{A_i}) + w_i(\boldd)
\end{align}
The subscript $A_i$ denotes a subset of active inputs which are the parameters deemed to be most influential for $\fid$, where $| A_i | = \Dprime \leq D$. Within the emulator the first term models the global function behaviour of $\fid$ where the $g_{ij}(\cdot)$ are deterministic functions of the active inputs with unknown scalar regression coefficients, $\beta_{ij}$ for $j = 1, \ldots, p$, where $p \in \mathbb{N}$. Collectively, these are denoted by the vector function $\boldg_i(\cdot) = \begin{psmallmatrix} g_{i1}(\cdot) \\ \vdots \\ g_{ip}(\cdot) \end{psmallmatrix}$, and the vector $\boldbeta_i = \begin{psmallmatrix} \beta_{i1}\\ \vdots \\ \beta_{ip} \end{psmallmatrix} \in \mathbb{R}^p$ respectively. The second term, $u_i(\cdot)$, models the local behaviour of $\fid$ and is a weakly stationary stochastic process with zero mean and a pre-specified covariance structure. A common choice is the squared exponential covariance function in \cref{eq:Squared-exponential-covariance-structure-long} \cite{2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2006:Rasmussen-Williams:Gaussian-Processes}, where $\sigma_{u_i}^2$ is a variance hyperparameter, and $\boldtheta_i = (\theta_{i1}, \ldots, \theta_{iD})$ is a $\Dprime$-vector of (distinct) correlation lengths.
\begin{align}
	\Cov[ u_i(\boldd_{A_i}), u_i(\bolddprime_{A_i}) ] = \sigma_{u_i}^2 \exp\left \{ - \sum_{k = 1}^{\Dprime} \left( \dfrac{d_{A_i, k} - d_{A_i, k}^\prime}{\theta_{ik}} \right)^2 \right \} \label{eq:Squared-exponential-covariance-structure-long}
\end{align}
The third term in \cref{eq:Bayes-linear-emulator-structure-in-decision-parameters-univariate-output}, $w_i(\boldx)$, is an uncorrelated, zero-mean nugget term with covariance:
\begin{align} \label{eq:Emulator-nugget-term-covariance-structure}
	\Cov[ w_i(\boldd), w_i(\bolddprime) ] = \sigma_{w_i}^2 \indicatorequalboldd
\end{align}
This is a white noise process which is included to account for the inactive variables \cite{2010:Cumming:Multiscale-Bayes-Linear-Uncertainty-Analysis-Oil-Reservoirs,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation} and ensure numerical stability \cite{2001:Kennedy:Bayesian-calibration-of-computer-models}. Further arguments for the inclusion of a nugget term are presented in \cite{2012:Andrianakis-and-Challenor:The-effect-of-the-nugget-on-Gaussian-process-emulators-of-computer-models,2012:Gramacy-and-Lee:Cases-for-the-nugget-in-modeling-computer-experiments}. 

We follow a Bayes linear paradigm following the foundations of De Finetti \cite{1974:DeFinetti:Theory-of-Probability,1975:DeFinetti:Theory-of-Probability} using expectation as a primitive within a second-order belief specification. Moreover, we subscribe to subjective Bayesianism to provide a coherent framework to structure and combine expert prior beliefs with observed data to achieve posterior inferences \cite{2006:Goldstein:Subjective-Bayesian-Analysis-Principles-and-Practice}. Bayes linear methods have the numerous advantages including: quick and simple elicitation of subjective prior beliefs; computational tractability; and robust inferences by removing the specification of full prior probability distributions, with Bayes linear emulators having been successfully implemented across numerous applications \cite{1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2018:Vernon:Bayesian-uncertainty-analysis-systems-biology,2006:Goldstein:Bayes-Linear-Calibrated-Prediction-for-Complex-Systems,2022:Vernon:Bayesian-Emulation-and-History-Matching-of-JUNE}. An in-depth discussion of Bayes linear statistics can be found in \cite{2007:Goldstein-and-Wooff:Bayes-Linear-Statistics-Theory-and-Methods}, with shorter summaries presented in \cite{2006:Goldstein:Bayes-Linear-Analysis,2011:Goldstein:External-Bayesian-analysis-for-computer-simulators}. Given a design $\mathcal{D} = \{ \boldd^{(1)}, \ldots, \boldd^{(n)} \}$ and computer model evaluations for output $i$, $\boldFi = \{ f_i(\boldd^{(1)}), \ldots, f_i(\boldd^{(n)}) \}$, the Bayes linear adjusted expectation, variance, and covariance are:
\begin{align}
	\EFifd &{}= \E[\fid] + \Cov[\fid, \boldFi] \Var[\boldFi]^{-1} (\boldFi - \E[\boldFi]) \label{eq:Bayes-linear-emulator-adjusted-expectation} \\
	\VarFifd &{}= \Var[\fid] - \Cov[\fid, \boldFi] \Var[\boldFi]^{-1} \Cov[\boldFi, \fid] \label{eq:Bayes-linear-emulator-adjusted-variance} \\
	\CovFifdfdprime &{}= \Cov[\fid, \fidprime] - \Cov[\fid, \boldFi] \Var[\boldFi]^{-1} \Cov[\boldFi, \fidprime] \label{eq:Bayes-linear-emulator-adjusted-covariance}
\end{align}
Full derivation of the Bayes linear emulator adjustment formulae is presented in \cite[Sec.~2.4.5]{2022:Owen:PhD-Thesis}. An alternative full Bayesian approach is Gaussian Process (GP) emulators, as discussed in \cite{2001:Kennedy:Bayesian-calibration-of-computer-models}. Under the Bayes linear formulation we opt for a hyperparameter plug-in approach where they are specified a priori, utilising expert elicitation, before validating using emulator diagnostic techniques \cite{2009:Bastos:Diagnostics-for-Gaussian-Process-Emulators}, as performed in \cite{1996:Craig:Bayes-linear-strategies-matching-hydrocarbon-reservoir-history,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2018:Vernon:Bayesian-uncertainty-analysis-systems-biology}.



%%% Notes %%%
%Introduce emulators.
%
%Show and describe form of emulator.
%
%Present the squared exponential covariance function, its hyperparameters, and how these may be assessed.
%
%State that we work within a Bayes linear paradigm.
%
%Show the Bayes linear adjusted expectation, variance and covariance formulate.
%
%%% Bayes Linear Paradigm and Subjective Bayesianism Paragraph Notes %%%
%We follow a Bayes linear paradigm working in a second-order belief specification.
%An in-depth discussion of the Bayes linear paradigm can be found in \cite{2007:Goldstein-and-Wooff:Bayes-Linear-Statistics-Theory-and-Methods}, with shorter summaries presented in \cite{2006:Goldstein:Bayes-Linear-Analysis,2011:Goldstein:External-Bayesian-analysis-for-computer-simulators}.
%Bayer linear adjustment formulae for the expectation and variance \cite{1974:DeFinetti:Theory-of-Probability,1975:DeFinetti:Theory-of-Probability}.
%
%% Alternative start to paragraph:
% We follow a Bayes linear paradigm following the foundations of De Finetti \cite{1974:DeFinetti:Theory-of-Probability,1975:DeFinetti:Theory-of-Probability} using expectation as a primitive within a second-order belief specification. Moreover, we subscribe to subjective Bayesianism to provide a coherent framework to structure and combine expert prior beliefs with observed data to achieve posterior inferences \cite{2006:Goldstein:Subjective-Bayesian-Analysis-Principles-and-Practice}. Bayes linear methods follow the foundational work of De Finetti \cite{1974:DeFinetti:Theory-of-Probability,1975:DeFinetti:Theory-of-Probability} with Bayes linear emulators having being successfully implemented across numerous applications \cite{1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2018:Vernon:Bayesian-uncertainty-analysis-systems-biology,2006:Goldstein:Bayes-Linear-Calibrated-Prediction-for-Complex-Systems,2022:Vernon:Bayesian-Emulation-and-History-Matching-of-JUNE}. An in-depth discussion of Bayes linear statistics can be found in \cite{2007:Goldstein-and-Wooff:Bayes-Linear-Statistics-Theory-and-Methods}, with shorter summaries presented in \cite{2006:Goldstein:Bayes-Linear-Analysis,2011:Goldstein:External-Bayesian-analysis-for-computer-simulators}.

==> Conclusion/Conclusion-V1.tex <==
\section{Conclusion} \label{sec:Conclusion}

We have presented a novel hierarchical emulation model in order to exploit known constrained and structured behaviour of simulator outputs for ``grey-box'' computer models in order to achieve more accurate predictions for quantities of interest. This is motivated by and applied to the \TNOChallengeWC{} from the petroleum industry where the aim is to maximise the expected NPV as a function of well control decision parameters. We reconstrue this as a decision support problem where the utility function consists of a discounted sum of oil production, water injection and production, both by well and control interval. The first two simulator outputs exhibit partially known behaviour, constrained by choices of inputs and physical limits with respect to their corresponding target production and injection rate decision parameters respectively, with this structure encompassed within our emulator formulation. Application demonstrates superior accuracy versus Bayes linear emulators, whilst the slower speed of evaluation is mitigated by the need for fewer (waves of) simulations from the expensive computer model. Both factors are important for the overall aim of providing robust decision support under uncertainty. Moreover, we introduce multi-model ensemble subsampling techniques to efficiently identify a representative subset of models which collectively best characterises the expected NPV (or other output(s) of interest), whilst also providing a method for their prediction. This constitutes a novel application to the petroleum industry where multi-model ensembles are commonly used to represent geological uncertainty, greatly reducing the computational cost of our decision analysis.
%%% Alternative final sentence %%%
%This constitutes a novel application to the petroleum industry to address the common issue of geological uncertainty which is commonly represented by a multi-model ensemble and greatly reduces the computational cost of our analysis.

The next step is to employ the presented hierarchical emulation methodology within iterative decision support, applied to the \TNOChallengeWC{}, which incorporates a comprehensive and realistic uncertainty quantification to statistically link inferences for the computer model (OLYMPUS) with the corresponding real world physical system. See \cite[Sec.~4.6 \& 4.7]{2022:Owen:PhD-Thesis} for details. In addition, further methodological development should focus on improving the hierarchical emulation framework. This may be achieved by revising the structured emulators change point estimation methods, classification and truncation, as well as via the refinement of the hierarchy uncertainty propagation. Another direction is multivariate structured emulation of the NPV constituents to assess their correlation and thus more accurately quantify the approximate NPV by ensemble member emulator variance in \cref{subsec:Emulation-of-the-Approximate-NPV}. Such further methodological developments must also be efficient so as not add to the computational burden.

The hierarchical emulation framework presented in this paper, whilst motivated by and tailored to the petroleum well control optimisation problem, is sufficiently flexible and adaptable to handle other (partially) known forms of computer model outputs and functions thereof. Opening ``black-box'' simulators and exploring functions of their output to investigate their behaviours is evidently beneficial, as is using domain expert prior knowledge and small carefully designed collections of simulations. Another example of emulating ``grey-box'' models is in known boundary emulation \cite{2019:Vernon:Known-Boundary-Emulation-of-Complex-Computer-Models,2023:Jackson:Efficient-Emulation-of-Computer-Models-Utilising-Multiple-Known-Boundaries-of-Differing-Dimensions}. The additional prior information can then be used guide the choice from existing emulation methods or to design novel forms which exploit known behavioural facets in order to achieve superior accuracy and enhance the usefulness of emulators for real world applications.
%The emulation framework presented here, whilst motivated by and tailored to the petroleum well control optimisation problem, should inspire other practitioners to open up ``black-box'' simulators, and functions of their output, to investigate their structures. The additional prior information can then be used guide the choice from existing emulation methods or in the design of novel forms which exploit known behavioural facets in order to achieve superior accuracy and enhance the usefulness of emulators for real world applications.



%%% Notes %%%
%Add conclusion.
%
%The suite of techniques, whilst tailored towards the well control optimisation challenge from the petroleum industry, is designed to inspire other practitioners to open up ``black-box'' simulators and functions of their output, and design or use emulators which exploit known facets in their behaviour.
%
%\textbf{Ideas for future work:} \\
%Multivariate emulation -- how to meaningfully assess the correlation structure between NPV constituents -- see PhD thesis paragraphs on multivariate emulation in the emulation of the approximate NPV. \\
%Employing the presented methodology within iterative decision support using a realistic statistical uncertainty quantification to link inferences for the computer model (OLYMPUS) with the corresponding real world physical system (if it existed), as discussed in \cite[Sec.~4.6 \& 4.7]{2022:Owen:PhD-Thesis} -- topic of another paper.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulation-of-the-Approximate-NPV.tex <==
\subsection{Emulation of the Approximate NPV} \label{subsec:Emulation-of-the-Approximate-NPV}

An intuitive means of combining emulators for the NPV constituents is via the NPV formula in \cref{eq:NPV-general-formula-in-decision-parameters,eq:Well-control-optimisation-challenge-NPV-R(d_t_i)}. However, control intervals are often formed by amalgamating multiple consecutive discounting intervals, hence the constituent emulators do not correspond exactly to the terms in the NPV formula, labelled as the exact NPV, and denoted by $\NPVjd$ for the $j$\textsuperscript{th} model. A formula for an approximate NPV, denoted $\approxNPVjd$, is presented in \cref{eq:Average-discounting-approximate-NPV_j-formula-for-well-control-optimisation}, where $\lambda_i$ is a weighted average discounting factor for the $i$\textsuperscript{th} interval defined in \cref{eq:Approximate-NPV-Average-discounting-coefficient} for which $k$ indexes the discounting intervals contained within the longer control interval, $N_{t_i}$ is the total number of such discounting intervals, and $t_{i, 0} = t_{i - 1}$.
\begin{align}
	\approxNPVjd &{} = \sum_{i = 1}^{N_t} \lambda_i \left[ Q_{j,op}(\boldd, t_i) \cdot r_{op} - Q_{j,wp}(\boldd, t_i) \cdot r_{wp} - Q_{j,wi}(\boldd, t_i) \cdot r_{wi} \right] \label{eq:Average-discounting-approximate-NPV_j-formula-for-well-control-optimisation} \\
	\lambda_i &{} = \dfrac{1}{t_i - t_{i - 1}}\sum_{k = 1}^{N_{t_i}} \dfrac{t_{i, k} - t_{i, k - 1}}{(1 + d)^{\frac{t_{i, k}}{\tau}}} \label{eq:Approximate-NPV-Average-discounting-coefficient}
\end{align}
Note that using an averaged discount factor yields a more accurate approximation compared with applying the discounting at the end of the control intervals only.

An emulator for $\NPVjd$ is obtained by substituting the simulator for emulators of $Q_{j,op}(\boldd, t_i)$, $Q_{j,wp}(\boldd, t_i)$ and $Q_{j,wi}(\boldd, t_i)$ using \cref{eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-expectation,eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-variance}. Assuming uncorrelated NPV constituents, and using a collection of univariate emulators, \cref{eq:Approximate-NPV_j-emulation-via-NPV-formula-adjusted-expectation,eq:Approximate-NPV_j-emulation-via-NPV-formula-adjusted-variance} are the adjusted expectation and variance formulae respectively. As above, $\mathbf{F}_j$ represents all data used to fit the NPV constituents emulators for the $j$\textsuperscript{th} ensemble member.
\begin{align*}
	\E_{\boldFj}\left[ \approxNPVjd \right] &{} = \sum_{i = 1}^{N_t} \lambda_i \left\{ r_{op} \E_{\boldFj}[ Q_{j,op}(\boldd, t_i)] \right. \alignmultilineeq \phantom{ \sum_{i = 1}^{N_t} \lambda_i \left\{ \right. } \left. - r_{wp} \E_{\boldFj}[Q_{j,wp}(\boldd, t_i)] - r_{wi} \E_{\boldFj}[Q_{j,wi}(\boldd, t_i)] \right\} \alignnumber \label{eq:Approximate-NPV_j-emulation-via-NPV-formula-adjusted-expectation} \\
	\Var_{\boldFj}\left[ \approxNPVjd \right] &{} = \sum_{i = 1}^{N_t} \lambda_i^2 \left\{ r_{op}^2 \Var_{\boldFj}[Q_{j,op}(\boldd, t_i)] \right. \alignmultilineeq \phantom{ \sum_{i = 1}^{N_t} \lambda_i^2 \left\{ \right. } \left. + r_{wp}^2 \Var_{\boldFj}[Q_{j,wp}(\boldd, t_i)] + r_{wi}^2 \Var_{\boldFj}[Q_{j,wi}(\boldd, t_i)] \right\} \alignnumber \label{eq:Approximate-NPV_j-emulation-via-NPV-formula-adjusted-variance}
\end{align*}
For each WOPT and WWIT contributor where structured emulation is applied, for new $\boldd$ identified as either in the plateau region or the uncertain region around the change point, the adjusted expectation and variance are obtained from the preliminary Bayes linear or truncated GP emulator respectively. In the slope region where the emulator is collapsed onto the slope, the expectation is known whilst the adjusted variance is approximated by treating $\delta_i$ as equal to 3 standard deviations. Since the WWPT constituents do not adhere to the structured mode of behaviour, these are emulated using a Bayes linear emulator.

%%% Discussion of Emulating Networks of Simulators %%%
%The NPV constituents are obtained from a single simulator, however the way in which they feed into the NPV calculation suggests that they may also be viewed as from a network of computer simulators. Alternative methodology for emulating simulator output which can be decomposed into a network of component simulators can be seen in \cite{2018:Kyzyurova:Coupling-Computer-Models-through-Linking-Their-Statistical-Emulators,2021:Jackson:Bayes-Linear-Emulation-of-Simulator-Networks}. This is best applied where the link between each of the simulator outputs is less well understood. In this instance there is a natural means of combining the emulators for each of the NPV constituents which is intuitive to understand, simple to construct, and quick to evaluate as a function of the individual contributors emulator output. The methodology for emulating networks of component simulators is therefore not employed.



%%% Notes %%%
%See PhD Thesis Section 3.3.3.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulation-of-the-Ensemble-Mean-NPV.tex <==
\subsection{Emulation of the Ensemble Mean NPV} \label{subsec:Emulation-of-the-Ensemble-Mean-NPV}

The objective is to emulate the ensemble mean NPV by combining emulators for individual models. A reasonable assumption is that the ensemble members are independent given the complexity of their different underlying geologies.



\subsubsection{When Simulations are Available for all Ensemble Members} \label{subsubsec:Emulation-of-the-Ensemble-Mean-NPV-when-Simulations-are-Available-for-all-Ensemble-Members}

When simulations are relatively quick to evaluate; large amounts of computing resources are available; or there is a desire to minimise the uncertainty (here due to the underlying geology, which is particularly relevant when the ensemble mean NPV is assumed equal to the expected NPV), it may be possible to simulate from the entire ensemble. The ensemble mean NPV is computed as either the arithmetic or a weighted mean (with weights obtained from a prior probability model over the geologies) of the individual model NPVs. This presents a natural method to emulate $\meanNPV$ with the adjusted expectation and variance defined in \cref{eq:Ensemble-Mean-NPV-all-members-emulator-adjusted-expectation,eq:Ensemble-Mean-NPV-all-members-emulator-adjusted-variance}, where $\boldF$ denotes all necessary simulation data, and weights $\omega_j$, with $\omega_j = \frac{1}{N}$ for the arithmetic mean.
\begin{align}
	\E_{\boldF}\left[ \meanNPVd \right] &{} = \sum_{j = 1}^{N} \omega_j \E_{\boldFj}[\NPVjd] \label{eq:Ensemble-Mean-NPV-all-members-emulator-adjusted-expectation} \\
	\Var_{\boldF}\left[ \meanNPVd \right] &{} =  \sum_{j = 1}^{N} \omega_j^2 \Var_{\boldFj}[\NPVjd] \label{eq:Ensemble-Mean-NPV-all-members-emulator-adjusted-variance}	
\end{align}
The variance formula may be adapted when different model NPVs are believed to be correlated by introducing the relevant covariance terms in \cref{eq:Ensemble-Mean-NPV-all-members-emulator-adjusted-variance}.



\subsubsection{Using the Ensemble Subsampling Linear Model} \label{subsubsec:Emulation-of-the-Ensemble-Mean-NPV-Using-the-Ensemble-Subampling-LM} %\label{subsubsec:Emulation-of-the-Ensemble-Mean-NPV-via-the-EGES-LM}


A more realistic and practical scenario is that simulations are only performed for a subset of the ensemble, such as selected using the techniques described in \cref{subsec:Subsampling-from-Multi-Model-Ensembles}. The linear model in \cref{eq:EGES-ensemble-mean-resp-linear-model-on-individual-model-resp-N_EGES-models-unknown} is used to emulate $\meanNPV$ with the emulated NPV for each of the sub-selected models as inputs. The estimated coefficients are denoted by $\hat{\alpha}_\mathEGES$ and $\hat{\beta}_{k, \mathEGES}$. It is assumed that the individual emulator outputs and the regression coefficients are uncorrelated, which is justifiable if two distinct simulation data sets are used to construct the linear model and fit the emulators. Under this formulation the adjusted expectation is shown in \cref{eq:Ensemble-Mean-NPV-Emulation-via-EGES-LM-adjusted-expectation}.
\begin{align*}
	\E_\boldF\left[ \meanNPVd \right] &{} = \E_{\boldF}\left[ \hat{\alpha}_\mathEGES + \sum_{k = 1}^{\Ntilde} \hat{\beta}_{k, \mathEGES} \NPV_{j_k}(\boldd) + \epsilonEGES(\boldd) \right] \\
	&{} = \hat{\alpha}_\mathEGES + \sum_{k = 1}^{\Ntilde} \hat{\beta}_{k, \mathEGES} \E_{\boldF_{j_k}}[\NPV_{j_k}(\boldd)] \alignnumber \label{eq:Ensemble-Mean-NPV-Emulation-via-EGES-LM-adjusted-expectation}
\end{align*}
Define $\betahatEGES = (\hat{\alpha}_\mathEGES, \hat{\beta}_{1, \mathEGES}, \ldots, \hat{\beta}_{\Ntilde, \mathEGES})^\Transpose \in \mathbb{R}^{\Ntilde + 1}$ with $\SigmabetaEGES = \Var\left[ \betahatEGES \right]$, and \lword{$\XEGESd = (1, \NPV_{j_1}(\boldd), \ldots, \NPV_{j_{\Ntilde}}(\boldd))^\Transpose \in \mathbb{R}^{\Ntilde + 1}$} with uncorrelated components, so $\Var_{\boldF}\left[ \XEGESd \right]$ is diagonal. The adjusted variance is presented in \cref{eq:Ensemble-Mean-NPV-Emulation-via-EGES-LM-adjusted-variance}, where $\sigmahatEGES$ is the estimated residual standard error for $\epsilonEGES(\boldd)$.
\begin{align*}
	\Var_{\boldF}\left[ \meanNPVd \right] &{}= \Var\left[ \hat{\alpha}_\mathEGES \right] \alignmultilineeq + \sum_{k = 1}^{\Ntilde} \Var\left[ \hat{\beta}_{k, \mathEGES} \right] \left( \Var_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] + \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right]^2 \right) \alignmultilineeq + 2 \sum_{k = 1}^{\Ntilde} \Cov\left[ \hat{\alpha}_\mathEGES, \hat{\beta}_{k, \mathEGES} \right] \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] \alignmultilineeq + \sum_{\substack{k \neq l \\ k, l = 1, \ldots, \Ntilde}} \left( \Cov\left[ \hat{\beta}_{k, \mathEGES}, \hat{\beta}_{l, \mathEGES} \right] \right. \alignmultilineeq \phantom{+ \sum_{\substack{k \neq l \\ k, l = 1, \ldots \Ntilde}}  \left( \right.} \left. \cdot \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] \E_{\boldF_{j_l}}[\NPV_{j_l}(\boldd)] \right) \alignmultilineeq + \sum_{k = 1}^{\Ntilde} \hat{\beta}_k^2 \Var_{\boldF_{j_k}}[\NPV_{j_k}(\boldd)] + \sigmahatEGES^2 \alignnumber \label{eq:Ensemble-Mean-NPV-Emulation-via-EGES-LM-adjusted-variance}
%	\Var_{\boldF}\left[ \meanNPVd \right] &{}= \Var_{\boldF}\left[ \hat{\alpha}_\mathEGES + \sum_{k = 1}^{\Ntilde} \hat{\beta}_{k, \mathEGES} \NPV_{j_k}(\boldd) + \epsilonEGES(\boldd) \right] \\
%	&{}= \Var_{\boldF}\left[ \XEGESTd \betahatEGES \right] + \Cov_{\boldF}\left[ \XEGESTd \betahatEGES, \epsilonEGES(\boldd) \right] \alignmultilineeq + \Cov_{\boldF}\left[ \epsilonEGES(\boldd), \XEGESTd \betahatEGES \right] + \Var_{\boldF}\left[ \epsilonEGES(\boldd) \right] \\
%	\intertext{Assuming that $\betaEGES$ and $\XEGESd$ are uncorrelated, and noting that \lword{$\Cov_{\boldF}\left[\XEGESTd \betahatEGES, \epsilonEGES(\boldd) \right] = \boldzero \in \mathbb{R}^{\Ntilde + 1}$}.}
%	&{}= \E_{\boldF}\left[ \XEGESTd \SigmabetaEGES \XEGESd \right] \alignmultilineeq + \betahatEGES^\Transpose \Var_{\boldF}\left[ \XEGESd \right] \betahatEGES + \sigmahatEGES^2 \\
%	\intertext{Assuming that the components of $\XEGESd$ are uncorrelated.}
%	&{}= \Var\left[ \hat{\alpha}_\mathEGES \right] \alignmultilineeq + \sum_{k = 1}^{\Ntilde} \Var\left[ \hat{\beta}_{k, \mathEGES} \right] \left( \Var_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] + \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right]^2 \right) \alignmultilineeq + 2 \sum_{k = 1}^{\Ntilde} \Cov\left[ \hat{\alpha}_\mathEGES, \hat{\beta}_{k, \mathEGES} \right] \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] \alignmultilineeq + \sum_{\substack{k \neq l \\ k, l = 1, \ldots, \Ntilde}} \left( \Cov\left[ \hat{\beta}_{k, \mathEGES}, \hat{\beta}_{l, \mathEGES} \right] \right. \alignmultilineeq \phantom{+ \sum_{\substack{k \neq l \\ k, l = 1, \ldots \Ntilde}}  \left( \right.} \left. \cdot \E_{\boldF_{j_k}}\left[ \NPV_{j_k}(\boldd) \right] \E_{\boldF_{j_l}}[\NPV_{j_l}(\boldd)] \right) \alignmultilineeq + \sum_{k = 1}^{\Ntilde} \hat{\beta}_k^2 \Var_{\boldF_{j_k}}[\NPV_{j_k}(\boldd)] + \sigmahatEGES^2 \alignnumber \label{eq:Ensemble-Mean-NPV-Emulation-via-EGES-LM-adjusted-variance}
\end{align*}



%%% Notes %%%
%See PhD Thesis Section 3.3.5.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents.tex <==
\subsection{Structured Emulators Exploiting Known Simulator Behaviour for NPV Constituents} \label{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents}

The emulation methodology presented here is motivated by the behavioural form observed for WOPT and WWIT outputs within control intervals with respect to the corresponding decision input parameters, the target production or injection rate for the control interval respectively, as shown in \cref{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-behaviour}. Within \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)} for OLYMPUS model $j$ the WOPT and WWIT are the by well constituents of the respective field totals $Q_{j,op}(\boldd, t_i)$ and $Q_{j,wi}(\boldd, t_i)$. Note that the $Q_{j,wp}(\boldd, t_i)$ can also be split by well to obtain WWPT outputs.
%Within \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)} the WOPT and WWIT are a decomposition of the terms $Q_{j,op}(\boldd, t_i)$ and $Q_{j,wi}(\boldd, t_i)$ by well.
%A by well decomposition also exists for $Q_{j,wp}(\boldd, t_i)$.
\begin{figure}[!th]
	\centering
	\includegraphics[page=1,width=\textwidth]{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Plots-OLYMPUS-25-w1-WOPT-contr-int-versus-corresponding-target-prod-rate-with-cp-lwr-and-cp-upr}
	\caption[OLYMPUS 25 WOPTPROD2\_20180101 versus prod\_2\_2016\_01]{OLYMPUS 25 WOPT output for producer well 2 during the first two years (ending 01/01/2018) versus the corresponding decision input parameter, the target production rate prod\_2\_2016\_01. For small values of prod\_2\_2016\_01 the target is achieved resulting in the perfect linear behaviour up to a change point beyond which the WOPT plateaus as a maximum threshold on the production rate is achieved. The vertical blue and red lines denote the extrapolation cut-off and change point upper bounds respectively.}
	\label{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-behaviour}
\end{figure}

Throughout this section we focus on emulating outputs for individual ensemble members and thus omit the OLYMPUS model index $j$ for clarity of notation. Let simulator output $f_i(\cdot)$ represent an NPV component by well. For the WOPT and WWIT constituents the corresponding decision input parameter which directly affects $f_i(\cdot)$ is labelled as $\dcp$. In this section the index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ refers to the well type ($P$ producer, $I$ injector), $k$ is the well number, and $t_i$ is the control interval start date. For each NPV contributor type $l \in \{ op, wp, wi \}$, the total over all wells, $Q_{l}(\boldd, t_i)$ (see \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)}), is obtained via a summation in \cref{eq:Q_l(d_t_i)-well-sum-decomposition}, where $N_l$ is the number of wells of the relevant type, and $f_{jk, t_i}^l(\boldd) \equiv f_i(\boldd)$ is the quantity for well $k$.
\begin{align} \label{eq:Q_l(d_t_i)-well-sum-decomposition}
	Q_{l}(\boldd, t_i) &{}= \sum_{k = 1}^{N_l} f_{jk, t_i}^l(\boldd)
\end{align}



%%% Version 4 %%%
%Throughout this section we omit the OLYMPUS model superscript $j$ for clarity of notation and emulate outputs for an individual ensemble member. In the well control optimisation problem let simulator output $f_i(\cdot)$ represent an NPV component by well. For the WOPT and WWIT constituents the corresponding decision input parameter which directly affects $f_i(\cdot)$ is labelled as $\dcp$. The index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ refers to the well type ($P$ producer, $I$ injector), $k$ is the well number, and $t_i$ is the control interval start date. The total of each NPV contributor over all wells, $Q_{op}(\boldd, t_i)$, $Q_{wp}(\boldd, t_i)$, and $Q_{wi}(\boldd, t_i)$, are obtained via a summation in \cref{eq:Q_j_op(d_t_i)-well-sum-decomposition,eq:Q_j_wp(d_t_i)-well-sum-decomposition,eq:Q_j_wi(d_t_i)-well-sum-decomposition}, where $N_P$ and $N_I$ are the number of producer and injector wells respectively. The additional superscript $l$ is used to clarify the well quantity type being summed such that $f_i(\boldd) \equiv f_i^l(\boldd)$ .
%\begin{align}
%	Q_{op}(\boldd, t_i) &{}= \sum_{k = 1}^{N_P} f_{Pk, t_i}^{op}(\boldd) \label{eq:Q_j_op(d_t_i)-well-sum-decomposition} \\
%	Q_{wp}(\boldd, t_i) &{}= \sum_{k = 1}^{N_I} f_{Ik, t_i}^{wp}(\boldd) \label{eq:Q_j_wp(d_t_i)-well-sum-decomposition} \\
%	Q_{wi}(\boldd, t_i) &{}= \sum_{k = 1}^{N_I} f_{Ik, t_i}^{wi}(\boldd) \label{eq:Q_j_wi(d_t_i)-well-sum-decomposition}
%\end{align}
%
%%% Version 3 %%%
%In the well control optimisation problem let simulator output $f_i(\cdot)$ represent an NPV component by well where the corresponding decision input parameter which directly affects $f_i(\cdot)$ is labelled as $\dcp$. The index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ refers to the well type ($P$ producer, $I$ injector), $k$ is the well number, and $t_i$ is the control interval start date. The terms $Q_{j,op}(\boldd, t_i)$ and $Q_{j,wi}(\boldd, t_i)$ are obtained via a summation in \cref{eq:Q_j_op(d_t_i)-well-sum-decomposition,eq:Q_j_wi(d_t_i)-well-sum-decomposition} where $N_P$ and $N_I$ are the number of producer and injector wells respectively.
%\begin{align}
%	Q_{j,op}(\boldd, t_i) &{}= \sum_{k = 1}^{N_P} f_{Pk, t_i}(\boldd) \label{eq:Q_j_op(d_t_i)-well-sum-decomposition} \\
%%	Q_{j,wp}(\boldd, t_i) &{}= \sum_{k = 1}^{N_I} f_{Ik, t_i}(\boldd) \label{eq:Q_j_wp(d_t_i)-well-sum-decomposition} \\
%	Q_{j,wi}(\boldd, t_i) &{}= \sum_{k = 1}^{N_I} f_{Ik, t_i}(\boldd) \label{eq:Q_j_wi(d_t_i)-well-sum-decomposition}
%\end{align}
%
%%% Version 2 %%%
%%% Note that this also uses the preceeding sentence regarding WWPT.uses 
%In the well control optimisation problem let simulator output $f_i(\cdot)$ represent an NPV component by well. For the WOPT and WWIT constituents the corresponding decision input parameter which directly affects $f_i(\cdot)$ is labelled as $\dcp$. The index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ refers to the well type ($P$ producer, $I$ injector), $k$ is the well number, and $t_i$ is the control interval start date. The terms .... are thus obtained via a summation in eq..., where $N_P$ and $N_I$ are the number of producer and injector wells respectively.
%
%%% Version 1 %%%
%In the well control optimisation problem we denote these by well NPV constituents as the simulator output $f_i(\cdot)$, where for WOPT and WWIT constituents the corresponding decision input parameter which directly effects $f_i(\cdot)$ is labelled as $\dcp$. The index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ refers to the well type ($P$ producer, $I$ injector), $k$ is the well number, and $t_i$ is the control interval start date.



\subsubsection{Change Points} \label{subsubsec:Structured-Emulation-Change-Points}

The target control rate should be adhered to for the duration of the interval. However, this is not always possible due to Bottom Hole Pressure (BHP) constraints suggesting two theoretical distinct modes of behaviour termed the slope and plateau regions. In the slope the target rate is adhered to for the full duration of the control interval, whilst within the plateau region this is not the case. The slope therefore possesses a known gradient which is equal to the length of the control interval, thus $\fid = \dcp \cdot \Delta t_i$. The decision parameter value of transition from slope to plateau is designated the change point and denoted $\cp{jk}{t_i}$. This is unknown, dependent on all other decision parameters, and given only a finite number of simulations is impossible to exactly determine. Consequently, in practical application, there are three distinct regions of behaviour: the slope and plateau separated by an additional uncertain region believed to contain the unknown change point. For a simulator output $f_i(\cdot)$ which follows such behaviour the left-hand slope is precisely known up to a tolerance $\delta_i \geq 0$; this can be used to estimate the mean change point location given a collection of simulations from design $\mathcal{D}$. 
%%% Version 1 %%%
%The target control rate should be adhered to for the duration of the interval. However, this is not always possible due to Bottom Hole Pressure (BHP) constraints suggesting two theoretical distinct modes of behaviour termed the slope and plateau regions. In the slope the target rate is adhered to for the full duration of the control interval, whilst within the plateau region this is not the case. The slope therefore possesses a known gradient which is equal to the length of the control interval, thus $\fid = \dcp \cdot \Delta t_i$. The decision parameter value of transition from slope to plateau is designated the change point. This is unknown, dependent on all other decision parameters, and given only a finite number of simulations is impossible to exactly determine. Consequently, in practical application, there are three distinct regions of behaviour: the slope and plateau separated by an additional uncertain region believed to contain the unknown change point. For a simulator output $f_i(\cdot)$ which follows such behaviour the left-hand slope is precisely known up to a tolerance $\delta_i \geq 0$; this can be used to estimate the mean change point location given a collection of simulations from design $\mathcal{D}$. In the well control optimisation problem, let $\dcp$ be the decision parameter which directly effects NPV constituent $f_i(\cdot)$ with change point $\cp{jk}{t_i}$. The index $i$ is condensed notation for the indices tuple $(jk, t_i)$, where $j \in \{ P, I \}$ and $k$ refer to the well type ($P$ producer, $I$ injector) and number respectively, whilst $t_i$ is the control interval start date.

A conservative change point upper bound estimate, $\cpu{jk}{t_i}$, is defined in \cref{eq:Change-point-upper-bound}, where $f_{i, \mathrm{max}} = \max_{\boldd \in \mathcal{D}} \fid$, and $\delta_{i,u} \geq 0$ is a tolerance included for numerical stability and to ensure that an upper bound is obtained.
\begin{align} \label{eq:Change-point-upper-bound}
	\cpu{jk}{t_i} = \min_{\dcp} \{ \dcp \mid \dcp \cdot \Delta t_i \geq f_{i, \mathrm{max}} + \delta_{i,u} \}
\end{align}
This is the smallest value of the corresponding decision parameter for which if the target was achieved for the entire control interval, then the simulator output would exceed the largest simulated value (plus a tolerance) over $\mathcal{D}$.

An estimate for the change point lower bound is defined in \cref{eq:Change-point-lower-bound}, where $f_{i, \mathrm{diff}}(\boldd) = f_{i, \mathrm{max}}(\boldd) - \fid = \dcp \cdot \Delta t_i - \fid$, and $\delta_{i, l} \geq 0$ is another numerical stability tolerance.
\begin{align*} \label{eq:Change-point-lower-bound}
	\cpl{jk}{t} &{} = \dfrac{1}{2} \left( \argmin_{\dcp \mid \boldd \in \mathcal{D}} \{ \fid < \dcp \cdot \Delta t_i - \delta_{i,l} \} \right. \alignmultilineeq \left. + \argmax_{\dcp \mid \boldd \in \mathcal{D}} \left\{ \dcp < \argmin_{\dcp \mid \boldd \in \mathcal{D}} \{ \fid < \dcp \cdot \Delta t_i - \delta_{i,l} \} \right\} \right) \alignnumber
\end{align*}
This is illustrated in \cref{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-for-cp-lwr-zoom} for the output WOPTPROD2\_20180101 versus the target rate prod\_2\_2016\_01 where the red line represents the slope upper bound if the target is fully adhered to. The vertical blue line denotes $\cpl{P2}{2016}$ as the midpoint between the first simulation decision parameter setting not on the slope; hence with $f_{i, \mathrm{diff}}(\boldd) > \delta_{i,l}$ (green point; first term in \cref{eq:Change-point-lower-bound}), and the decision parameter setting with the largest value of $d_{jk,t_i}$ which is less than this first departure point previously obtained (magenta point; second term in \cref{eq:Change-point-lower-bound}).

\begin{figure}[!t]%[!ht]
	\centering
	\includegraphics[page=1,width=\textwidth]{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Plots-OLYMPUS-25-w1-WOPT-contr-int-versus-corresponding-target-prod-rate-cp-lwr-plot-zoom}
	\caption[OLYMPUS 25 WOPTPROD2\_20180101 versus prod\_2\_2016\_01 focused around $\cppl{2}{2016}$]{OLYMPUS 25 WOPT for producer well 2 during the first two years (ending 01/01/2018) versus the corresponding target production rate, prod\_2\_2016\_01. The focus on the change point lower bound, $\cppl{2}{2016}$, computed using \cref{eq:Change-point-lower-bound}, and denoted by the vertical blue line. The red line depicts the slope upper bound attained when the target production rate is adhered to for the full control interval. It is shown that $\cppl{2}{2016}$ is the midpoint of the first point not on the slope coloured green, and preceding point which is on the slope coloured magenta.}
	\label{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-for-cp-lwr-zoom}
\end{figure}



\subsubsection{Extrapolation Cut-Offs} \label{subsubsec:Structured-Emulation-Extrapolation-Cut-Offs}

The two distinct modes of behaviour for NPV constituents suggests an emulator be fitted piecewise using a combination of the more accurate knowledge in the slope region, and the less well understood behaviour in the plateau region. Noting the change point location uncertainty, for the plateau region we propose fitting an emulator based only on data which is almost certainly on plateau using the change point upper bound estimate. For $f_i(\cdot)$ this is design points with $\dcp \geq \cpu{jk}{t_i}$. In order to connect the slope and plateau regions we must extrapolate the plateau emulator. It is necessary to introduce an extrapolation cut-off, denoted $\extrapco{jk}{t_i}$, beyond which the emulator should not be extrapolated. This is due to limited plateau training data issues. For simulator output $\fid$ this is defined with respect to the same decision parameter, $\dcp$. The decision space is thus split into three distinct regions:
\begin{enumerate}
	\item \textbf{Slope Region:} where $\dcp < \extrapco{jk}{t_i}$;
	
	\item \textbf{Intermediate Region:} where $\extrapco{jk}{t_i} \leq \dcp < \cpu{jk}{t_i}$, for which there is uncertainty as to whether simulator output falls on the slope or in the plateau;
	
	\item \textbf{Plateau Region:} where $\dcp \geq \cpu{jk}{t_i}$.
\end{enumerate}
There is an estimation trade-off between overly cautious small values which fails to alleviate the above issue, and large values risking  points being wrongly classified as on the slope. A suitable and sufficiently conservative approach is to use the change point lower bound, so $\extrapco{jk}{t_i} = \cpl{jk}{t_i}$ (see \cref{eq:Change-point-lower-bound}). %, thus it is guaranteed that the smallest value of $\dcp$ for which the simulated data does not lie on the slope will exceed $\extrapco{jk}{t_i}$.
The three regions obtained by splitting WOPTPROD2\_20180101 versus prod\_2\_2016\_01 at $\extrapcop{2}{2016} = \cppl{2}{2016}$ and $\cppu{2}{2016}$ are illustrated in \cref{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-behaviour} by the vertical blue and red lines respectively.



\subsubsection{Structured Emulation with Upper Truncation} \label{subsubsec:Structured-Emulation-Methodology}
%\subsubsection{Structured Emulation with Upper Truncation}%Note that this should actually be a subsubsubsection or paragraph.

Prior information stipulates that the WOPT and WWIT NPV constituents cannot exceed a maximum (up to a tolerance) determined by the prescribed target rate and control interval length. This upper bound is $\dcp \cdot \Delta t_i$. Alongside the above parameter space dichotomy, this constraint is imposed through an upper truncation with structured emulators respecting partially known behaviour of these simulator outputs. First a preliminary Bayes linear emulator for $\fid$ is fitted using a sub-design, $\mathcal{D}_i^\prime = \{ \boldd \mid \boldd \in \mathcal{D},\ \dcp > \cpu{jk}{t_i} \}$, with corresponding simulator output $\boldFi^\prime = \{ \fid \mid \boldd \in \mathcal{D}_i^\prime \}$. This represents the behaviour in the plateau region. By construction, all parameter settings in $\mathcal{D}_i^\prime$ do not adhere to the target rate and hence are in the plateau, thus providing reliable information on which to construct this part of the emulator. % Note that there may exist simulated parameter settings with $\extrapco{jk}{t_i} \leq \dcp < \cpu{jk}{t_i}$ which are not on the slope, although these are more difficult to accurately determine and less reliable for use in fitting this preliminary emulator.
This preliminary emulator is only evaluated for $\boldd$ satisfying $\dcp \geq \extrapco{jk}{t_i}$ and is compared with the upper bound in a classification step determining the structured emulator form:
\begin{enumerate*}
	\item \textbf{Slope Region:} If $\dcp < \extrapco{jk}{t_i}$ \textbf{or} for the preliminary emulator  \lword{$\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} > \dcp \cdot \Delta t_i$}, then collapse the emulator such that for the structured emulator $\E_{\boldFi^\prime}[\fid] = \dcp \cdot \Delta t_i$ with fixed maximum absolute errors of size $\delta_i$.% This corresponds to when the output is strongly believed to be in the slope region.
	
%	\item \textbf{Uncertain Region around Change Point:} If the preliminary emulator satisfies $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i < \E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]}$, a truncated Gaussian process (truncated GP) emulator which is evaluated with mean and variance determined by \cref{eq:Truncated-normal-distribution-mean,eq:Truncated-normal-distribution-variance} respectively \cite{1994:Johnson:Continuous-Univariate-Distributions-Vol-1}, where $\phi(\cdot)$ and $\Phi(\cdot)$ represent the probability density and cumulative distribution functions respectively of a standard normal distribution. These are computed assuming a preliminary Gaussian process emulator with posterior mean and variance, abbreviated to $\mu_i$ and $\sigma_i^2$ respectively, equal to the computed adjusted expectation and variance. The truncation bounds are $a_i = -\infty$ and $b_i = \dcp \cdot \Delta t_i$, with $\alpha_i = \frac{a_i - \mu_i}{\sigma_i} = -\infty$, and \lword{$\beta_i = \frac{b_i - \mu_i}{\sigma_i}$}. This form of emulation is used in the uncertain region around the true location of the change point.
	\item \textbf{Intermediate Region:} If the preliminary emulator satisfies $\E_{\boldFi^\prime}[\fid] - 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i < \E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]}$, a truncated Gaussian process (truncated GP) emulator is used with mean and variance determined by \cref{eq:Truncated-normal-distribution-mean,eq:Truncated-normal-distribution-variance} respectively \cite{1994:Johnson:Continuous-Univariate-Distributions-Vol-1}.% This form of emulation is used in the uncertain region around the true location of the change point.
	
	\item \textbf{Plateau Region:} In all other cases where $\E_{\boldFi^\prime}[\fid] + 3 \sqrt{\Var_{\boldFi^\prime}[\fid]} \leq \dcp \cdot \Delta t_i$, the preliminary emulator output is used.% which corresponds to when the output is strongly believed to be in the plateau region.
\end{enumerate*}
A structured emulation two-sided truncated variant is also developed and presented in \cref{sec:Structured-Emulation-with-Two-Sided-Truncation}, although is unnecessary for the purposes of this application to the \TNOChallengeWC{}. Alternative width credible intervals may be used depending on the level of conservativeness desired within an analysis with justification based on the Vysochanskij-Petunin inequality \cite{1980:Vysochanskij:3-sigma-rule-for-unimodal-distributions}.
%An alternative structured emulator variant using a two-sided truncation is also developed and presented in \cref{sec:Structured-Emulation-with-Two-Sided-Truncation}, although is unnecessary for the purposes of this application to the \TNOChallengeWC{}.

Compared to using standard Gaussian process or Bayes linear emulators, the above described structured approach yields improved accuracy, along with an increase in speed and efficiency; a consequence of using fewer design points in the fitting. Moreover, both the change point upper bound and extrapolation cut-off estimation processes are computationally very cheap, whilst the use of a truncated GP helps reduce the reliance on accurate estimation of the extrapolation cut-off. The presented methodology is also preferred to alternative partition based emulation approaches for functions with distinct modes of behaviour in different regions of the parameter space such as Treed Gaussian processes \cite{2008:Gramacy-and-Lee:Bayesian-Treed-Gaussian-Process-Models-with-an-Application-to-Computer-Modeling} because for each NPV constituent the form of the behaviour within the slope region is almost exactly known up to a very small tolerance. This is encapsulated within the developed form of structured emulation. However, treed GPs maintain a much larger uncertainty over this region than necessary, whilst struggling when the number of design points within each region is relatively limited impacting further on the treed GP accuracy. This consideration has implications during subsequent (decision) analyses.

Each NPV constituent is emulated separately by well before combining in a ``divide and conquer approach'' to obtain an overall emulator of improved accuracy. The emulator adjusted expectation and variance for $Q_{j,op}(\boldd, t_i)$, $Q_{j,wp}(\boldd, t_i)$, and $Q_{j,wi}(\boldd, t_i)$ in \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)} are shown in \cref{eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-expectation,eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-variance} respectively, where $\mathbf{F}_j$ represents all data used to fit the NPV constituents emulators for OLYMPUS model $j$.
\begin{align} 
	\E_\boldF\left[ Q_{l}(\boldd, t_i) \right] &{}= \sum_{k = 1}^{N_l} \E_\boldF\left[ f_{jk, t_i}^l(\boldd) \right] \label{eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-expectation} \\
	\Var_\boldF\left[ Q_{l}(\boldd, t_i) \right] &{}= \sum_{k = 1}^{N_l} \Var_\boldF\left[ f_{jk, t_i}^l(\boldd) \right] \label{eq:Q_l(d_t_i)-well-sum-decomposition-adjusted-variance}
\end{align}



%%% Full justification for the presented structured emulation methodology. %%%
%Compared to applying standard methods such as Gaussian process or Bayes linear emulation, the structured approach demonstrates improvements in accuracy. Moreover, an auxiliary benefit is the increased speed of emulator evaluation and efficiency. This is as a consequence of using fewer design points in the fitting (only those which exceed the change point upper bound) leading to inversions and multiplications of smaller matrices, and the restriction to only performing a full emulator update at new decision parameter vectors which exceed the extrapolation cut-off whilst all others are automatically collapsed onto the slope in order to satisfy the physical constraints. The estimation processes for both the change point upper bound and extrapolation cut-off are computationally very cheap, whilst the use of a truncated GP helps reduce the reliance on accurate estimation of the extrapolation cut-off.
%
%The presented methods are also preferred over alternative approaches to emulating functions with distinct modes of behaviour in different regions of the parameter space such as Treed Gaussian processes \cite{2008:Gramacy-and-Lee:Bayesian-Treed-Gaussian-Process-Models-with-an-Application-to-Computer-Modeling} because for each NPV constituent the form of the behaviour within the slope region is almost exactly known up to a very small tolerance. This is encapsulated within the developed form of structured emulation where as a Treed GP would maintain a much larger uncertainty over this region than is necessary with potential implications during subsequent analyses. Moreover, in later application it is highlighted how in certain instances the number of points within these distinct regions can be relatively limited. This potentially impacts on the accuracy of a Treed GP.
%
%Both developed forms of the structured emulation technique allow more complex outputs such as the NPV to be deconstructed into their constituents which exhibit features such as slopes and plateaus. These are emulated separately before combining in a ``divide and conquer approach'' to obtain an emulator of improved accuracy.



%%% Notes %%%
%See PhD Thesis Section 3.3.2.
%
%A structured emulation two-sided truncated variant is also developed in \cite[Sec.~3.3.2]{2022:Owen:PhD-Thesis}, although it is unnecessary for the purposes of this application to the \TNOChallengeWC{}.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour.tex <==
\section{Hierarchical Emulators Exploiting Known Simulator Behaviour} \label{sec:Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour}

Bayesian emulators frequently yield fast and effective approximations to the outputs of ``black-box'' computer models for which the user possesses no insight of the structure or links between individual processes, as well as no knowledge of the model behaviour for specific outputs at a given parameter setting prior to its evaluation. However, this may limit the accuracy of general emulators in scenarios where such prior information is available: a ``grey-box'' simulator. This is the case for the \TNOChallengeWC{} in \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge} where the quantity of interest, the expected NPV objective function in \cref{eq:Expected-NPV-general-formula-in-decision-parameters}, is first split by OLYMPUS model in \cref{eq:NPV-general-formula-in-decision-parameters}, and then by time interval and field total outputs in \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)}. This is divided further into Well Oil Production Total (WOPT), Well Water Injection Total (WWIT), and Well Water Production Total (WWPT), within each time interval. WOPT and WWIT exhibit constrained and structured behaviour with respect to their corresponding target rate parameters. 

In this section we present a hierarchical emulator designed to open the ``black-box'' and exploit known structures between the simulator outputs and any functions thereof. To reduce computational costs, we first describe methods for identifying a representative subset of models in \ref{subsec:Subsampling-from-Multi-Model-Ensembles}. Next we present structured emulation of outputs of a recurring form in \ref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents}. In the context of well control optimisation we introduce an approximation to the NPV for an individual model and its emulation in \ref{subsec:Emulation-of-the-Approximate-NPV}, before linking to the exact NPV in \ref{subsec:Linking-the-Exact-and-Approximate-NPV}. Finally, the methods of \cref{subsec:Subsampling-from-Multi-Model-Ensembles} are employed to emulate the ensemble mean NPV as a proxy for the expected NPV in \ref{subsec:Emulation-of-the-Ensemble-Mean-NPV}.%, with a summary in \ref{subsec:Summary-Hierarchical-Emulation}.



%%% Notes %%%
%Introduction comments.
%
%The quantity of interest is a function of multiple simulator outputs these may be emulated more accurately by breaking into the simulator structure (treating it as a grey box) and exploiting partially known behaviour of certain computer model outputs

\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Subsampling-from-Multi-Model-Ensembles.tex}

\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents.tex}

\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulation-of-the-Approximate-NPV.tex}

\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Linking-the-Exact-and-Approximate-NPV.tex}

\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Emulation-of-the-Ensemble-Mean-NPV.tex}

%\input{Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Summary-Hierarchical-Emulation.tex}

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Linking-the-Exact-and-Approximate-NPV.tex <==
\subsection{Linking the Exact and Approximate NPV} \label{subsec:Linking-the-Exact-and-Approximate-NPV}

There exists a very strong linear relationship between the approximate and exact NPV for which a simple linear regression in \cref{eq:Exact-NPV_j-on-Approximate-NPV_j-LM-form} provides a meaningful statistical link whilst capturing the additional induced uncertainties.
\begin{align} \label{eq:Exact-NPV_j-on-Approximate-NPV_j-LM-form}
	\NPVjd = \beta_{0, \approxNPVj} + \beta_{1, \approxNPVj} \approxNPVjd	+ \varepsilon_{\approxNPVj}
\end{align}
The adjusted expectation and variance are then computed using \cref{eq:Exact-NPV_j-on-Approximate-NPV_j-emulation-via-LM-adjusted-expectation,eq:Exact-NPV_j-on-Approximate-NPV_j-emulation-via-LM-adjusted-variance} respectively. 
Estimates of the regression coefficients, $\hat{\beta}_{0, \approxNPVj}$ and $\hat{\beta}_{1, \approxNPVj}$, along with their variances and covariance, are obtained using the wave 0 simulation data, whilst $\varepsilon_{\approxNPVj}$ is treated as independent with residual standard error $\sigma_{\approxNPVj}$.
%The regression coefficients, their variances, and covariance are estimated using the simulation data, whilst $\varepsilon_{\approxNPVj}$ is treated as independent with residual standard error $\sigma_{\approxNPVj}$.
\begin{align*}
	\E_{\boldFj}[\NPVjd] &{} = \hat{\beta}_{0, \approxNPVj} + \hat{\beta}_{1, \approxNPVj} \E_{\boldFj}\left[ \approxNPVjd \right] \alignnumber \label{eq:Exact-NPV_j-on-Approximate-NPV_j-emulation-via-LM-adjusted-expectation} \\
	\Var_{\boldFj}[\NPVjd] &{} = \Var\left[ \hat{\beta}_{0, \approxNPVj} \right] + 2 \Cov\left[ \hat{\beta}_{0, \approxNPVj}, \hat{\beta}_{1, \approxNPVj} \right] \E_{\boldFj}\left[ \approxNPVjd \right] \alignmultilineeq
	+ \left\{ \hat{\beta}_{1, \approxNPVj}^2 + \Var\left[ \hat{\beta}_{1, \approxNPVj} \right] \right\} \Var_{\boldFj}\left[ \approxNPVjd \right] \alignmultilineeq
	+ \Var\left[ \hat{\beta}_{1, \approxNPVj} \right] \left( \E_{\boldFj}\left[ \approxNPVjd \right] \right)^2 + \sigma_{\approxNPVj}^2 \alignnumber \label{eq:Exact-NPV_j-on-Approximate-NPV_j-emulation-via-LM-adjusted-variance}
\end{align*}



%%% Notes %%%
%See PhD Thesis Section 3.3.4.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Subsampling-from-Multi-Model-Ensembles.tex <==
\subsection{Subsampling from Multi-Model Ensembles} \label{subsec:Subsampling-from-Multi-Model-Ensembles}

Multi-model ensembles are frequently employed to characterise various forms of uncertainty. In the petroleum industry these are prevalent for representing uncertainty induced by the unknown underlying field geology, reflecting the geologist's beliefs. In the \TNOChallengeshort{} this consists of 50 versions of the OLYMPUS model realised from an underlying stochastic geology model (note that the geology model was not released so no further realisations were possible). However, running every model requires a greater number of simulations placing a higher strain on computational resources. In many analyses the multi-model outputs are amalgamated such as through averaging; termed the ensemble mean. This is the case in the \TNOChallengeshort{} where the ensemble mean NPV is the focus. Whilst such quantities are easier to analyse and use, the averaging process reduces the benefits of starting with an ensemble by collapsing the uncertainty onto a single value. It is therefore desirable to establish a subset of the ensemble to use as a surrogate, whilst acknowledging any reduction in information gained from the simulations.

The process of identifying a representative subset requires a small exploratory design using all models in the ensemble; a wave 0 design, for example, constructed using a maximin Latin hypercube design \cite{1989:Sacks:Design-and-Analysis-of-Computer-Experiments,2003:Santner:The-Design-and-Analysis-of-Computer-Experiments}, in order to assess how well a given subset of models represents the ensemble mean for certain key outputs. First we propose an initial graphical investigation using plots of ensemble mean outputs versus that obtained using individual models. This provides insight into patterns where a strong linear correlation indicates that an individual model may be a good representative for the ensemble mean. Note that such plots are unable to capture the interaction between multiple models' outputs, thus missing where two or more models are jointly able to characterise the ensemble mean, often to a better extent than any one individual model. For large ensembles, this can be a useful screening process to identify a preliminary ensemble subset for further analysis.% and on which to perform the next step of this EGES technique where it may be computationally impractical from both a time or memory perspective to perform exhaustive investigations over all possible subsets.

Linear models provide a fast and effective tool for predicting the ensemble mean output, $\bar{f}(\cdot)$, for example, $\bar{f}(\boldd) = \meanNPVd$, from individual model outputs, $f^{(i_k)}(\cdot)$, $i_k \in \{ 1, \ldots, N \}$ distinct, as well as for quantifying the induced uncertainty. For an ensemble of size $N$ the aim is to select the best subset of $\Ntilde < N$ (to be determined) models. Since the ensemble mean is a linear combination of the individual models' output, an affine linear transformation of a subset of models is expected to yield good approximations. We propose the linear model in \cref{eq:EGES-ensemble-mean-resp-linear-model-on-individual-model-resp-N_EGES-models-unknown} where $\alpha_\mathEGES$ and $\beta_{k, \mathEGES}$ are unknown regression coefficients to be estimated, and $\varepsilon_{\mathEGES}(\boldd)$ is an uncorrelated error term.
\begin{align} \label{eq:EGES-ensemble-mean-resp-linear-model-on-individual-model-resp-N_EGES-models-unknown}
	\bar{f}(\boldd) &{} = \alpha_\mathEGES + \sum_{k = 1}^{\Ntilde} \beta_{k, \mathEGES} f^{(i_k)}(\boldd) + \varepsilon_{\mathEGES}(\boldd)
\end{align}
Depending on the size of $N$, either an exhaustive or stepwise model selection may be performed to identify the most suitable choice of $\Ntilde$ and model subset, for example, using the Akaike Information Criterion (AIC) or Bayesian information Criterion (BIC). Note that at later stages within an analysis it is always possible to modify this choice if increased accuracy is required; a scenario that naturally occurs within iterative procedures such as history matching and decision support. In the context of petroleum reservoir field development optimisation we refer to this as Efficient Geological Ensemble Subsampling (EGES) \cite{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty}. This technique is related to second-order multi-model ensemble exchangeability in \cite{2013:Rougier:Second-Order-Exchangeability-Analysis-for-Multimodel-Ensembles} where coexchangeability is used to establish a link between: the output of individual models; a common ``representative simulator'', which we interpret as the ensemble mean simulator; the output for the real world system as the true expected NPV with respect to all possible geological configurations; as well as any system observations.% Note that our approach does not explicitly assume second-order exchangeability of ensemble members.



%%% Notes %%%
%Describe efficient geological ensemble subsampling.
%
%See PhD Thesis Section 3.2.

==> Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Summary-Hierarchical-Emulation.tex <==
\subsection{Summary} \label{subsec:Summary-Hierarchical-Emulation}

See PhD Thesis Section 3.3.6.

==> Introduction/Introduction-V1.tex <==
\section{Introduction} \label{sec:Introduction}

Mathematical models of complex real world physical systems in the form of numerical codes known as computer models or simulators are prevalent across many scientific disciplines, industry, and government. They are used to: study the dynamics of physical systems; calibrate or history match to observation data; and to guide decision making processes. However, computer models commonly exhibit a complex structure; possess large numbers of inputs and outputs, including spatial-temporal fields; and crucially have a high computational expense of evaluation. In order to address such challenges, a suite of Bayesian uncertainty analysis methodology has been developed for using computer models to perform inferences about real world systems. Of principal importance are Bayesian emulators, also known as surrogate models, which provide fast statistical approximations to (functions of) the computer model outputs for as yet unevaluated parameter settings, along with a corresponding statement of the associated uncertainty. They are typically many orders of magnitude quicker to evaluate than the computer model. Emulators have been successfully employed across a wide range of applications including: climate science \cite{2006:Goldstein:Bayes-Linear-Calibrated-Prediction-for-Complex-Systems,2009:Rougier:Expert-Knowledge-and-Multivariate-Emulation-The-TIE-GCM,2013:Williamson:History-matching-for-exploring-and-reducing-climate-model-parameter-space-using-observations-and-a-large-perturbed-physics-ensemble,2019:Edwards:Revisiting-Antarctic-ice-loss-due-to-marine-ice-cliff-instability}; cosmology \cite{2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2014:Vernon:Bayesian-History-Matching-Galaxy-Formation,2009:Heitmann:The-Coyote-Universe-II-Cosmological-Models-and-Precision-Emulation-of-the-Nonlinear-Matter-Power-Spectrum,2011:Kaufman:Efficient-emulators-of-computer-experiments-using-compactly-supported-correlation-functions-with-an-application-to-cosmology}; epidemiology \cite{2015:Andrianakis:Bayesian-History-Matching-of-Complex-Infectious-Disease-Models-Using-Emulation-A-Tutorial-and-a-Case-Study-on-HIV-in-Uganda,2017:Andrianakis:History-matching-of-a-complex-epidemiological-model-of-HIV-transmission-by-using-variance-emulation,2022:Vernon:Bayesian-Emulation-and-History-Matching-of-JUNE}; and petroleum reservoir engineering \cite{1996:Craig:Bayes-linear-strategies-matching-hydrocarbon-reservoir-history,1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,1998:Craig:Constructing-partial-prior-specifications,2001:Craig:Bayesian-Forecasting-Using-Computer-Simulators,1998:O'Hagan:Uncertainty-Analysis-and-other-Inference-Tools-for-Complex-Computer-Codes,2010:Cumming:Multiscale-Bayes-Linear-Uncertainty-Analysis-Oil-Reservoirs}.

Emulation is frequently based on the assumption that a computer model behaves like a ``black-box'' function: the output at a given parameter setting is unknown prior to model evaluation; as well as users' possessing no insight of the structure or links between individual physical processes. Whilst this assumption ensures that emulation methodology is generalisable, it potentially limits the emulator accuracy compared to when a user has an understanding of how certain outputs behave with respect to changes in the inputs. In this paper we assume a ``grey-box'' simulator and address the problem of exploiting known behaviour of components of the simulator output of interest by developing a novel hierarchical emulation framework to obtain a physically interpretable emulator and more accurate predictions.

This research is motivated by the highly complex and commercially significant \TNOChallengeWC{} \cite{2017:TNO:OLYMPUS-oil-Reservoir-Model,2018:ISAPP:Website} from the petroleum industry. The aim is to maximise the expected Net Present Value (NPV) objective function over the field lifetime with respect to well control decision parameters (target production and injection rates), whilst accounting for geological uncertainty represented through a multi-model ensemble of 50 realisations from an underlying stochastic geology model. We recast this as a decision support problem for which emulation and Bayesian uncertainty analysis techniques are essential due to the computational expense of the ensemble and high-dimensionality of the decision parameter space. First we present efficient multi-model ensemble subsampling techniques to identify a representative subset of models in a novel application to petroleum reservoir engineering, thus greatly reducing the computational expense of the analysis. For each ensemble member the NPV is computed as the discounted sum of numerous simulator outputs; many exhibiting known constrained or structured behaviour with respect to their corresponding well control parameters, for which we formulate structured emulators and combine within our hierarchical emulation construction. We demonstrate a notable reduction in the emulator uncertainty compared with uninformed Bayes linear emulators. Whilst we establish our techniques in the context of decision support for well control optimisation under uncertainty, the overarching framework is flexible and adaptable to handle other structured forms of simulator outputs. 

In \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge} we describe the motivating \TNOChallenge{}. \Cref{sec:Bayesian-Emulation} provides an overview of Bayesian emulation methodology. The hierarchical emulator exploiting known constrained and structured behaviour of simulator outputs is devised in \cref{sec:Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour}, along with a multi-model ensemble subsampling technique. The methodology is applied to the \TNOChallengeWC{} expected NPV utility function in view of performing a decision support analysis in \cref{sec:Results}, with a conclusion and future directions in \cref{sec:Conclusion}.



%%% Notes %%%
%Present overview of problem.
%
%See PhD Thesis Section 3.3.1 -- Motivation.
%
%Motivation: Improved decision support under uncertainty using complex computer models by obtaining more accurate emulators.
%This research was motivated by the highly complex and commercially significant \TNOChallenge{} \cite{2018:ISAPP:Website}.
%
%Question to answer: How can we exploit structure within components of the simulator output of interest to build more accurate emulation models?
%
%Treat the simulator as a grey box. Can we use the knowledge of underlying physical behaviour, rather than purely creating more flexible models such as deep GPs.
%
%Describe the large amount of literature on emulating computer models.
%
%Introduce the TNO OLYMPUS Well Control Optimisation Challenge
%\cite{2018:ISAPP:Website}
%\cite{2017:TNO:OLYMPUS-oil-Reservoir-Model}
%
%Add plot showing WOPT vs target production rate to illustrate the type of behaviour.
%Also occurs for WWIT vs target injection rate.
%Comment that this is not the case for WWPT since there is no direct control variable and is a consequence of both types of controls and the constraints imposed within the simulator.
%
%Overview of Bayesian emulators, noting that these usually treat the output of interest as a black box function. These have been (successfully) employed across a wide range of applications including:
%Cosmology \cite{2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation,2014:Vernon:Bayesian-History-Matching-Galaxy-Formation,2009:Heitmann:The-Coyote-Universe-II-Cosmological-Models-and-Precision-Emulation-of-the-Nonlinear-Matter-Power-Spectrum}
%Epidemiology \cite{2015:Andrianakis:Bayesian-History-Matching-of-Complex-Infectious-Disease-Models-Using-Emulation-A-Tutorial-and-a-Case-Study-on-HIV-in-Uganda,2017:Andrianakis:History-matching-of-a-complex-epidemiological-model-of-HIV-transmission-by-using-variance-emulation,2022:Vernon:Bayesian-Emulation-and-History-Matching-of-JUNE}
%Climate science \cite{2009:Rougier:Expert-Knowledge-and-Multivariate-Emulation-The-TIE-GCM,2019:Edwards:Revisiting-Antarctic-ice-loss-due-to-marine-ice-cliff-instability,2013:Williamson:History-matching-for-exploring-and-reducing-climate-model-parameter-space-using-observations-and-a-large-perturbed-physics-ensemble}
%Petroleum reservoir modelling \cite{1996:Craig:Bayes-linear-strategies-matching-hydrocarbon-reservoir-history,1997:Craig:Pressure-matching-Bayes-linear-strategies-large-computer-experiments,2010:Cumming:Multiscale-Bayes-Linear-Uncertainty-Analysis-Oil-Reservoirs}
%
%Finish with details of the contents of each section of the paper.

==> PhD-Paper-1-NPV-Emulation-Preamble-Newcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Preamble Document Defining New Commands and Environments %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Paper Drafting Commands %%%

% Add comments within paper draft.
\newcommand{\comment}[1]{\textcolor{red}{\textbf{#1}}}

% Add note to add citation.
\newcommand{\addcitation}[1]{\textcolor{blue}{\textbf{ADD CITATION: #1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Provide itemize without extra spacing.
\newenvironment{itemize*}%
{\begin{itemize}%
		\setlength{\itemsep}{0pt}%
		\setlength{\parskip}{0pt}}%
	{\end{itemize}}
% Provide enumerate without extra spacing.
\newenvironment{enumerate*}%
{\begin{enumerate}%
		\setlength{\itemsep}{0pt}%
		\setlength{\parskip}{0pt}}%
	{\end{enumerate}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% R Commands %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\R}{R}    % Define the R Statistical programming language symbol.
\newcommand{\Rpkg}[1]{\textsf{#1}}    % R Package formatting.
\newcommand{\Rcode}[1]{\texttt{#1}}    % R code formatting

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Command for handling long words by forcing line breaks.
\newcommand{\lword}[1]{\leavevmode\nobreak\hskip0pt plus \linewidth\penalty50\hskip0pt plus-\linewidth\nobreak{#1}}    % Define command for handling long words or commands forcing line breaks if required. "lword" is short for long-word.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TNO OLYMPUS Field Development Optimisation Challenge New Commands %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Challenge Names %%%

\newcommand{\TNOChallenge}{TNO OLYMPUS Field Development Optimisation Challenge}    % Define the name of the TNO OLYMPUS Field Development Optimisation Challenge.
\newcommand{\TNOChallengeshort}{TNO OLYMPUS Challenge}    % Define a shortened name for the TNO OLYMPUS Field Development Optimisation Challenge.
\newcommand{\TNOChallengeWC}{TNO OLYMPUS Well Control Optimisation Challenge}    % Define the name of the TNO OLYMPUS Well ControlOptimisation Challenge.
\newcommand{\TNOChallengeWP}{TNO OLYMPUS Well Placement Optimisation Challenge}    % Define the name of the TNO OLYMPUS Well Placement Optimisation Challenge.
\newcommand{\TNOChallengeJFDWC}{TNO OLYMPUS Joint Field Development and Well Placement Optimisation Challenge}    % Define the name of the TNO OLYMPUS Joint Field Development and Well Control Optimisation Challenge.

\newcommand{\OLYMPUSWorkshop}{EAGE/TNO Workshop on OLYMPUS Field Development Optimization}    % Define the name of the EAGE/TNO Workshop on OLYMPUS Field Development Optimization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands for formatting the name of decision parameters in text.
% Note that "vm" at the end of the name denotes the ability to vary the month as well.
\newcommand{\decparvm}[4]{\lword{{#1}\_{#2}\_{#3}\_{#4}}}    % Define decision parameter with four arguments: well type, well number, year and month of control, for use in text.
\newcommand{\prodparvm}[3]{\decparvm{prod}{#1}{#2}{#3}}    % Define the target production rate parameter with three arguments: production well number and year of control, for use in text.
\newcommand{\injparvm}[3]{\decparvm{inj}{#1}{#2}{#3}}    % Define the target injection rate parameter with three arguments: injector well number, year and month of control, for use in text.

\newcommand{\decpar}[3]{\decparvm{#1}{#2}{#3}{01}}    % Define decision parameter with three arguments: well type, well number, year of control, for use in text. The month is fixed as January (01).
\newcommand{\prodpar}[2]{\decpar{prod}{#1}{#2}}    % Define the target production rate parameter with two arguments: production well number and year of control, for use in text.
\newcommand{\injpar}[2]{\decpar{inj}{#1}{#2}}    % Define the target injection rate parameter with two arguments: injector well number and year of control, for use in text.

% Commands for formatting the name of simulator output in text.
\newcommand{\simout}[3]{\lword{{#1}{#2}\_{#3}}}    % Define the simulator output with three arguments: property type, well type and number, and date in the format YYYYMMDD.

\newcommand{\WOPTPRODtwofirst}{\simout{WOPT}{PROD2}{20180101}}    % Define the WOPT for producer well 2 in the first control interval beginning January 1, 2016 and ending January 1, 2018.
\newcommand{\WOPTPRODtenfirst}{\simout{WOPT}{PROD10}{20180101}}    % Define the WOPT for producer well 10 in the first control interval beginning January 1, 2016 and ending January 1, 2018.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Design for Simulations %%%

%%% Parameter Difference Constraints %%%
\newcommand{\pardiff}{\delta}    % Define the (scaled) difference between two time consecutive parameters.
\newcommand{\pardiffi}{\pardiff_i}    % Define the (scaled)difference between the i-th and (i-1)-th parameters.

\newcommand{\pardiffvec}{\boldsymbol{\pardiff}}    % Define a vector of (scaled) differences between time consecutive parameters.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Change Points %%%

\newcommand{\dcp}{d_{jk,t_i}}    % Define the general individual decision parameter for change points and extrapolation cut-offs of an output with respect to this target rate.

\newcommand{\cp}[2]{c_{#1,#2}}    % Define the change point of an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\cpp}[2]{\cp{P#1}{#2}}    % Define the change point of an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\cpi}[2]{\cp{I#1}{#2}}    % Define the change point of an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

\newcommand{\cpl}[2]{c_{#1,#2}^l}    % Define the change point lower bound of an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\cppl}[2]{\cpl{P#1}{#2}}    % Define the change point lower bound of an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\cpil}[2]{\cpl{I#1}{#2}}    % Define the change point lower bound of an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

\newcommand{\cpu}[2]{c_{#1,#2}^u}    % Define the change point upper bound of an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\cppu}[2]{\cpu{P#1}{#2}}    % Define the change point upper bound of an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\cpiu}[2]{\cpu{I#1}{#2}}    % Define the change point upper bound of an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Extrapolation Cut-Offs %%%

\newcommand{\extrapco}[2]{b_{#1,#2}}    % Define the extrapolation cut-off of an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\extrapcop}[2]{\extrapco{P#1}{#2}}    % Define the extrapolation cut-off of an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\extrapcoi}[2]{\extrapco{I#1}{#2}}    % Define the extrapolation cut-off of an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

\newcommand{\extrapcocpl}[2]{b_{#1,#2}^{cp^l}}    % Define the extrapolation cut-off as the change point lower bound for an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\extrapcopcpl}[2]{\extrapcocpl{P#1}{#2}}    % Define the extrapolation cut-off as the change point lower bound for an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\extrapcoicpl}[2]{\extrapcocpl{I#1}{#2}}    % Define the extrapolation cut-off as the change point lower bound for an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

\newcommand{\extrapcominos}[2]{b_{#1,#2}^{\text{min}}}    % Define the extrapolation cut-off based on the minimum off-slope data for an output with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\extrapcopminos}[2]{\extrapcominos{P#1}{#2}}    % Define the extrapolation cut-off based on the minimum off-slope data for an output with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\extrapcoiminos}[2]{\extrapcominos{I#1}{#2}}    % Define the extrapolation cut-off based on the minimum off-slope data for an output with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

\newcommand{\extrapcoCIlwr}[2]{b_{#1,#2}^{\text{CI}}}    % Define the extrapolation cut-off based on the credible interval (CI) lower bound for data exceeding the change point with respect to a target rate. The two arguments are: the well number and the control interval starting year respectively.
\newcommand{\extrapcopCIlwr}[2]{\extrapcoCIlwr{p#1}{#2}}    % Define the extrapolation cut-off based on the credible interval (CI) lower bound for data exceeding the change point with respect to a target production rate. The two arguments are: the producer well number and the control interval starting year respectively.
\newcommand{\extrapcoiCIlwr}[2]{\extrapcoCIlwr{i#1}{#2}}    % Define the extrapolation cut-off based on the credible interval (CI) lower bound for data exceeding the change point with respect to a target injection rate. The two arguments are: the injector well number and the control interval starting year respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% NPV %%%

\newcommand{\NPV}{\mathrm{NPV}}    % Symbol for NPV for use in equations.
\newcommand{\NPVd}{\NPV(\boldd)}    % Symbol for NPV evaluated at decision parameter vector, \boldd, for use in equations.
\newcommand{\NPVj}{\NPV_j}    % Symbol for NPV for the j-th ensemble member for use in equations.
\newcommand{\NPVjd}{\NPV_j(\boldd)}    % Symbol for NPV for the j-th ensemble member evaluated at decision parameter vector, \boldd, for use in equations.

\newcommand{\approxNPV}{\widetilde{\NPV}}    % Symbol for the approximate NPV for use in equations.
\newcommand{\approxNPVd}{\approxNPV(\boldd)}    % Symbol for the approximate NPV evaluated at decision parameter vector, \boldd, for use in equations.
\newcommand{\approxNPVj}{\approxNPV_j}    % Symbol for the approximate NPV for the j-th ensemble member for use in equations.
\newcommand{\approxNPVjd}{\approxNPV_j(\boldd)}    % Symbol for the approximate NPV for the j-th ensemble member evaluated at decision parameter vector, \boldd, for use in equations.

\newcommand{\ENPV}{\E[\NPV]}    % Symbol for expected NPV for use in equations.
\newcommand{\ENPVd}{\ENPV(\boldd)}    % Symbol for expected NPV evaluated at decision parameter vector, \boldd, for use in equations.

\newcommand{\meanNPV}{\overline{\NPV}}    % Symbol for the ensemble mean NPV as an approximation to the expected NPV for use in equations.
\newcommand{\meanNPVd}{\meanNPV(\boldd)}    % Symbol for the ensemble mean NPV as an approximation to the expected NPV evaluted at decision parameter vector, \boldd, for use in equations.

\newcommand{\CWGNPV}{CWG NPV}    % Define the CWG NPV for use in text.
\newcommand{\ECWGNPV}{expected CWG NPV}    % Define the expected CWG NPV for use in text.
\newcommand{\meanCWGNPV}{ensemble mean \CWGNPV}    % Define the ensemble mean CWG NPV as an approximation to the expected CWG NPV for use in text.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Commands for Bayesian Emulators %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Typesetting of probabilistic quantities %%%

% The following commands are for the typesetting of probability, expectation, variance, covariance and standard deviation as operators.
\DeclareMathOperator{\Prob}{\mathbb{P}}    % Command for probability.
\DeclareMathOperator{\E}{\mathbb{E}}    % Command for expectation.
\DeclareMathOperator{\Var}{\mathrm{Var}}    % Command for variance.
\DeclareMathOperator{\Cov}{\mathrm{Cov}}    %Command for covariance.
\DeclareMathOperator{\sd}{\mathrm{sd}}    % Command for the standard deviation.

% Previous commands for the typesetting of probability, expectation, variance, covariance and standard deviation.
%\newcommand{\Prob}{\mathbb{P}}    % Command for probability.
%\newcommand{\E}{\mathbb{E}}    % Command for expectation.
%\newcommand{\Var}{\mathrm{Var}}    % Command for variance.
%\newcommand{\Cov}{\mathrm{Cov}}    %Command for covariance.
%\newcommand{\sd}{\mathrm{sd}}    % Command for the standard deviation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Simulator Input %%%

\newcommand{\boldx}{\mathbf{x}}    % Define a vector of model parameters, x.
\newcommand{\boldxprime}{\boldx^\prime}    % Define a vector of model parameters, x^\prime.
\newcommand{\boldxO}{\boldx_0}    % Define a vector of model parameters, x_0.
%\newcommand{\xspace}{\mathcal{X}}    % Define a symbol for the model parameter space.

\newcommand{\boldd}{\mathbf{d}}    % Define a vector of decision parameters, d.
\newcommand{\bolddprime}{\boldd^\prime}    % Define a vector of decision parameters, d^\prime.
\newcommand{\dspace}{\Omega}    % Define a symbol for the decision parameter space.

\newcommand{\djkti}{d_{jk, t_i}}    % Define the decision parameter for well type j, well number k, at time t_i.
\newcommand{\djktiminusone}{d_{jk, t_i - 1}}    % Define the decision parameter for well type j, well number k, at time t_i - 1.

\newcommand{\Dprime}{D^\prime}    % Define the active input parameter space dimension, where D is used to denote the dimension fo the parameter space.

\newcommand{\Djk}{D^{(jk)}}    % Define the number of decision parameters in the subgroup for well type j and well number k.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Indicator functions for equality of inputs %%%

\newcommand{\indicator}[1]{\mathbbm{1}_{ \left\{ #1 \right\} }}    % Define an indicator function.

\newcommand{\indicatorequalij}{\indicator{ i = j }}    % Define an indicator function for use in maths mode for the equality of two indices, i and j.

\newcommand{\indicatorequalboldx}{\indicator{ \boldx = \boldxprime }}    % Define an indicator function for use in maths mode for the equality of two vectors of model parameters, x and x^\prime.
\newcommand{\indicatorequalboldd}{\indicator{ \boldd = \bolddprime }}    % Define an indicator function for use in maths mode for the equality of two vectors of decision parameters, d and d^\prime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General System Output %%%

\newcommand{\boldy}{\mathbf{y}}    % Define a vector of system output, y.

\newcommand{\boldz}{\mathbf{z}}    % Define a vector of observations of the system, z.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Simulator Output %%%

\newcommand{\fx}{f(\boldx)}    % Define the output of a simulator or function for (model) parameter vector x.
\newcommand{\fxprime}{f(\boldxprime)}    % Define the output of a simulator or function for (model) parameter vector xprime.
\newcommand{\fd}{f(\boldd)}    % Define the output of a simulator or function for decision parameter vector d.
\newcommand{\fdprime}{f(\bolddprime)}    % Define the output of a simulator or function for decision parameter vector dprime.
\newcommand{\fxd}{f(\boldx, \boldd)}    % Define the output of a simulator or function for model parameter vector x and decision parameter vector d.
%\newcommand{\fx}{f(\mathbf{x})}    % Define the output of a simulator or function for (model) parameter vector x.
%\newcommand{\fd}{f(\mathbf{d})}    % Define the output of a simulator or function for decision parameter vector d.

\newcommand{\fix}{f_i(\boldx)}    % Define the i-th output of a simulator or function for (model) parameter vector x.
\newcommand{\fid}{f_i(\boldd)}    % Define the i-th output of a simulator or function for decision parameter vector d.
\newcommand{\fidprime}{f_i(\bolddprime)}    % Define the i-th output of a simulator or function for decision parameter vector dprime.
\newcommand{\fixd}{f_i(\boldx, \boldd)}    % Define the i-th output of a simulator or function for model parameter vector x and decision parameter vector d.
%\newcommand{\fix}{f_i(\mathbf{x})}    % Define the i-th output of a simulator or function for (model) parameter vector x.
%\newcommand{\fid}{f_i(\mathbf{d})}    % Define the i-th output of a simulator or function for decision parameter vector d.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Linear Model Output %%%

\newcommand{\fLMx}{\hat{f}_{\mathrm{LM}}(\boldx)}    % Define the output of a linear model for a simulator output for (model) parameter vector x.
\newcommand{\fLMd}{\hat{f}_{\mathrm{LM}}(\boldd)}    % Define the output of a linear model for a simulator output for decision parameter vector d.

\newcommand{\fiLMx}{\hat{f}_{i, \mathrm{LM}}(\boldx)}    % Define the output of a linear model for the i-th simulator output for (model) parameter vector x.
\newcommand{\fiLMd}{\hat{f}_{i, \mathrm{LM}}(\boldd)}    % Define the output of a linear model for the i-th simulator output. for decision parameter vector d.

\newcommand{\sigmaLM}{\sigma_{\mathrm{LM}}}    % Symbol for the standard deviation of a linear model used for the regression part of an emulator.
\newcommand{\sigmaLMsquared}{\sigmaLM^2}    % Symbol for the variance of a linear model used for the regression part of an emulator.
\newcommand{\sigmaLMi}{\sigma_{\mathrm{LM}_i}}    % Symbol for the standard deviation of a linear model used for the regression part of an emulator for the i-th simulator response.
\newcommand{\sigmaLMisquared}{\sigmaLMi^2}    % Symbol for the variance of a linear model used for the regression part of an emulator for the i-th simulator response.

\newcommand{\sigmahatLM}{\hat{\sigma}_{\mathrm{LM}}}    % Symbol for the estimated standard deviation of a linear model used for the regression part of an emulator.
\newcommand{\sigmahatLMsquared}{\sigmahatLM^2}    % Symbol for the estimated variance of a linear model used for the regression part of an emulator.
\newcommand{\sigmahatLMi}{\hat{\sigma}_{\mathrm{LM}_i}}    % Symbol for the estimated standard deviation of a linear model used for the regression part of an emulator for the i-th simulator response.
\newcommand{\sigmahatLMisquared}{\sigmahatLMi^2}    % Symbol for the estimated variance of a linear model used for the regression part of an emulator for the i-th simulator response.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Gaussian Process Emulation %%%

\newcommand{\GP}{\mathcal{GP}}    % Define the symbol for a Gaussian Process for use in equations.
\newcommand{\normdist}{\mathcal{N}}    % Define the symbol for a normal distributino for use in equations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Multivariate Gaussian Process Emulation %%%

\newcommand{\GPmv}[1]{\GP_{#1}}    % Define the symbol for a multivariate Gaussian Process emulator for use in equations.
\newcommand{\boldm}{\mathbf{m}}    % Define the symbol for multivariate (GP) emulator mean function for use in equations.
\newcommand{\boldg}{\mathbf{g}}    % Define the symbol for multivaraite (GP) emulator mean function vector of deterministic functions for use in equations.
\newcommand{\SigmaMV}{\Sigma_{\mathrm{MV}}}    % Define the symbol for multivaraite (GP) emulator covariance matrix between outputs for use in equations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Emulator Diagnostics %%%

\newcommand{\loo}{leave-one-out}    % Define a short command for formatting leave-one-out (diagnostics or cross-validation) for use in text.
\newcommand{\Loo}{Leave-one-out}    % Define a short command for formatting Leave-one-out (diagnostics or cross-validation) for use in text. Note that the first letter is capitalised.

\newcommand{\lko}{leave-$k$-out}    % Define a short command for formatting leave-k-out (diagnostics or cross-validation) for use in text.
\newcommand{\Lko}{Leave-$k$-out}    % Define a short command for formatting Leave-k-out (diagnostics or cross-validation) for use in text. Note that the first letter is capitalised.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Linear Regression Models %%%

\newcommand{\RSSI}{\mathrm{RSS}_{\mathcal{I}}}    % Symbol for the Residual Sum of Squares for a fitted linear model.

\newcommand{\adjRsq}{adjusted $R^2$}    % Define a command for the adjusted R squared value.
\newcommand{\AdjRsq}{Adjusted $R^2$}    % Define a command for the adjusted R squared value. Note that the first letter is capitalised.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Commands for Uncertainty Quantification %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Types of Uncertainty  %%%

%%% Model Discrepancy %%%
\newcommand{\mathMD}{\mathrm{MD}}    % Math roman letters for denoting model discrepancy.
\newcommand{\epsilonMD}{\varepsilon_{\mathMD}}    % Symbol for the model discrepancy.
\newcommand{\epsilonMDi}{\varepsilon_{\mathMD, i}}    % Symbol for the model discrepancy.
\newcommand{\mathMDint}{\mathrm{MD,int}}    % Math roman letters for denoting internal model discrepancy.
\newcommand{\epsilonMDint}{\varepsilon_{\mathMDint}}    % Symbol for internal model discrepancy.
\newcommand{\mathMDext}{\mathrm{MD,ext}}    % Math roman letters for denoting internal model discrepancy.
\newcommand{\epsilonMDext}{\varepsilon_{\mathMDext}}    % Symbol for internal model discrepancy.

%%% Geological (or Ensemble) Uncertainty %%%
\newcommand{\epsilonGeo}{\varepsilon_{\mathrm{G}}}    % Symbol for the geological uncertainty.

%%% Efficient Geological Ensemble Subsampling (EGES) Uncertainty %%%
\newcommand{\Ntilde}{\tilde{N}}    % Symbol for the number of models from the ensemble used.
\newcommand{\mathEGES}{\mathrm{ES}}    % Math roman letters for denoting Multi-Model Ensemble Subsampling (ES) uncertainty.
%\newcommand{\mathEGES}{\mathrm{MM}}    % Math roman letters for denoting Multi-Model Ensemble Subsampling (MM) uncertainty. Alternative to the above.
%\newcommand{\mathEGES}{\mathrm{EGES}}    % Math roman letters for denoting Efficient Geological Ensemble Subsampling (EGES) uncertainty. This is for the original application in my PhD thesis.
\newcommand{\epsilonEGES}{\varepsilon_{\mathEGES}}    % Symbol for the Efficient Geological Ensemble Subsampling (EGES) uncertainty.

%%% Utility Function or NPV Objective Function Cost Parameter Uncertainty %%%
\newcommand{\mathC}{\mathrm{C}}    % Math roman letters for denoting the utility function / NPV objective function cost parameter uncertainty.
\newcommand{\epsilonC}{\varepsilon_{\mathC}}    % Symbol for the utility function / NPV objective function cost parameter uncertainty.

%%% Decision Implementation Error %%%
\newcommand{\mathImplement}{\mathrm{I}}    % Math roman letters for denoting the decision implementation error.
\newcommand{\bolddeltaImplement}{\boldsymbol{\delta}_{\mathImplement}}    % Bold delta for the actually implemented decisions.
\newcommand{\bolddeltaImplementij}{\boldsymbol{\delta}_{i, j}}    % Bold delta for the simulated actually implemented decisions for the i-th individual decision parameter, and the j-th simulated implementation error.
\newcommand{\eImplement}{e_{\mathImplement}}    % Symbol for the decision implementation error on an individual decision parameter.
\newcommand{\eImplementi}{e_{\mathImplement, i}}    % Symbol for the decision implementation error on the i-th individual decision parameter.
\newcommand{\boldeImplement}{\bolde_{\mathImplement}}    % Symbol for the decision implementation error on the decisions themselves.
\newcommand{\epsilonImplement}{\varepsilon_{\mathImplement}}    % Symbol for the induced decision implementation error for the utility function / NPV objective function.

%%% Observational Errors %%%
\newcommand{\bolde}{\mathbf{e}}    % Symbol for a vector of observational errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Uncertainty Variance Matrices %%%

%%% Model Discrepancy %%%
\newcommand{\sigmaMD}{\sigma_{\mathMD}}    % Symbol for the model discrepancy univariate standard deviation.
\newcommand{\SigmaMD}{\Sigma_{\mathMD}}    % Symbol for the model discrepancy variance matrix.
\newcommand{\SigmaMDint}{\Sigma_{\mathMDint}}    % Symbol for the internal model discrepancy variance matrix.
\newcommand{\SigmaMDext}{\Sigma_{\mathMDext}}    % Symbol for the internal model discrepancy variance matrix.

%%% Observational Errors %%%
\newcommand{\Sigmae}{\Sigma_{e}}    % Symbol for the observational error variance matrix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% EGES Uncertainty %%%

\newcommand{\sigmaEGES}{\sigma_\mathEGES}    % Symbol for the EGES standard deviation.
\newcommand{\sigmahatEGES}{\hat{\sigma}_\mathEGES}    % Symbol for the estimated EGES standard deviation.

\newcommand{\betaEGES}{\boldbeta_\mathEGES}   % Symbol for a vector of EGES linear model regression coefficients.
\newcommand{\betahatEGES}{\hat{\boldbeta}_\mathEGES}   % Symbol for a vector of the estimated EGES linear model regression coefficients.

\newcommand{\XEGESd}{X_\mathEGES(\boldd)}    % Symbol for a vector of the constant intercept 1, and individual model NPV for the EGES members evaluated at a decision parameter vector, d.
\newcommand{\XEGESTd}{X_\mathEGES^\Transpose(\boldd)}    % Symbol for a transposed vector of the constant intercept 1, and individual model NPV for the EGES members evaluated at a decision parameter vector, d.

\newcommand{\SigmabetaEGES}{\Sigma_{\beta, \mathEGES}}    % Symbol for the covariance matrix for the EGES linear model regression coefficients.
%\newcommand{\SigmahatbetaEGES}{\hat{\Sigma}_{\beta, \mathEGES}}    % Symbol for the estimated covariance matrix for the EGES linear model regression coefficients.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Utility Function Cost Parameter Uncertainty %%%

\newcommand{\boldc}{\mathbf{c}}    % Define a vector of utility function / NPV objective function cost parameters, c.

\newcommand{\Udc}{U(\boldd,\boldc)}    % Symbol for the utility function evaluated at a decision parameter vector, \boldd, for an explicit cost parameter setting, \boldc.
\newcommand{\Ufxddc}{U(\fxd, \boldd, \boldc)}    % Symbol for the utility function evaluated at a decision parameter vector, \boldd, for cost parameter setting, \boldc, with an explicit dependence on the simulator evaluation for a particular model parameter vector, \boldx, and decision parameter vector, \boldd.

\newcommand{\Udci}{U(\boldd,\boldc_i)}    % Symbol for the utility function evaluated at a decision parameter vector, \boldd, for the i-th cost parameter setting, \boldc_i.
\newcommand{\Udjci}{U(\boldd_j,\boldc_i)}    % Symbol for the utility function evaluated at the j-th decision parameter vector, \boldd_j, for the i-th cost parameter setting, \boldc_i.

\newcommand{\Udcnought}{U(\boldd,\boldc_0)}    % Symbol for the utility function evaluated at a decision parameter vector, \boldd, for the (TNO) fixed reference cost parameter setting, \boldc_0.
\newcommand{\Udjcnought}{U(\boldd_j,\boldc_0)}    % Symbol for the utility function evaluated at the j-th decision parameter vector, \boldd_j, for the (TNO) fixed reference cost parameter setting, \boldc_0.

\newcommand{\epsilonCi}{\varepsilon_{\boldc_i}}    % Symbol for the uncertainty for the i-th cost parameter setting, \boldc_i.
\newcommand{\epsilonCid}{\epsilonCi(\boldd)}    % Symbol for the uncertainty for the i-th cost parameter setting, \boldc_i, with an explicit dependence on the decision parameter vector, \boldd.

\newcommand{\epsilonChatdci}{\hat{\varepsilon}_{\mathC}(\boldd, \boldc_i)}    % Symbol for the utility function / NPV objective function cost parameter uncertainty linear model residual for the decision parameter vector \boldd, evaluated at the i-th cost parameter setting, \boldc_i.
\newcommand{\epsilonChatdjci}{\hat{\varepsilon}_{\mathC}(\boldd_j, \boldc_i)}    % Symbol for the utility function / NPV objective function cost parameter uncertainty linear model residual for the j-th decision parameter vector \boldd_j, evaluated at the i-th cost parameter setting, \boldc_i.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Decision Implementation Error %%%

\newcommand{\sigmaeImplementi}{\sigma_{\eImplement, i}}    % Define a symbol for the standard deviation of the decision implementation error on the i-th individual decision parameter.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Commands for Iterative Decision Support %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Decision Support Utility Function %%%

\newcommand{\Ud}{U(\boldd)}    % Symbol for the utility function evaluated at a decision parameter vector, \boldd.
\newcommand{\EFUd}{\E_F[\Ud]}    % Symbol for the adjusted expectation of the utility function for decision parameter vector, \boldd.
\newcommand{\VarFUd}{\Var_F[\Ud]}    % Symbol for the adjusted variance of the utility function for decision parameter vector, \boldd.

\newcommand{\mathDS}{\mathrm{DS}}    % Math roman letters for denoting decision support.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Decision Support Implausibility Measures %%%

\newcommand{\IDS}{I_{\mathDS}}    % Define a command for the decision support implausibility measure.
\newcommand{\IDSd}{\IDS(\boldd)}    % Define a command for the decision support implausibility measure evaluated at a decision parameter vector, \boldd.
\newcommand{\Umax}{U_{\mathrm{max}}}    % Define a command for the current maximum simulated utility function.

\newcommand{\epsilonDS}{\varepsilon_{\mathDS}}    % Symbol for the collective decision support uncertainty.
\newcommand{\epsilonDSd}{\epsilonDS(\boldd)}    % Symbol for the collective decision support uncertainty evaluated at decision parameter vector, \boldd.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Math Mode Commands for the Derivation of the Bayes Linear Adjustment Formulae for Bayesian Emulators %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Math Mode Commands %%%

%%% Equation formatting %%%
\newcommand{\alignnumber}{\addtocounter{equation}{1}\tag{\theequation}}    % Add a number to a specified line(s) of an equation in the align* (or other maths environment).
\newcommand{\alignmultilineeq}{\\ &{} \phantom{=}\;}    % Split equation into multiline equation within the align environment.
%\newcommand{\alignmultilineeq}{\\ &{} \quad}    % Split equation into multiline equation within the align environment.    % This is the previous method of splitting an equation into multiple lines within the align environment. Note that the indentation is not as large as for the new version using "\phantom{=}\;".

%%% Mathematical Operators %%%
\DeclareMathOperator*{\argmax}{arg\,max}    % argmax operator.
\DeclareMathOperator*{\argmin}{arg\,min}    % argmin operator.
\DeclareMathOperator*{\mean}{mean}    % Mean operator.

%%% Mathematical Operators for Matrices %%%
\DeclareMathOperator{\Tr}{Tr}    % Trace of a matrix.
\DeclareMathOperator{\diag}{diag}    % Diagonal matrix.

\newcommand{\Transpose}{\mathrm{T}}    % Define a symbol for vector of matrix transpose.

%%% Function Derivatives and Variants %%%
\newcommand{\dprime}{{\prime\prime}}    % Double prime notation.
\newcommand{\trprime}{{\prime\prime\prime}}    % Triple prime notation.

%%% Independence Symbol %%%
\newcommand{\indep}{\perp \!\!\! \perp}    % Symbol for independence.

%%% Big O and Little O Notation %%%
\newcommand{\BigO}[1]{\mathcal{O}(#1)}    % Big O notation.
\newcommand{\LittleO}[1]{\mathcal{o}(#1)}    % Little O notation.

%%% Identity Matrix %%%
\newcommand{\Idmatrix}[1]{I_{#1}}    % Symbol for the identity matrix of a specified size.

%%% Zero Vector of Matrix %%%
\newcommand{\boldzero}{\mathbf{0}}    % Bold zero for representing a zero vector or matrix.

%%% Sign Operator %%%
\DeclareMathOperator{\sign}{sign}    % Define the sign operator.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Presentation of the Bayes Linear Adjustment Formulae %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Symbols for the Collections of Random Quantities %%%

\newcommand{\mathBL}{\mathrm{BL}}    % Symbol for Bayes Linear acronym for use in equations.

\newcommand{\boldB}{\mathbf{B}}    % Symbol for the collection of random quantities, B.
\newcommand{\boldC}{\mathbf{C}}    % Symbol for the collection of random quantities, C.
\newcommand{\boldD}{\mathbf{D}}    % Symbol for the collection of random quantities, D.

%%% Symbols for Bayes Linear Adjusted Expectations, Variances and Covariance for these Collections of Random Quantities %%%

\newcommand{\EDB}{\E_D[\boldB]}    % Symbol for the adjusted expectation of the collection of random quantities, \boldB, given observations, \boldD.
\newcommand{\VarDB}{\Var_D[\boldB]}    % Symbol for the adjusted variance of the collection of random quantities, \boldB, given observations, \boldD.
\newcommand{\CovDBC}{\Cov_D[\boldB,\boldC]}    % Symbol for the adjusted covariance between the collections of random quantities, \boldB and \boldC, given observations, \boldD.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General Presentation for a Full Bayesian Update %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Symbols for the Collections of Random Quantities %%%

\newcommand{\boldtheta}{\boldsymbol{\theta}}    % Symbol for the collection of random quantities / variables, \theta.

%%% Notation for the Likelihood %%%

\newcommand{\Dgiventhetalikeli}{\pi(\boldD \mid \boldtheta)}    % Notation for the likelihood of observed data, \boldD, given a collection of random quantities, \boldtheta.

%%% Notation for the Full Bayesian Prior Probability Distribution %%%

\newcommand{\thetapriordist}{\pi(\boldtheta)}    % Notation for the full Bayesian prior distribution of the collection of random quantities, \boldtheta.
\newcommand{\Dpriordist}{\pi(\boldD)}    % Notation for the full Bayesian prior probability of the data, \boldD, obtained via either a summation or integral over the random quantities, \boldtheta, of interest.

%%% Notation for the Full Bayesian Posterior Probability Distribution %%%

\newcommand{\thetaposteriordist}{\pi(\boldtheta \mid \boldD)}    % Notation for the full Bayesian posterior distribution of the collection of random quantities, \boldtheta, given data, \boldD.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Symbols, Equations & Expressions %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Emulator Form %%%

\newcommand{\boldbeta}{\boldsymbol{\beta}}    % Symbol for a vector of regression coefficients for use in equations.

%%% Previously used commands for the weakly stationary stochastic process term within an emulator %%%
%\newcommand{\epsx}{\varepsilon(x)}    % Symbol for the weakly stationary stochastic process for a parameter input vector x.    % This is under the formulation used in my report on the Bayes linear adjustment formulae.
%\newcommand{\boldepsilon}{\boldsymbol{\varepsilon}}    % Symbol for the realisations of the weakly stationary stochastic process at the inputs of the simulator evaluations.    % This is under the formulation used in my report on the Bayes linear adjustment formulae.

\newcommand{\ux}{u(\boldx)}    % Symbol for the weakly stationary stochastic process for a parameter input vector x.
\newcommand{\uxprime}{u(\boldxprime)}    % Symbol for the weakly stationary stochastic process for a parameter input vector x^\prime.
\newcommand{\boldu}{\mathbf{u}}    % Symbol for the realisations of the weakly stationary stochastic process at the inputs of the simulator evaluations.

\newcommand{\wx}{w(\boldx)}    % Symbol for the nugget term process for a parameter input vector x.
\newcommand{\wxprime}{w(\boldxprime)}    % Symbol for the nugget term process for a parameter input vector x^\prime.
%\newcommand{\boldw}{\boldsymbol{w}}    % Symbol for the realisations of the residual process at the inputs of the simulator evaluations. Note: This is defined above as a general orthonormal w-basis vector for use in embedding a 2-dimensional input parameter space in 3-dimensions for use in emulation of computer model output with structured discontinuities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Prior Specification %%%

\newcommand{\Efx}{\E[\fx]}    % Symbol for the prior expectation of a function in terms of a vector of model parameters, boldx.
\newcommand{\Varfx}{\Var[\fx]}    % Symbol for the prior expectation of a function in terms of a vector of model parameters, boldx.

\newcommand{\Sigmainput}{M}    % Symbol for the prior covariance matrix between the input parameters.
\newcommand{\Sigmainputinv}{M^{-1}}    % Symbol for the inverse of the prior covariance matrix between the input parameters.

\newcommand{\mubeta}{\boldsymbol{\mu}_{\beta}}    % Symbol for the prior expectation of the regression coefficients.
\newcommand{\mubetai}{\boldsymbol{\mu}_{\beta_i}}    % Symbol for the prior expectation of the regression coefficients for the i-th computer model output.
\newcommand{\mubetaBL}{\boldsymbol{\mu}_{\mathBL, \beta}}    % Symbol for the prior expectation of the regression coefficients in Bayes linear emulation.
\newcommand{\Varbeta}{\Var[\boldbeta]}    % Symbol for the prior variance of the regression coefficients.
\newcommand{\Sigmabeta}{\Sigma_{\beta}}    % Symbol for the prior variance matrix of the regression coefficients.
\newcommand{\Sigmabetainv}{\Sigmabeta^{-1}}    % Symbol for the prior precision (inverse variance) matrix of the regression coefficients

\newcommand{\boldrx}{\mathbf{r}(\boldx, X)}    % Symbol for the correlation column vector between new input x and design points in X.
\newcommand{\boldrtransposex}{\mathbf{r}^\Transpose(\boldx, X)}    % Symbol for the correlation row vector between new input x and design points in X.
\newcommand{\Sigmainv}{\Sigma^{-1}}    % Symbol for the prior precision (inverse variance) matrix of the weakly stationary stochastic process within an emulator.
%\newcommand{\Covbetaepsilonzero}[1][ ]{$\Cov[\boldbeta, \boldepsilon] = \boldzero$#1}    % Equation giving the prior assumption of the zero prior covariance between the unknown regression coefficients and the realisations of the stochastic process part of the emulator. For inline equation use only with optional argument, default is " ".    % This is under the formulation used in my report on the Bayes linear adjustment formulae.
\newcommand{\Covbetauzero}[1][ ]{$\Cov[\boldbeta, \boldu] = \boldzero$#1}    % Equation giving the prior assumption of the zero prior covariance between the unknown regression coefficients and the realisations of the stochastic process part of the emulator. For inline equation use only with optional argument, default is " ".
 \newcommand{\VarFeq}{G \Sigmabeta G^\Transpose + \Sigma}    % Equation of the prior variance of simulator data F.
 \newcommand{\VarFeqinv}{(\VarFeq)^{-1}}    % Equation for the inverse of the prior variance (precision) of the simulator data F.

\newcommand{\zeromatrix}[2]{0_{#1, #2}}    % Symbol for a general matrix of zeroes where the number of rows are given by the first two dimensions respectively.
\newcommand{\zerosqmatrix}[1]{\zeromatrix{#1}{#1}}    % Symbol for a square zero matrix of the dimensions given by the argument.
\newcommand{\Sigmabetaeqzero}[1]{\Sigmabeta = \zerosqmatrix{#1}}    % Symbol for assigning the prior variance matrix for the regression coefficients to be a zero matrix of dimensions given by the argument.

\newcommand{\sigmau}{\sigma_u}    % Symbol for the standard deviation of the stochastic process of an emulator.
\newcommand{\sigmausquared}{\sigmau^2}        % Symbol for the variance of the stochastic process of an emulator.
\newcommand{\sigmaui}{\sigma_{u_i}}    % Symbol for the standard deviation of the stochastic process of an emulator for the i-th simulator response.
\newcommand{\sigmauisquared}{\sigmaui^2}    % Symbol for the variance of the stochastic process of an emulator for the i-th simulator response.

\newcommand{\sigmawsquared}{\sigma_{w}^2}    % Symbol for the variance of the nugget term / residual process of an emulator with a nugget term.
\newcommand{\Sigmaw}{\sigmawsquared \Idmatrix{n}}    % Symbol for the variance matrix of the nugget term / residual process of an emulator with a nugget term.

\newcommand{\Covbetawzero}[1][ ]{$\Cov[\boldbeta, \boldw] = \boldzero$#1}    % Equation giving the prior assumption of the zero prior covariance between the unknown regression coefficients and the realisations of the residual process part of the emulator. For inline equation use only with optional argument, default is " ".
%\newcommand{\Covepsilonwzero}[1][ ]{$\Cov[\boldepsilon, \boldw] = \boldzero$#1}    % Equation giving the prior assumption of the zero prior covariance between the realisations of the stochastic process and the realisations of the residual process part of the emulator. For inline equation use only with optional argument, default is " ".    % This is under the formulation used in my report on the Bayes linear adjustment formulae.
\newcommand{\Covuwzero}[1][ ]{$\Cov[\boldu, \boldw] = \boldzero$#1}    % Equation giving the prior assumption of the zero prior covariance between the realisations of the stochastic process and the realisations of the residual process part of the emulator. For inline equation use only with optional argument, default is " ".
\newcommand{\VarFeqwithnuggetfull}{\VarFeq + \Sigmaw}    % Equation for the prior variance of the simulator data F when using an emulator structure with a nugget term. Note that this is the full version without the notational simplificaiton.
\newcommand{\VarFeqwithnuggetfullinv}{(\VarFeqwithnuggetfull)^{-1}}    % Equation for the inverse of the prior variance of the simulator data F when using an emulator structure with a nugget term. Note that this is the full version without the notational simplificaiton.

%\newcommand{\VarFeqwithnuggetseqfit}{\Sigma + \Sigmaw}    % Equation for the prior variance of the simulator data F when using an emulator structure with a nugget term and the prior variance for the regression coefficients is set to zero.
%\newcommand{\VarFeqwithnuggetseqfitinv}{(\Sigma + \Sigmaw)^{-1}}    % Equation for the inverse of the prior variance of the simulator data F when using an emulator structure with a nugget term and the prior variance for the regression coefficients is set to zero.

\newcommand{\SigmaplusSigmaw}{\Omega}    % Short notation for the sum of the variance of the weakly stationary stochastic process and nugget term for the initial set of simulations.
\newcommand{\SigmaplusSigmawinv}{\SigmaplusSigmaw^{-1}}    % Short notation for the inverse of the sum of the variance of the weakly stationary stochastic process and nugget term for the initial set of simulations.
\newcommand{\SigmaplusSigmawfull}{\Sigma + \Sigmaw}    % Equation for the sum of the variance of the weakly stationary stochastic process and nugget term for the initial set of simulations. Note that this is the full version without the notational simplificaiton.
\newcommand{\SigmaplusSigmawfullinv}{(\SigmaplusSigmawfull)^{-1}}    % Equation for the inverse of the sum of the variance of the weakly stationary stochastic process and nugget term for the initial set of simulations. Note that this is the full version without the notational simplificaiton.

\newcommand{\VarFeqwithnugget}{G \Sigmabeta G^\Transpose + \SigmaplusSigmaw}    % Short notation for the equation for the prior variance of the simulator data F when using an emulator structure with a nugget term.
\newcommand{\VarFeqwithnuggetinv}{(\VarFeqwithnugget)^{-1}}    % Short notation for the equation for the inverse of the prior variance of the simulator data F when using an emulator structure with a nugget term.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Adjusted Emulator Quantities %%%

\newcommand{\boldF}{\mathbf{F}}    % Symbol for a vector of function / computer model / simulator evaluations.
\newcommand{\boldFi}{\boldF_i}    % Symbol for a vector of the univaraiate i-th function / computer model / simulator evaluations.
\newcommand{\boldFj}{\boldF_j}    % Symbol for a vector of the univaraiate j-th function / computer model / simulator evaluations.

%%% Symbols %%%
% The following commands are for the correct type-setting of probability, expectation, variance, covariance and standard deviation.
%\newcommand{\Prob}{\mathbb{P}}    % Symbol for probability in equations.
%\newcommand{\E}{\mathbb{E}}    % Symbol for expectation in equations.
%\newcommand{{\mathrm{Var}}    % Symbol for variance in equations.
%\newcommand{\Cov}{\mathrm{Cov}}    % Symbol for covariance in equations.
%\newcommand{\sd}{\mathrm{sd}}    % Symbol for the standard deviation in equations.

\newcommand{\EFfx}{\E_F[\fx]}    % Symbol for the adjusted expectation of the emulator of the form without a nugget term.
\newcommand{\EFfd}{\E_F[\fd]}    % Symbol for the adjusted expectation of the emulator for decision parameters, d.
\newcommand{\VarFfx}{\Var_F[\fx]}    % Symbol for the adjusted variance of the emulator of the form without a nugget term.
\newcommand{\VarFfd}{\Var_F[\fd]}    % Symbol for the adjusted variance of the emulator for decision parameters, d.

\newcommand{\EFifd}{\E_{\boldFi}[ \fid ]}    % Symbol for the adjusted expectation of the emulator for the i-th computer model for decision parameters, d.
\newcommand{\VarFifd}{\Var_{\boldFi}[ \fid ]}    % Symbol for the adjusted variance of the emulator for the i-th computer model for decision parameters, d.
\newcommand{\CovFifdfdprime}{\Cov_{\boldFi}[ \fid, \fidprime ]}    % Symbol for the adjusted covariance of the emulator for the i-th computer model at decision parameters, d and dprime.

\newcommand{\EFbeta}{\E_F[\boldbeta]}    % Symbol for the adjusted expectation of the regression coefficients.
\newcommand{\VarFbeta}{\Var_F[\boldbeta]}    % Symbol for the adjusted variance of the regression coefficients.

\newcommand{\EFux}{\E_F[\ux]}    % Symbol for the adjusted expectation of the weakly stationary stochastic process.
\newcommand{\VarFux}{\Var_F[\ux]}    % Symbol for the adjusted variance of the weakly stationary stochastic process.
\newcommand{\CovFbetaux}{\Cov_F[\boldbeta, \ux]}    % Symbol for the adjusted covariance between \beta and the weakly stationary stochastic process.
%%% Previously used commands for the weakly stationary stochastic process term within an emulator %%%
%\newcommand{\EFepsilonx}{\E_F[\epsx]}    % Symbol for the adjusted expectation of the weakly stationary stochastic process.
%\newcommand{\VarFepsilonx}{\Var_F[\epsx]}    % Symbol for the adjusted variance of the weakly stationary stochastic process.
%\newcommand{\CovFbetaepsilonx}{\Cov_F[\boldbeta, \epsx]}    % Symbol for the adjusted covariance between \beta and the weakly stationary stochastic process.

\newcommand{\EFwx}{\E_F[\wx]}    % Symbol for the adjusted expectation of the residual process.
\newcommand{\VarFwx}{\Var_F[\wx]}    % Symbol for the adjusted variance of the residual process.
\newcommand{\CovFbetawx}{\Cov_F[\boldbeta, \wx]}    % Symbol for the adjusted covariance between \beta and the residual process.
\newcommand{\CovFuwx}{\Cov_F[\ux, \wx]}    % Symbol for the adjusted covariance between the weakly stationary stochastic process term and the residual process.
%%% Previously used commands for the weakly stationary stochastic process term within an emulator %%%
%\newcommand{\CovFepsilonwx}{\Cov_F[\epsx, \wx]}    % Symbol for the adjusted covariance between the weakly stationary stochastic process term and the residual process.


%%% Expressions %%%
\newcommand{\adjVarbetaeq}{(G^\Transpose \Sigma^{-1} G + \Sigmabeta^{-1})^{-1}}    % Equation for the adjusted variance of beta.
\newcommand{\adjVarbetaeqwithnugget}{(G^\Transpose \SigmaplusSigmawinv G + \Sigmabetainv)^{-1}}    % Short notation for the equation for the adjusted variance of beta when using an emulator with a nugget term. 
\newcommand{\adjVarbetaeqwithnuggetfull}{(G^\Transpose (\Sigma + \Sigmaw)^{-1} G + \Sigmabetainv)^{-1}}    % Equation for the adjusted variance of beta when using an emulator with a nugget term.  Note that this is the full version without the notational simplificaiton.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Limiting Results %%%

\newcommand{\betahatols}{\hat{\boldbeta}_{OLS}}    % Symbol: \hat{\beta}_{OLS}.

\newcommand{\Varbetalimit}{\Var[\boldbeta] \rightarrow \infty}    % Limit statement as the prior variance of the regression coefficients tends towards infinity.
\newcommand{\betahatgls}{\hat{\boldbeta}_{GLS}}    % Symbol: \hat{\beta}_{GLS}.
\newcommand{\Varbetahatglssymb}{\Var\left[ \betahatgls \right]}    % Symbol: \Var[\betahatgls].

\newcommand{\betahatglseq}{(G^\Transpose \Sigmainv G)^{-1} G^\Transpose \Sigmainv \boldF}    % Formula for the \hat{\beta}_{GLS} estimate.
\newcommand{\Varbetahatgls}{(G^\Transpose \Sigmainv G)^{-1}}    % Formula for the variance of the \hat{\beta}_{GLS} estimate. This is also the limit as the prior variance of the regression coefficients tends towards infinity.

\newcommand{\betahatglseqmod}{(G^\Transpose \SigmaplusSigmawinv G)^{-1} G^\Transpose \SigmaplusSigmawinv \boldF}    % Formula for the \hat{\beta}_{GLS} estimate using a modified form of the resiual process variance matrix.
\newcommand{\Varbetahatglsmod}{(G^\Transpose \SigmaplusSigmawinv G)^{-1}}    % Formula for the variance of the \hat{\beta}_{GLS} estimate using a modified form of the resiual process variance matrix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bayesian Emulation Methodology for Computer Models with Structured Partial Discontinuities %%%
%%% Application to the TNO OLYMPUS Well Placement Optimisation Challenge %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Embedding the input parameter space in higher dimensions %%%

\newcommand{\boldv}{\mathbf{v}}    % Define a general embedding function for input parameters in higher dimensions.
\newcommand{\boldvofx}{\boldv(\boldx)}    % Define a general embedding function evaluated at a general input parameter vector \boldx to transform it into higher dimensions.
\newcommand{\boldvofxprime}{\boldv(\boldxprime)}    % Define a general embedding function evaluated at a general input parameter vector \boldxprime to transform it into higher dimensions.
\newcommand{\boldvofxO}{\boldv(\boldxO)}    % Define a general embedding function evaluated at the specific input parameter vector \boldxO to transform it into higher dimensions.

\newcommand{\vofxy}{v(x, y)}    % Define the general vector embedding function from 2D to 3D in terms of general (x, y).
\newcommand{\vofxOyO}{v(x_0, y_0)}    % Define the general vector embedding function from 2D to 3D evaluated at (x_0, y_0).

\newcommand{\vofboldx}{v(\boldx)}    % Define a general scalar embedding function from 2D to 3D in terms of general \boldx.
\newcommand{\vofboldxO}{v(\boldxO)}    % Define a general scalar embedding function from 2D to 3D evaluated at \boldxO.

\newcommand{\Vspace}{\mathcal{V}}    % Define a symbol for the embedding parameter space.

\newcommand{\partialdvx}{v_x}    % Define the partial derivative of the scalar embedding function from 2D to 3D with respect to the first argument, x.
\newcommand{\partialdvy}{v_y}    % Define the partial derivative of the scalar embedding function from 2D to 3D with respect to the second argument, y.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Simulator or Function Outputs %%%

\newcommand{\fxy}{f(x, y)}    % Define the output of a simulator or function for parameters (x, y).
\newcommand{\fxO}{f(\boldxO)}    % Define the output of a simulator or function for the parameter vector \boldxO.
\newcommand{\fxOyO}{f(x_0, y_0)}    % Define the output of a simulator or function for parameters (x_0, y_0).

\newcommand{\fboldvofx}{f(\boldvofx)}    % Define the output of a simulator or function with parameters embedded in higher dimensions \boldvofx.
\newcommand{\fboldvofxprime}{f(\boldvofxprime)}    % Define the output of a simulator or function with parameters embedded in higher dimensions \boldvofxprime.
\newcommand{\fboldvofxO}{f(\boldvofxO)}    % Define the output of a simulator of function with parameters embedded in higher dimensions \boldvofxO.

\newcommand{\uxy}{u(x,y)}    % Symbol for the weakly stationary stochastic process for a parameter input (x, y).
\newcommand{\uboldvofx}{u(\boldvofx)}    % Symbol for the weakly stationary stochastic process for an embedded parameter input \boldvofx.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Adjusted Emulator Quantities %%%

%\newcommand{\boldD}{\mathbf{D}}    % Symbol for a vector of function / computer model / simulator evaluations. Note that this is already defined above as a collection of random quantities, D.
\newcommand{\boldDi}{\boldD_i}    % Symbol for a vector of the univaraiate i-th function / computer model / simulator evaluations.

\newcommand{\EDfx}{\E_D[\fx]}    % Symbol for the adjusted expectation of the emulators for the parameter vector \boldx.
\newcommand{\EDfxy}{\E_D[\fxy]}    % Symbol for the adjusted expectation of the emulator for parameters (x, y).
\newcommand{\EDfboldvofx}{\E_D[\fboldvofx]}    % Symbol for the adjusted expectation of the emulator embedded in higher dimensions for embedded parameters, \boldvofx.

\newcommand{\VarDfx}{\Var_D[\fx]}    % Symbol for the adjusted variance of the emulator for the parameter vector \boldx.
\newcommand{\VarDfxy}{\Var_D[\fxy]}    % Symbol for the adjusted variance of the emulator for parameters (x, y).
\newcommand{\VarDfboldvofx}{\Var_D[\fboldvofx]}    % Symbol for the adjusted variance of the emulator embedded in higher dimensions for the embedded parameters, \boldvofx.

\newcommand{\EDuxy}{\E_D[\uxy]}    % Symbol for the adjusted expectation of the weakly stationary stochastic process for parameters (x, y).
\newcommand{\EDuboldvofx}{\E_D[\uboldvofx]}    % Symbol for the adjusted expectation of the weakly stationary stochastic process for the emulator embedded in higher dimensions for the embedded parameters, \boldvofx.

\newcommand{\VarDuxy}{\Var_D[\uxy]}    % Symbol for the adjusted variance of the weakly stationary stochastic process for the parameters, (x, y).
\newcommand{\VarDu}{\Var_D[\uboldvofx]}    % Symbol for the adjusted variance of the weakly stationary stochastic process for the emulator embedded in higher dimensions for the embedded parameters, \boldvofx.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Covariance Matrices %%%

\newcommand{\SigmaND}[1]{\Sigma_{#1\mathrm{D}}}    % Define a command for an N-dimensional variance matrix with the option to specify the dimension, N. This is either the variance matrix for the induced original or higher-dimensional embedded input parameter space.
\newcommand{\SigmaTwoD}{\SigmaND{2}}    % Define the desired induced variance matrix for the original 2D input parameter space.
\newcommand{\SigmaThreeD}{\SigmaND{3}}    % Define the 3D variance matrix for the embedded input parameter space.

\newcommand{\SigmaThreeDx}{\SigmaThreeD(\boldx)}    % Define the 3D variance matrix for the embedded input parameter space evaluated for the parameter vector \boldx.
\newcommand{\SigmaThreeDxprime}{\SigmaThreeD(\boldxprime)}    % Define the 3D variance matrix for the embedded input parameter space evaluated for the parameter vector \boldxprime.
\newcommand{\SigmaThreeDxO}{\SigmaThreeD(\boldxO)}    % Define the 3D variance matrix for the embedded input parameter space evaluated for the parameter vector \boldxO.
\newcommand{\SigmaThreeDvx}{\SigmaThreeD(\boldvofx)}    % Define the 3D variance matrix for the embedded input parameter space evaluated for the parameter vector \boldvofx.
\newcommand{\SigmaThreeDvxprime}{\SigmaThreeD(\boldvofxprime)}    % Define the 3D variance matrix for the embedded input parameter space evaluated for the parameter vector \boldvofxprime.

\newcommand{\SigmaNDInv}[1]{\Sigma_{#1\mathrm{D}}^{-1}}    % Define a command for the inverse of an N-dimensional variance matrix with the option to specify the dimension, N. This is either the variance matrix for the induced original or higher-dimensional embedded input parameter space.
\newcommand{\SigmaTwoDInv}{\SigmaNDInv{2}}    % Define the inverse of the desired induced variance matrix for the original 2D input parameter space.
\newcommand{\SigmaThreeDInv}{\SigmaNDInv{3}}    % Define the inverse of the 3D variance matrix for the embedded input parameter space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Standard Basis  %%%

\newcommand{\boldex}{\bolde_x}    % Define the standard basis vector in the x-direction.
\newcommand{\boldey}{\bolde_y}    % Define the standard basis vector in the y-direction.
\newcommand{\boldez}{\bolde_z}    % Define the standard basis vector in the z-direction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Basis for the construction of the covariance matrix in the embedded space %%%

\newcommand{\boldw}{\mathbf{w}}    % Define a general orthonormal w-basis vector.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% For general SigmaTwoD working in a rotated and scaled 2D parameter space %%%

\newcommand{\boldt}{\mathbf{t}}    % Define a basis vector in the rotated 2D parameter space.
\newcommand{\boldh}{\mathbf{h}}    % Define a basis vector in the rotated and scaled 2D parameter space.

\newcommand{\boldp}{\mathbf{p}}    % Define a vector of model parameters in the t-basis, p.
\newcommand{\boldq}{\mathbf{q}}    % Define a vector of model parameters in the h-basis, q.
\newcommand{\vofq}{v(q_1, q_2)}    % Define the general vector embedding function from 2D to 3D in terms of the derived (q_1, q_2) parameters in the h-basis.
\newcommand{\vofboldq}{v(\boldq)}    % Define a general scalar embedding function from 2D to 3D in terms of the derived parameter vector \boldq in the h-basis.

\newcommand{\partialdvqone}{v_{q_1}}    % Define the partial derivative of the scalar embedding function from 2D to 3D with respect to the first argument in the h-basis, q_1.
\newcommand{\partialdvqtwo}{v_{q_2}}    % Define the partial derivative of the scalar embedding function from 2D to 3D with respect to the second argument in the h-basis, q_2.


\newcommand{\SigmaTwoDt}{\SigmaTwoD^\boldt}   % Define the desired induced variance matrix for the rotated 2D input parameter space.
\newcommand{\SigmaTwoDh}{\SigmaTwoD^\boldh}   % Define the desired induced variance matrix for the rotated and scaled 2D input parameter space.

\newcommand{\SigmaThreeDh}{\SigmaThreeD^\boldh}   % Define the 3D variance matrix for the embedded input parameter space using the rotated and scaled 2D input parameter space given by the h-basis.
\newcommand{\SigmaThreeDhInv}{\SigmaThreeD^{\boldh^{-1}}}   % Define the inverse of the 3D variance matrix for the embedded input parameter space using the rotated and scaled 2D input parameter space given by the h-basis.


\newcommand{\STwoD}{S_{2\mathrm{D}}}    % Define the scaling matrix in the 2D parameter space.
\newcommand{\RTwoD}{R_{2\mathrm{D}}}    % Define the rotation matrix in the 2D parameter space.

\newcommand{\STwoDInv}{\STwoD^{-1}}    % Define the inverse of the scaling matrix in the 2D parameter space.
\newcommand{\RTwoDInv}{\RTwoD^{-1}}    % Define the inverse of the rotation matrix in the 2D parameter space.

\newcommand{\SThreeD}{S_{3\mathrm{D}}}    % Define the scaling matrix in the 3D embedded parameter space.
\newcommand{\RThreeD}{R_{3\mathrm{D}}}    % Define the rotation matrix in the 3D embedded parameter space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TNO OLYMPUS Well Placement Optimisation Challenge %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% NPV Expressed as a Function of Well Location Parameter Vectors %%%

%%% Note %%%
% See the above definitions for the TNO OLYMPUS Well Control Optimisation Challenge.

\newcommand{\NPVx}{\NPV(\boldx)}    % Symbol for NPV evaluated at well location parameter vector, \boldx, for use in equations.
\newcommand{\NPVjx}{\NPV_j(\boldx)}    % Symbol for NPV for the j-th ensemble member evaluated at well location parameter vector, \boldx, for use in equations.

\newcommand{\approxNPVx}{\approxNPV(\boldx)}    % Symbol for the approximate NPV evaluated at well location parameter vector, \boldx, for use in equations.
\newcommand{\approxNPVjx}{\approxNPV_j(\boldx)}    % Symbol for the approximate NPV for the j-th ensemble member evaluated at well location parameter vector, \boldx, for use in equations.

\newcommand{\ENPVx}{\ENPV(\boldx)}    % Symbol for expected NPV evaluated at well location parameter vector, \boldx, for use in equations.

\newcommand{\meanNPVx}{\meanNPV(\boldx)}    % Symbol for the ensemble mean NPV as an approximation to the expected NPV evaluted at well location parameter vector, \boldx, for use in equations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Modified Decision Support Implausibility Measures for the TNO OLYMPUS Well Placement Optimisation Challenge %%%

\newcommand{\IDSalt}{I_{\mathrm{DS}}^\prime}    % Define a command for a modified form of the decision support implausibility measure which includes an extra tolerance parameter for how far from the maximum simulated value to search.
\newcommand{\IDSaltx}{\IDSalt(\boldx)}    % Define a command for the modified form of the decision support implausibility measure evaluated at a vector of well location parameters, \boldx.
\newcommand{\fplus}{f^+}    % Define a command for the current maximum simulated function.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Results/Bayes-Linear-Emulation-of-the-Expected-NPV.tex <==
\subsection{Bayes Linear Emulation of the Expected NPV} \label{subsec:Bayes-Linear-Emulation-of-the-Expected-NPV}
%\subsection{Bayes Linear Emulation of the Ensemble Mean NPV} \label{subsec:Bayes-Linear-Emulation-of-the-Expected-NPV}

Bayes linear emulation is directly applied to the expected NPV to explore the 32-dimensional wave 1 decision parameter space utilising the above design and linear model predictions for the ensemble mean NPV for training and validation. This serves as a comparison with our proposed hierarchical emulation approach in \cref{subsec:Emulator-Comparison}. Following the methodology summarised in \cref{sec:Bayesian-Emulation}, an emulator with a nugget term (see \cref{eq:Bayes-linear-emulator-structure-in-decision-parameters-univariate-output}) is employed with $\fd = \Ud = \ENPVd$. Investigations using linear modelling, stepwise selection with the AIC criterion, and with all parameters transformed onto $[-1, 1]$, as in \cite{2010:Vernon:Bayesian-Uncertainty-Analysis-Galaxy-Formation}, yields a subset of 12 active decision parameters and a suggested second-order polynomial mean function form:
\begin{align} \label{eq:Expected-NPV-Bayes-linear-emulator-active-variable-selection-linear-model}
	\ENPV(\boldd_{A_\mathBL}) = \beta_{0} + \sum_{d_i \in A_\mathBL} \{ \beta_{i, 1} d_i + \beta_{i, 2} d_i^2 \} + \varepsilon
\end{align}
The residual uncertainty is captured through $\varepsilon$ which possesses an estimate residual standard error $\sigma_{lm}$. The unknown regression coefficients are assumed to have prior expectation $\mubeta = \boldzero$ and an infinite prior uncertainty, with emulator updates exploiting limiting results as $\Varbetalimit$ for which formulae are presented in \cite[Sec.~2.4.5]{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty}.

For the residual process it is assumed that $\E[u(\boldd_{A_\mathBL})] = 0$ and $\E[w(\boldd)] = 0$ with a squared exponential covariance structure (\cref{eq:Squared-exponential-covariance-structure-long}) using a single common correlation length hyperparameter. Following the substitution approach for the hyperparameters: \lword{$\sigma_{u}^2 = (1 - \rho) \sigma_{lm}^2$} and $\sigma_{w}^2 = \rho \sigma_{lm}^2$ where $\rho = 0.05$; whilst the correlation length parameter is set to half of the parameter range, hence $\theta = 1$. These choices are validated via emulator diagnostics discussed below. Bayes linear emulator adjustment is performed using \cref{eq:Bayes-linear-emulator-adjusted-expectation,eq:Bayes-linear-emulator-adjusted-variance,eq:Bayes-linear-emulator-adjusted-covariance}.

\Loo{} diagnostics suggest that the emulator fits well across the decision space, as shown in \cref{fig:OLYMPUS-w1-BL-emulator-theta-0_5-LOO-diagnostics-plot-adj-exp-3-adj-sd-CI-vs-sim-NPV} of the adjusted expectation with an approximate 95\% credible interval of width 3 adjusted standard deviations (following Pukelsheim's 3-sigma rule \cite{1994:Pukelsheim:the-3-sigma-rule}) versus the expected NPV. 691 of the 702 (98.4\%) credible intervals contain the simulated expected NPV, as highlighted by the red dashed line representing equality. Moreover, if we instead employed a Gaussian process emulator, then the 95\% credible intervals contain 679 of the simulated expected NPVs; a 96.7\% coverage. It is noted that the few cases where these diagnostics are not satisfied tend to yield over-prediction. With a view to decision support this is less of a concern as these regions will not be incorrectly ruled out due to low expected NPVs, while iterative refinement enables more accurate emulation at later waves.% Other \loo{} diagnostics for the emulator residuals highlight no major issues or misspecification.
\begin{figure}[!t]
	\centering
	\includegraphics[page=1,width=\linewidth]{Results/Graphics/Bayes-Linear-Emulation-of-the-Expected-NPV/OLYMPUS-w1-active-prod-dec-par-emulator-ensemble-mean-CWG-NPV-theta-0_5-LOO-diagnostics-variable-prior-plots-std}
	\caption{Bayes linear emulator for the expected NPV \loo{} diagnostics plot showing the emulator adjusted expectations with 95\% 3 adjusted standard deviation credible interval error bars versus the simulated expected NPV. The red dashed line denotes equality of the emulator prediction and the simulator output.}
%	\caption[Bayes linear emulator for the expected NPV \loo{} diagnostic plot]{Bayes linear emulator for expected NPV \loo{} diagnostic plot of the emulator adjusted expectations with 3 adjusted standard deviation credible interval error bars versus the simulated expected NPV. The red dashed line denotes equality of the emulator prediction and the observed value.}
	\label{fig:OLYMPUS-w1-BL-emulator-theta-0_5-LOO-diagnostics-plot-adj-exp-3-adj-sd-CI-vs-sim-NPV}
\end{figure}



%%% Notes %%%
%See PhD Thesis Section 4.4.

==> Results/Design.tex <==
\subsection{Targeted Bayesian Design of Simulations} \label{subsec:Bayesian-Design.tex}

We employ a novel targeted Bayesian design method, based on that presented in \cite{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty} and \cite[Sec.~4.3]{2022:Owen:PhD-Thesis}, which is tailored to performing decision support through targeted sampling based on prior beliefs of experienced petroleum reservoir engineers regarding the location of optimal decision parameter settings, as well as imposing practical and physical constraints. Firstly, TNO stipulate operational range constraints to be $[ 0 , 900 ]$m\textsuperscript{3}/day and $[ 0, 1600 ]$m\textsuperscript{3}/day for production and injection rates respectively; leading to a 32-dimensional hypercube parameter space. Oil reservoir engineers deem large temporal variation in controls to be unphysical and poor practice, thus suggesting a difference constraint between time consecutive controls. The 32 decision inputs are therefore split into four independent subgroups by well with difference constraint $\lvert \djkti - \djktiminusone \rvert \leq \Delta_i, \ i = 2, \ldots, \Djk$, where $\Djk = 8$ is the number of control intervals for well $jk$. A conservative choice is that the maximum permitted change over a two year time interval is $\Delta_i = \frac{1}{3}$ of the operational range for the well type. Consequently the decision parameter space is no longer a hypercube with a volume of 3.45\% of the initial hypercube due to the range constraints only.
%volume to approximately 3.4529\% of the initial hypercube due to the range constraints only.

The targeted Bayesian design algorithm is implemented to generate a $n = 700$ point design. First, for each of the above four subgroups of eight decision parameters the normalised parameter sums are sampled from a truncated normal distribution in order to facilitate the exploration of more extreme values of the total sums of the eight normalised parameters than would be the case using a standard uniform or Latin hypercube design. This is perceived to be important based on reservoir engineering insight. Next, the differences are sampled according to the specified value of $\Delta_i$ before imposing the operational range constraints (after transforming the normalised parameters to their physical values). Each parameter subgroup and the overall design are approximately optimised with respect to the minimax design selection criterion by comparing candidate designs to a large $20,000$ point uniform random sample (over the constrained parameter space) \cite{2003:Santner:The-Design-and-Analysis-of-Computer-Experiments}. Moreover, the optimised design is augmented to include two further decision parameter vectors with all parameters set to either their minimum or maximum values since it is of interest to observe the model behaviour at these extremes. Full details of the targeted Bayesian design algorithm are presented in \cref{subsec:Extended-Results-Targeted-Bayesian-Design-Methodology}.

The final wave 1 design for eight producer well 2 parameters is illustrated in \cref{fig:OLYMPUS-w1-sampleSumDiff-pres-par-sum-truncnorm-minimax-design-prod2-Pairs-Plots}. The plots next to the diagonal highlights the difference constraints as points are clustered between two clearly defined diagonal parallel bounds. Since the final two control intervals are of length 4 years a greater change of up to $\frac{2}{3}$ of the parameter operational range is permitted, hence the wider bands. In addition, the difference constraints affect decision parameters at larger time separations where there are fewer points away from the diagonal, although is less pronounced for greater time gaps. This design is evaluated for the identified subset of 3 OLYMPUS models with the linear model used to predict the ensemble mean NPV for which points are coloured green, yellow and red for high, moderate and low NPVs respectively in \cref{fig:OLYMPUS-w1-sampleSumDiff-pres-par-sum-truncnorm-minimax-design-prod2-Pairs-Plots}.
\begin{figure}[!t]%[!h]
	\centering
	\includegraphics[width=\linewidth]{Results/Graphics/Wave-1-Targeted-Bayesian-Design/Design-Pairs-Plots-with-Predicted-CWG-NPV-prod-2}
	\caption{Wave 1 702 point design OLYMPUS producer well 2 decision parameters pairs plots. Points are coloured by the multi-model ensemble subsampling linear model predicted NPV where green, yellow and red correspond to high, moderate and low NPVs respectively.}
%	\caption[OLYMPUS wave 1 design pairs plot for producer well 2 coloured by NPV]{Wave 1 design pairs plots of the 702 well control strategies for producer well 2 for a design generated using \cref{alg:Sampling-of-Parameter-Sum-and-Differences-preserving-Parameter-Sum-Sampling-Distribution-adjust-Difference-Sampling-Range} and selected using the minimax distance criterion. A fixed initial sample of parameter sums from a truncated normal distribution was used when forming all candidate designs. Points are coloured according to the simulated NPV obtained from the EGES linear model with green, yellow and red corresponding to high, moderate and low NPVs respectively.}
	\label{fig:OLYMPUS-w1-sampleSumDiff-pres-par-sum-truncnorm-minimax-design-prod2-Pairs-Plots}
\end{figure}
Note that the presented emulation methodology also works with more traditional space filling designs. Employment of a targeted Bayesian design is to enhance the overall decision support aim, and to incorporate expert knowledge regarding the reservoir behaviour and practical decision implementation.



%%% Notes %%%
%See PhD Thesis Section 4.3.
%
%Provide a brief overview of the methodology, how this incorporates the physical constraints proposed by experienced oil reservoir engineers, and results.
%
%Discuss both the constraints and the design mechanism.
%
%%% Other Useful Notes Regarding the Wave 1 Design %%%
%A priori a 700 point design is justified by the heuristic of sampling at least 10 times the dimension of the parameter space, $n \geq 10\cdot D$ \cite{2009:Loeppky:Choosing-the-Sample-Size-of-a-Computer-Experiment-A-Practical-Guide}
%
%Compared to uniform sampling there are more points sampled for smaller and larger parameter values, thus there is better exploration of the corner and edge regions of the decision space, but still sufficiently many points near the centre for constructing Bayesian emulators. This design is evaluated for only the subset of 3 OLYMPUS models identified in \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Application-of-EGES-Techniques}, with the EGES linear model used to predicted the ensemble mean NPV.
%
%Observations confirm reservoir engineering insight with high early time target production rates required to achieve a high NPV. As time progresses, the effect of discounting results in an increasing spread of red and yellow points across each parameters range until the final control interval, prod\_2\_2032\_01, which encompasses the full range and hence a high NPV may be achieved for any control value when combined with suitable other decisions.
%A similar pairs plot is generated and checked for producer well 10 which is omitted for space, although the apparent association between high early time target rates is less substantive. This is indicative of the behaviour for producer well 2 being more important than producer well 10 in determining the overall NPV.
%Pairs plot for the two injector wells also possess the structure induced by the difference constraints, but with no dominant behavioural insight into which values are likely to yield a high expected NPV.

==> Results/Emulator-Comparison.tex <==
\subsection{Emulator Comparison} \label{subsec:Emulator-Comparison}

Two approaches here implemented for emulating the ensemble mean NPV: a Bayes linear emulator; and a hierarchical emulator which exploits known constrained behaviour for certain simulator outputs. Firstly, comparing each emulator's adjusted variances evaluated for the same large collection of decision parameter vectors in \cref{fig:OLYMPUS-w1-comparison-BL-and-hier-emulator-ensemble-mean-NPV-hist-adj-var} demonstrates how the hierarchical emulator achieves a discernible reduction in the uncertainty versus with the Bayes linear emulator. This feature is also evident when comparing the \loo{} diagnostics plots in \cref{fig:OLYMPUS-w1-BL-emulator-theta-0_5-LOO-diagnostics-plot-adj-exp-3-adj-sd-CI-vs-sim-NPV,subfig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics-adj-CI-vs-sim} where there is a prevalent reduction in the credible interval widths. A direct comparison of the adjusted variances for each decision parameter vector highlights an average reduction in the adjusted variance of more than a half. Note that there exist a small number of cases where there is a moderate increase in the uncertainty, although this is outweighed by the gains achieved across the majority of sampled locations within the decision parameter space.
%For context, the seemingly large variances are inline with the scale of the ensemble mean NPV which is typically of order of $\num{5.0e+07}$ \$ to $\num{6.0e+07}$ \$.
\begin{figure}
	\centering
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Results/Graphics/Bayes-Linear-Emulation-of-the-Expected-NPV/Hist-adjust-var-OLYMPUS-w1-dec-par-BL-emul-ensemble-mean-CWG-NPV-theta-0_5-no-title}
		\caption{Bayes linear emulator.}
		\label{subfig:OLYMPUS-w1-BL-emulator-ensemble-mean-NPV-theta-0_5-hist-adj-var}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Hist-adj-var-OLYMPUS-w1-hier-emul-ensemble-mean-CWG-NPV-V6-k3-extrap-co-cp_lwr-no-title}
		\caption{Hierarchical emulator.}
		\label{subfig:OLYMPUS-w1-hier-emulator-ensemble-mean-NPV-hist-adj-var}
	\end{subfigure}
	\caption{Histograms comparing the Bayes linear and hierarchical emulators adjusted variances for the ensemble mean NPV. Note that the seemingly large variances are inline with the simulated ensemble mean NPV which is of the order $\num{5.0e+07}$ \$ to $\num{6e+07}$ \$.}
%	\caption[Histograms of the wave 1 Bayes linear and hierarchical emulators adjusted variances for the OLYMPUS ensemble mean NPV]{Comparison of the wave 1 Bayes linear and hierarchical emulators for the OLYMPUS ensemble mean NPV via histograms of their adjusted variances. For context, the seemingly large variances are inline with the scale of the ensemble mean NPV which is typically of order of $\num{5.0e+07}$ \$ to $\num{6e+07}$ \$.}
	\label{fig:OLYMPUS-w1-comparison-BL-and-hier-emulator-ensemble-mean-NPV-hist-adj-var}
\end{figure}

A crucial motivation for employing emulators as a surrogate to computer models is their speed of evaluation in order to enable further analyses such as decision support. Bayes linear emulation is known to be a very fast and efficient means of constructing emulators. In this application we achieve a substantial reduction in computation time with over 2000 emulator evaluations for new decision parameter settings per second using a single core of a standard desktop computer or laptop. This is juxtaposed with approximately 30 minutes per OLYMPUS model simulation, or 25 hours when using the entire ensemble. The combination of ensemble subsampling and Bayes linear emulation equates to an efficiency gain of the order of $10^8$.

The full hierarchical emulation process applied to the ensemble mean NPV requires for each OLYMPUS model the fitting of 48 separate emulators: 32 of the structured type; and 16 Bayes linear emulators, a total of 144 emulators over the three sub-selected OLYMPUS models. Next, these are combined to obtain emulators for the approximate and exact NPVs for each OLYMPUS model, before emulating the ensemble mean NPV, and then linking to the expected NPV. The computational performance is more modest achieving emulator evaluations at approximately 4 new decision parameter vectors per second using a single core, and is thus slower than Bayes linear emulation. However, in comparison with direct simulation from the OLYMPUS ensemble there is a considerable efficiency improvement of the order of $10^4$. This is sufficient for comprehensively exploring the decision parameter space. Moreover, the additional computational expense of hierarchical emulation can be justified by the reduction in emulator uncertainty. This is highly beneficial to performing an iterative decision support analysis where reducing emulator uncertainty is imperative for efficiently eliminating non-implausible regions of the decision parameter space, thus avoiding extra waves of extremely expensive simulations at locations that would have been ruled out by more accurate emulators. The additional computational cost is therefore offset versus the need for extra simulations. Such arguments are also relevant to analyses using single-stage (or one-shot) designs where fewer expensive computer model evaluations are required to achieve similar emulator accuracy across the parameter space. Both forms of emulators are easily parallelisable, thus permitting further efficiency gains.



%%% Notes %%%
%See PhD Thesis Section 4.5.5.
%
%\textbf{Bayes linear emulation speed:} \\
%In comparison with the direct use of the simulator we observe a substantial reduction in computation time with over 2000 emulations for new decision parameter settings per second using a single core compared to approximately 30 minutes per OLYMPUS model, or 25 hours using the entire ensemble. The combination of EGES and Bayes linear emulation equates to an efficiency gain of the order of $10^8$, thus highlighting one of the key benefits of emulation. Moreover the process is easily parallelisable to achieve even greater increases in speed.
%
%\textbf{Hierarchical Emulation:} \\
%Within this application, for each OLYMPUS model, this requires the fitting of 48 separate emulators: 32 of the structured type; and 16 Bayes linear emulators. This leads to a total of 144 emulators over the three sub-selected OLYMPUS models. The next stage of this analysis is to combine these constituent structured and Bayes linear emulators to first emulate the NPV for a particular model, before subsequently emulating the ensemble mean NPV and linking this to the expected NPV.
%
%Compare to hierarchical emulation speed and efficiency. The main conclusions are that hierarchical emulation is far more accurate, whilst the speed increase versus running the OLYMPUS model remains substantial, even if not as great at using Bayes linear emulators. The increase in accuracy has the potential to reduce the number of waves required in a decision support analysis, thereby reducing the number of computationally expensive simulations, and thus justifying the slightly slower speed of fitting and evaluation.
%
%Consider quantifying how many decision parameter vectors were used in the analysis.
%Total number of new decision parameter vectors used = 10^4
%Proportion of new decision parameter vectors for which there was a decrease in the adjusted variance for the hierarchical emulator versus the direct Bayes linear emulator for the ensemble mean CWG NPV = 0.75 = 75\%.
%Maximum proportional increase in the emulator adjusted variance at a new decision parameter vector for the hierarchical emulator versus the direct Bayes linear emulator for the ensemble mean CWG NPV = 3.1593488.
%Maximum proportional increase in the emulator adjusted standard deviation at a new decision parameter vector for the hierarchical emulator versus the direct Bayes linear emulator for the ensemble mean CWG NPV = 1.7774557.

==> Results/Hierarchical-Emulation-of-the-Expected-NPV.tex <==
\subsection{Hierarchical Emulation of the Expected NPV} \label{subsec:Hierarchical-Emulation-of-the-Expected-NPV}
%\subsection{Hierarchical Emulation of the Ensemble Mean NPV} \label{subsec:Hierarchical-Emulation-of-the-Expected-NPV}

We present an application of our hierarchical emulation framework to the \TNOChallengeWC{} for the decision support setup outlined in \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge}. As for Bayes linear emulation, this analysis utilises the ensemble subsampling linear model to predict the expected NPV using only 3 geological realisations, as described in \cref{subsec:Subsampling-from-Geological-Multi-Model-Ensemble}, along with the design constructed in \cref{subsec:Bayesian-Design.tex}.



\subsubsection{Structured Emulation of the NPV Constituents} \label{subsec:Results-Structured-Emulation-of-the-NPV-Constituents} % \label{subsec:TNO-OLYMPUS-Well-Control-Optimisation-Structured-Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents}

For each OLYMPUS model the NPV is determined by the oil production, water injection and production. We therefore decompose the NPV calculation into WOPT, WWIT, and WWPT, by both model and control interval. As discussed, the WOPT and WWIT within a control interval are observed to follow structured behaviour where the quantity is equal to the corresponding target rate decision parameter multiplied by the length of the time interval up to an unknown change point beyond which there is a plateau in the behaviour due to the BHP constraint. This is illustrated for the OLYMPUS 25 WOPT for producer well 2 over the first two year control interval (01/01/2016 to 01/01/2018) in \cref{fig:OLYMPUS-25-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-behaviour} which we use as a running example. We therefore employ the structured emulation technique of \cref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents} separately for each of the WOPT and WWIT within control interval constituents for wells in the CWG. % Note that such structured behaviour is not observed for WWPT within a control interval since there is no corresponding target rate; its behaviour is a consequence of attempting to achieve a given target production rate subject to the BHP constraint with water present within the oil field, hence we utilise Bayes linear emulators.
Conservative change points upper bounds and extrapolation cut-offs are estimated using \cref{eq:Change-point-upper-bound,eq:Change-point-lower-bound} respectively over the wave 1 simulations, with tolerances $\delta_{i,u} = \delta_{i, l} = 10$ chosen to ensure numerical stability. \Cref{fig:OLYMPUS-w1-WOPT-WWIT-cp-and-extrap-co-intervals} (in \cref{subsec:Extended-Results-Hierarchical-Emulation-of-the-Expected-NPV}) depicts the regions in which the ``true'' change points are believed to be situated for all WOPT and WWIT for each of the three wave 1 OLYMPUS models.

For each NPV constituent the next stage is to fit a preliminary Bayes linear emulator where the deterministic functions of the active decision parameters are:%$m_i(\boldd_{A_i})$
\begin{align} \label{eq:NPV-constituent-preliminary-Bayes-linear-emulator-active-variable-selection-linear-model}
	m_i(\boldd_{A_i}) = \boldg_i(\boldd_{A_i})^\Transpose \boldbeta_i = \beta_{i, 0} + \sum_{d_j \in A_i} \{ \beta_{i, j, 1} d_j + \beta_{i, j, 2} d_j^2 \}
\end{align}
It is assumed that the active decision parameters comprise all decisions which take place in the past of the output. For our running example this is $A_i = \{${prod\_2\_2016\_01}, {prod\_10\_2016\_01}, {inj\_2\_2016\_01}, {inj\_3\_2016\_01}$\}$. This is a logical choice since future decisions are physically unable to impact on an output up to the current time, however any past decisions may potentially have an effect. The remainder of each emulator's prior specification is analogous to in \cref{subsec:Bayes-Linear-Emulation-of-the-Expected-NPV}, but with the distinction that only those simulation points in $\mathcal{D}_i^\prime = \{ \boldd \mid \boldd \in \mathcal{D},\ \dcp > \cpu{jk}{t_i} \}$ with output $\boldFi^\prime = \{ \fid \mid \boldd \in \mathcal{D}_i^\prime \}$ are used in the fitting.

For our example of the OLYMPUS 25 WOPT for producer well 2 in the first control interval (ending 01/01/2018) the preliminary emulator predictive 3-sigma credible intervals are illustrated in \cref{subfig:OLYMPUS-25-w1-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-prelim-BL-emul-CI} versus the corresponding decision parameter, {prod\_2\_2016\_01}. This is compared to the theoretical maximum output depicted by the black dotted line determined by the effective target rate for the control interval. The vertical blue and red lines are situated at $\extrapcop{2}{2016}$ and $\cppu{2}{2016}$ respectively. The structured emulation methodology using an upper truncation yields the results shown in \cref{subfig:OLYMPUS-25-w1-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-struc-emul-CI}. Within the slope region, shown in purple, the preliminary emulator credible intervals exceed the constraint and are thus collapsed onto the slope yielding very narrow intervals representing strong beliefs that these decisions will be adhered to for the full control interval. Included are all decision parameter vectors with $d_{P2,2016} < \extrapcop{2}{2016}$, as well as cases where $d_{P2,2016} \geq \extrapcop{2}{2016}$ in which the preliminary emulator credible interval lower bound exceeds the slope. The uncertain intermediate region, shown in orange, is handled by a truncated GP reflecting the uncertainty in whether the model output is on the slope or relatively close when a target rate is achieved for the majority of a control interval. All of these points lie close to the black dotted slope line with much narrower credible intervals than the preliminary Bayes linear emulator. For the plateau region, shown in green, the preliminary emulator credible interval is well below this slope. It is therefore unnecessary to impose a truncation due to the very small probability that an emulator realisation actually exceeds this physical constraint, hence these intervals are unchanged between the two plots.
\begin{figure}
	\centering
	\begin{subfigure}{\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Plot-OLYMPUS-25-w1-WOPTPROD2_20180101-prelim-BL-emul-CI-versus-prod_2_2016_01}
		\vspace{-10pt}
		\caption{Preliminary Bayes linear emulator predictive CI versus prod\_2\_2016\_01.}
		\label{subfig:OLYMPUS-25-w1-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-prelim-BL-emul-CI}
	\end{subfigure}
	
	\vspace{-18pt}
	
	\begin{subfigure}{\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/Plot-OLYMPUS-25-w1-WOPTPROD2_20180101-structured-emul-CI-versus-prod_2_2016_01}
		\vspace{-10pt}
		\caption{Structured emulator with upper truncation predictive CI versus prod\_2\_2016\_01.}
		\label{subfig:OLYMPUS-25-w1-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-struc-emul-CI}
	\end{subfigure}
	\vspace{-5pt}
	\caption{OLYMPUS 25 wave 1 WOPT for producer well 2 during the first two years (ending 01/01/2018) versus the corresponding target production rate, prod\_2\_2016\_01. The top plot shows the wave 1 preliminary Bayes linear emulator predictive 3-sigma credible interval (CI) fitted using only the simulations with $d_{P2,2016} \geq \cppu{2}{2016}$. This is used within the structured emulation algorithm imposing the upper truncation due to the slope (black dotted line) with the CI shown in the bottom plot. The vertical blue and red lines are situated at $\extrapcop{2}{2016}$ and $\cppu{2}{2016}$ respectively. The purple, orange and green CI correspond to points in the slope, uncertain, and plateau regions respectively.}
%	\caption[OLYMPUS 25 WOPTPROD2\_20180101 wave 1 preliminary Bayes linear emulator and structured emulator predictive credible intervals versus prod\_2\_2016\_01]{OLYMPUS 25 wave 1 WOPT for producer well 2 during the first two years (ending 01/01/2018) versus the corresponding target production rate, prod\_2\_2016\_01. The top plot shows the wave 1 preliminary Bayes linear emulator predictive 3-sigma credible interval (CI) fitted using only the simulations with $d_{P2,2016} \geq \cppu{2}{2016}$. This is used within the structured emulation algorithm imposing the upper truncation due to the slope (black dotted line) with the CI shown in the bottom plot. The vertical blue and red lines are situated at $\extrapcop{2}{2016}$ and $\cppu{2}{2016}$ respectively. The purple, orange and green CI correspond to points in the slope, uncertain and plateau regions respectively.}
	\label{fig:OLYMPUS-25-w1-WOPTPROD2_20180101_diff-vs-prod_2_2016_01-prelim-BL-emul-and-struc-emul-CI}
\end{figure}

\Loo{} structured emulator diagnostics demonstrate satisfactory results with examples shown in \cref{fig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-and-WOPTPROD2_20280101-V6-k3-extrap-co-cp_lwr-LOO-diagnostics} for OLYMPUS 25 NPV constituents WOPT and WWIT in the control intervals ending 01/01/2018 and 01/01/2022 respectively. The first is our running example.
\begin{figure}[!t]
	\centering
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WOPTPROD2_20180101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
		\caption{$\text{WOPTPROD2\_2018\_01 emulator CI}$ versus simulated output.}
		\label{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=2,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WOPTPROD2_20180101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
		\caption{$\text{WOPTPROD2\_2018\_01 emulator CI}$ versus prod\_2\_2016\_01.}
		\label{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-prod_2_2016_01}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WWITINJ2_20220101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
		\caption{$\text{WWITINJ2\_2022\_01 emulator CI}$ versus simulated output.}
		\label{subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=2,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WWITINJ2_20220101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
		\caption{$\text{WWITINJ2\_2022\_01 emulator CI}$ versus inj\_2\_2020\_01.}
		\label{subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-inj_2_2020_01}
	\end{subfigure}
	\caption{Structured emulation \loo{} diagnostic plots for OLYMPUS 25 WOPTPROD2\_2018\_01 (top) and WWITINJ2\_2022\_01 (bottom). Left: Adjusted expectation with 95\% credible intervals (CI) of width 3 adjusted standard deviations versus the simulated value. The red dashed line denotes equality of the emulator and simulator. Right: Credible interval versus the output's corresponding target production and injection rate respectively. Red points denote the simulated output.}
	%	\caption[\Loo{} diagnostic plots for the structured emulation of OLYMPUS 25 WOPT for producer well 2]{\Loo{} diagnostic plots for the structured emulation of OLYMPUS 25 WOPTPROD2\_2018\_01 (top) and WOPTPROD2\_2028\_01 (bottom). The left column shows the adjusted expectation with credible intervals (CI) of width 3 adjusted standard deviations error bars versus the simulated value where the red dashed line denotes equality of the structured emulator and simulator. The right column shows the adjusted expectation with credible intervals of width 3 adjusted standard deviations error bars versus the output's corresponding decision parameter, the target production rate, with red points denoting the simulated values.}
	\label{fig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-and-WOPTPROD2_20280101-V6-k3-extrap-co-cp_lwr-LOO-diagnostics}
\end{figure}
\Cref{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim,subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim} show the emulator adjusted expectation with 95\% (3 adjusted standard deviations) credible intervals versus the simulated output. In each case the emulator is exceptionally accurate for smaller NPV constituent values corresponding to where the target rate is adhered to for the entire control interval. For larger simulated outputs believed to be on plateau, the credible interval is wider, whilst the use of a truncated GP emulator for intermediate values demonstrates a reduction in the uncertainty in these locations. The classification step emulator type is best observed in \cref{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-prod_2_2016_01,subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-inj_2_2020_01} of the credible intervals versus each NPV constituents' corresponding decision parameter. For all NPV constituents the majority of the credible intervals contain the simulated value and no issues are detected in other \loo{} diagnostic analyses. This demonstrates how incorporating known structures within the emulator enables very accurate emulators for the WOPT and WWIT NPV constituents based on a relatively small number of simulations whilst also capturing the change in behaviour.
%Another observation is that structured emulators for a fixed output type are generally more accurate where the truncated GP or Bayes linear emulator is applied for earlier time intervals. This is to be expected since there is less uncertainty of the preceding oil field behaviour, as well as fewer decision parameters which may affect the output. 
%\begin{figure}[!t]
%	\centering
%	\begin{subfigure}[t]{0.4955\linewidth}
%		\centering
%		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WOPTPROD2_20180101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
%		\caption{$\text{WOPTPROD2\_2018\_01 emulator CI}$ versus simulated output.}
%		\label{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[t]{0.4955\linewidth}
%		\centering
%		\includegraphics[page=2,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WOPTPROD2_20180101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
%		\caption{$\text{WOPTPROD2\_2018\_01 emulator CI}$ versus prod\_2\_2016\_01.}
%		\label{subfig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-prod_2_2016_01}
%	\end{subfigure}
%	
%	\begin{subfigure}[t]{0.4955\linewidth}
%		\centering
%		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WWITINJ2_20220101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
%		\caption{$\text{WWITINJ2\_2022\_01 emulator CI}$ versus simulated output.}
%		\label{subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-sim}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[t]{0.4955\linewidth}
%		\centering
%		\includegraphics[page=2,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-GP-emulator-WWITINJ2_20220101_diff-theta-0_5-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std-all-dec-par}
%		\caption{$\text{WWITINJ2\_2022\_01 emulator CI}$ versus inj\_2\_2020\_01.}
%		\label{subfig:OLYMPUS-25-w1-emul-WWITINJ2_20220101-v6-k3-extrap-co-cp_lwr-LOO-diagnostics-adj-CI-vs-inj_2_2020_01}
%	\end{subfigure}
%	\caption{Structured emulation \loo{} diagnostic plots for OLYMPUS 25 WOPTPROD2\_2018\_01 (top) and WWITINJ2\_2022\_01 (bottom). Left: Adjusted expectation with 95\% credible intervals (CI) of width 3 adjusted standard deviations versus the simulated value. The red dashed line denotes equality of the emulator and simulator. Right: Credible interval versus the output's corresponding target production and injection rate respectively. Red points denote the simulated output.}
%%	\caption[\Loo{} diagnostic plots for the structured emulation of OLYMPUS 25 WOPT for producer well 2]{\Loo{} diagnostic plots for the structured emulation of OLYMPUS 25 WOPTPROD2\_2018\_01 (top) and WOPTPROD2\_2028\_01 (bottom). The left column shows the adjusted expectation with credible intervals (CI) of width 3 adjusted standard deviations error bars versus the simulated value where the red dashed line denotes equality of the structured emulator and simulator. The right column shows the adjusted expectation with credible intervals of width 3 adjusted standard deviations error bars versus the output's corresponding decision parameter, the target production rate, with red points denoting the simulated values.}
%	\label{fig:OLYMPUS-25-w1-emul-WOPTPROD2_20180101-and-WOPTPROD2_20280101-V6-k3-extrap-co-cp_lwr-LOO-diagnostics}
%\end{figure}

Structured behaviour is not observed for WWPT within a control interval since there is no corresponding target rate; its behaviour is a consequence of attempting to achieve a given target production rate subject to BHP constraints with water present within the oil field. We separately employ Bayes linear emulators for the WWIT following the same approach as above, but fitted using all simulations in $\mathcal{D}$.

%%% More Detailed Paragaph on WWPT Emulation %%%
%As commented above, WWPT within a control interval does not follow the same structured behaviour as WOPT and WWIT, hence it is emulated separately using a Bayes linear emulator. This follows the same construction as for the preliminary Bayes linear emulator within the structured emulation approach implemented above with active decision parameters consisting of all those which occur in the past of the output. The prior specification is determined as above with deterministic functions of the same form as in \cref{eq:NPV-constituent-preliminary-Bayes-linear-emulator-active-variable-selection-linear-model}, but with all simulations in $\mathcal{D}$ used to fit the respective emulators since there is no obvious and easily exploitable structure.

%%% Paragraph on Number of Emulations %%%
%Within this application, for each OLYMPUS model, this requires the fitting of 48 separate emulators: 32 of the structured type; and 16 Bayes linear emulators. This leads to a total of 144 emulators over the three sub-selected OLYMPUS models. The next stage of this analysis is to combine these constituent structured and Bayes linear emulators to first emulate the NPV for a particular model, before subsequently emulating the ensemble mean NPV and linking this to the expected NPV.



\subsubsection{Emulation of the OLYMPUS Approximate NPV} \label{subsubsec:Results-Emulation-of-the-OLYMPUS-Approximate-NPV} % \label{subsec:TNO-OLYMPUS-Well-Control-Optimisation-Emulation-of-the-Approximate-NPV}

In this application the 8 decisions for each well are enacted over periods constructed by amalgamating consecutive 3-month discounting intervals. Emulation of the average discounting approximate NPV (\cref{eq:Average-discounting-approximate-NPV_j-formula-for-well-control-optimisation}) for each OLYMPUS model is performed as described in \cref{subsec:Emulation-of-the-Approximate-NPV} with \loo{} diagnostics plots for the OLYMPUS 25 approximate NPV shown in \cref{subfig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-via-NPV-summation-LOO-diagnostics-v6-k3-adj-CI-vs-sim}. There exists a strong linear relation between the emulator adjusted expectation and the simulated approximate NPV with the majority of points situated close to the red dashed equality line. It is observed that the uncertainty generally increases with the value of the approximate NPV. Petroleum reservoir engineering provides insight: higher target production and injection rates are generally necessary to achieve the largest NPVs. For the WOPT and WWIT structured emulators this occurs above the extrapolation cut-off and thus each constituent emulator exhibits a larger uncertainty. Furthermore, when many of the NPV constituents fall in their slope regions the structured emulator returns a small uncertainty determined by the tolerance. These linearly combine to produce a small uncertainty for the approximate NPV.
\begin{figure}[!t]
	\centering
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-emulator-avg-discount-approx-CWG-NPV-V6-k3-extrap-co-cp_lwr-LOO-diagnostics-plots-std}
		\caption{Approx NPV CI versus simulated values.}
		\label{subfig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-via-NPV-summation-LOO-diagnostics-v6-k3-adj-CI-vs-sim}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-25-w1-dec-par-emulator-CWG-NPV-via-lm-on-avg-discount-approx-CWG-NPV-sum-LOO-diagnostics-plots-std}
		\caption{Exact NPV CI versus simulated values.}
		\label{subfig:OLYMPUS-25-w1-emul-NPV-via-lm-on-avg-discount-approx-NPV-sum-LOO-diagnostics-v6-k3-adj-CI-vs-sim}
	\end{subfigure}
	\caption{Emulator \loo{} diagnostic plots for OLYMPUS 25 average discounting approximate NPV (left) and exact NPV (right, obtained via the linear model in \cref{eq:Exact-NPV_j-on-Approximate-NPV_j-LM-form} on the emulated approximate NPV) showing the adjusted expectation with 3 adjusted standard deviation Credible Intervals (CI) versus simulated values. The red dashed line denotes when the emulator and simulator coincide.}
%	\caption[\Loo{} diagnostic plots for the structured emulation of OLYMPUS 25 approximate and exact NPV]{\Loo{} diagnostics for emulators of the OLYMPUS 25 average discounting approximate NPV (left column) and the exact NPV (right column) via a simple linear model on the emulated approximate NPV. The top row shows the emulator adjusted expectation with 3 adjusted standard deviation credible intervals versus simulated values where the red dashed line denotes when the emulator and simulator coincide. The bottom row shows the emulator standardised residuals versus the simulated values.}
	\label{fig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-and-NPV-via-lm-on-avg-discount-approx-NPV-sum-LOO-diagnostics-v6-k3}
\end{figure}

%%% Paragraphs Describing LOO Diagnostics Residuals for the Average Discounting Approximate NPV by OLYMPUS Model %%%
% \Cref{subfig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-via-NPV-summation-LOO-diagnostics-v6-k3-std-resid-vs-sim} shows the emulator standardised residuals versus the simulated approximate NPV. There is evidence of a linearly decreasing pattern, particularly for smaller values of the simulated approximate NPV where there exist a number of larger, mainly positive residuals corresponding to underprediction. For moderate to high simulated approximate NPVs, the majority of the standardised residuals have an acceptable magnitude less than three.
%
%Comparing \cref{subfig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-via-NPV-summation-LOO-diagnostics-v6-k3-adj-CI-vs-sim,subfig:OLYMPUS-25-w1-emul-avg-discount-approx-NPV-via-NPV-summation-LOO-diagnostics-v6-k3-std-resid-vs-sim}, it is evident that these occur for smaller simulated approximate NPVs and hence with a view to decision support, it is expected that these will be discarded at wave 1 and so are possibly not a concern. There are also a few cases with large negative residuals due to overprediction. The iterative nature of decision support enables further investigation of these parameter vectors at later waves. In addition, the overall aim is to construct an accurate emulator for the final utility function, where the approximate NPV for each OLYMPUS model are intermediate quantities. Assessment of their \loo{} diagnostics therefore provides valuable insight into the potential sources of any failures in the \loo{} diagnostics for $\Ud$.

%%% Paragraph on Multivariate Emulation %%%
%Intuition and reservoir engineering insight suggest there exists temporal (and potentially spatial) correlation between the NPV constituents. However, a consequence of the individual emulator constructions and the differing subsets of simulation design points on which they are fitted results in it being challenging to meaningfully assess the correlation structure required for a separable multivariate emulator. Realisation of a multivariate framework via \cref{eq:Approximate-NPV_j-emulation-via-NPV-formula-adjusted-expectation,eq:Approximate-NPV_j-multivariate-emulation-via-NPV-formula-adjusted-variance} leads to various approximate NPV emulator variances depending on the chosen correlation structure and hence is non-robust whilst also demonstrating little or no improvement in uncertainty versus the implemented approach, therefore justifying the independence assumption.



\subsubsection{Linking the OLYMPUS Exact and Approximate NPV} \label{subsubsec:Results-Linking-the-OLYMPUS-Exact-and-Approximate-NPV} % \label{subsec:TNO-OLYMPUS-Well-Control-Optimisation-Linking-the-Exact-and-Approximate-NPV}

The next step within the hierarchical emulator construction is to link the exact and approximate NPV for each OLYMPUS model. This accounts for the discrepancy induced by coalescing the discounting intervals. This follows the simple linear regression framework in \cref{eq:Exact-NPV_j-on-Approximate-NPV_j-LM-form} where the coefficients are estimated using the wave 1 simulation data. \Loo{} emulator diagnostics for the OLYMPUS 25 NPV are shown in \cref{subfig:OLYMPUS-25-w1-emul-NPV-via-lm-on-avg-discount-approx-NPV-sum-LOO-diagnostics-v6-k3-adj-CI-vs-sim}. The results are very similar to those for the approximate NPV with our commentary and interpretation mirroring that in \cref{subsec:Emulation-of-the-Ensemble-Mean-NPV}.

%%% Paragraphs Describing LOO Diagnostics Residuals for the Exact NPV by OLYMPUS Model %%%
%\Cref{subfig:OLYMPUS-25-w1-emul-NPV-via-lm-on-avg-discount-approx-NPV-sum-LOO-diagnostics-v6-k3-std-resid-vs-sim} exhibits a linearly decreasing trend for smaller values of the simulated approximate NPV and occurs due to underprediction highlighted by a number of larger, mainly positive residuals. Within decision support this is potentially not a concern as it is expected that these will be discarded at wave 1. This highlights how the simple linear regression approach to linking the approximate and exact NPV introduces very little additional uncertainty compared to the initial combination of the NPV constituent emulators.



\subsubsection{Emulation of the OLYMPUS Ensemble Mean NPV} \label{subsubsec:Results-Emulation-of-the-OLYMPUS-Ensemble-Mean-NPV} % \label{subsec:TNO-OLYMPUS-Well-Control-Optimisation-Emulation-of-the-Ensemble-Mean-NPV}

The process of building structured emulators for each of the NPV constituents, their combination via the NPV formula to obtain the average discounting approximate NPV, and subsequent linking to the exact NPV is repeated for each of the three sub-selected OLYMPUS models. For the \TNOChallengeWC{} and our decision support setup the ensemble mean NPV is the quantity of interest as the objective and utility function respectively. This is emulated using the ensemble subsampling linear model devised in \cref{subsec:Subsampling-from-Geological-Multi-Model-Ensemble} to combine the emulators for the OLYMPUS 25, 33, \& 45 NPVs, following the approach in \cref{subsec:Emulation-of-the-Ensemble-Mean-NPV}.

It is not possible to perform \loo{} diagnostics for the true ensemble mean NPV because simulations have only been performed for the identified subset of OLYMPUS models. Note that the additional uncertainty pertaining to the ensemble subsampling linear model is accounted for within the hierarchical emulator construction. Instead we compare the hierarchical emulator with the predicted ensemble mean NPV in  \cref{fig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics} where \cref{subfig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics-adj-CI-vs-sim} demonstrates accurate predictions. Moreover, the increase in the uncertainty compared to individually emulating a single OLYMPUS model NPV, such as for OLYMPUS 25 NPV in \cref{subfig:OLYMPUS-25-w1-emul-NPV-via-lm-on-avg-discount-approx-NPV-sum-LOO-diagnostics-v6-k3-adj-CI-vs-sim}, is modest; thus the process of subsampling from the ensemble before reconstructing the ensemble mean NPV contributes relatively little additional uncertainty versus the structured emulation of the NPV constituents for each model.  \Cref{subfig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics-std-resid-vs-sim} shows no distinguishable pattern in the pseudo standardised residuals, whilst the majority are of magnitude less than three.
\begin{figure}[!t]
	\centering
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-w1-dec-par-hierarchical-emulator-ensemble-mean-CWG-NPV-LOO-diagnostics-plots-V6-k3-extrap-co-cp_lwr-std-variable-prior}
		\caption{Hierarchical emulator CI versus subsampling predicted ensemble mean NPV. The red dashed line denotes emulator and simulator equality.}
		\label{subfig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics-adj-CI-vs-sim}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\centering
		\includegraphics[page=3,width=\linewidth]{Results/Graphics/Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour/OLYMPUS-w1-dec-par-hierarchical-emulator-ensemble-mean-CWG-NPV-LOO-diagnostics-plots-V6-k3-extrap-co-cp_lwr-std-variable-prior}
		\caption{Hierarchical emulator standardised residuals versus the simulated ensemble mean NPV.}
		\label{subfig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics-std-resid-vs-sim}
	\end{subfigure}
	\caption{OLYMPUS wave 1 hierarchical emulation diagnostics plots for the predicted ensemble mean NPV via the ensemble subsampling linear model combining the emulation output for the exact NPV of the three sub-selected OLYMPUS models.}
%	\caption[OLYMPUS wave 1 hierarchical emulation diagnostic plots for the ensemble mean NPV]{OLYMPUS wave 1 hierarchical emulation diagnostic plots for the predicted ensemble mean NPV via the EGES linear regression model combining the emulation output for the exact NPV of the three sub-selected OLYMPUS models.}
	\label{fig:OLYMPUS-w1-hier-emul-Ensemble-Mean-NPV-via-EGES-LM-diagnostics}
\end{figure}



%%% Notes %%%
%See PhD Thesis Section 4.5.

==> Results/OLYMPUS-Exploratory-Analysis.tex <==
\subsection{OLYMPUS Exploratory Analysis} \label{subsec:OLYMPUS-Exploratory-Analysis}

We first construct a maximum Latin hypercube design and run a wave 0 of $n = 20$ exploratory simulations using all $N = 50$ OLYMPUS models. An important feature is the adherence of OLYMPUS simulations to target production and injection rate decision parameters. For one vector of decision parameter settings \cref{fig:OLYMPUS-Exploratory-Analysis-Decision-Output-Rates-vs-time-all-decisions-SIM-1} compares the input target control rates (black dashed lines) with the corresponding outputted achieved rates over the 50 ensemble members (coloured traces). It is immediately evident in all plots that the input targets are not strictly adhered to for the full duration of the control intervals; a consequence of the underlying physics programmed into the OLYMPUS model, including constraints on BHP, resulting in such deviations between the actual and targetted control values. It is this behaviour which motivates our structured emulation approach in \cref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents} which is demonstrated in \cref{subsec:Results-Structured-Emulation-of-the-NPV-Constituents}. Another interesting facet with potential ramifications for emulation and decision support is the vastly different relative absolute contributions of oil and water to the NPV objective function. An assessment is shown in \cref{fig:OLYMPUS-25-Exploratory-Analysis-NPV-Oil-Water-Contribution-all-decisions}, along with further discussion in \cref{subsec:Extended-Results-OLYMPUS-Exploratory-Analysis}.
\begin{figure}[!h]
	\centering
	\begin{subfigure}[t]{0.4955\linewidth}
		\includegraphics[page=1,width=\linewidth]{Results/Graphics/Exploratory-Analysis/Decision-Output-vs-Time/Decision-Output-vs-Time-SIM_1}
		\caption{WOPR.PROD.2.}
		\label{subfig:OLYMPUS-Exploratory-Analysis-WOPRPROD2-vs-time-all-decisions-SIM-1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\includegraphics[page=2,width=\linewidth]{Results/Graphics/Exploratory-Analysis/Decision-Output-vs-Time/Decision-Output-vs-Time-SIM_1}
		\caption{WOPR.PROD.10.}
		\label{subfig:OLYMPUS-Exploratory-Analysis-WOPRPROD10-vs-time-all-decisions-SIM-1}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.4955\linewidth}
		\includegraphics[page=3,width=\linewidth]{Results/Graphics/Exploratory-Analysis/Decision-Output-vs-Time/Decision-Output-vs-Time-SIM_1}
		\caption{WWIR.INJ.2.}
		\label{subfig:OLYMPUS-Exploratory-Analysis-WWIRINJ2-vs-time-all-decisions-SIM-1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.4955\linewidth}
		\includegraphics[page=4,width=\linewidth]{Results/Graphics/Exploratory-Analysis/Decision-Output-vs-Time/Decision-Output-vs-Time-SIM_1}
		\caption{WWIR.INJ.3.}
		\label{subfig:OLYMPUS-Exploratory-Analysis-WWIRINJ3-vs-time-all-decisions-SIM-1}
	\end{subfigure}
	\caption{Comparison of the target and achieved control rate decision parameters for an OLYMPUS wave 0 exploratory simulation over the full multi-model ensemble. Plots show the OLYMPUS output actual control rates time series as coloured lines for each ensemble member for the Well Oil Production Rates (WOPR, top) or Well Water Injection Rates (WWIR, bottom) for the four wells within the CWG. The black dashed lines that show the corresponding decision parameters of target production or injection rates respectively. The differences between the output traces and the inputs highlights the deviations between the target control and what is achieved due to physical constraints applied in the model.}
	%	\caption[Comparison of the target and achieved rate controls for the OLYMPUS exploratory simulations]{Comparison of the target and achieved rate controls for the OLYMPUS model using the first exploratory simulation. Each plot shows the simulator output as coloured lines for each ensemble member of the well oil production rates (top) or water injection rates (bottom) within the CWG versus time. This is compared with the black dashed lines that show the corresponding decision parameters of target production or injection rates respectively over time. The differences between the output traces and the inputs highlights the deviations between the target control and what is achieved due to physical constraints applied in the model.}
	\label{fig:OLYMPUS-Exploratory-Analysis-Decision-Output-Rates-vs-time-all-decisions-SIM-1}
\end{figure}



%%% Additional Section for Paragraph Describing Adherence of Controls to Specified Targets %%%
%For producer wells the BHP must not fall too low (minimum of 150 bar), hence it is easier to achieve a desired target production rate at earlier times, and whilst the injection rates are sufficiently high. This can be seen up to the start of 2021 in \cref{subfig:OLYMPUS-Exploratory-Analysis-WOPRPROD2-vs-time-all-decisions-SIM-1,subfig:OLYMPUS-Exploratory-Analysis-WOPRPROD10-vs-time-all-decisions-SIM-1}, noting that there exists some variation due to the differing geologies, especially when a high target production rate is requested. In later time intervals there is a persistent struggle to maintain BHP, particularly for producer well 10. For injector wells the BHP must not be too high (maximum of 235 bar) which would be exceeded as a result of high water injection whilst not extracting sufficient quantities of fluid from the field. Consequently at earlier time intervals it is harder to maintain a requested injection rate, whilst at later times this can be achieved. Examples of this behaviour can be seen in \cref{subfig:OLYMPUS-Exploratory-Analysis-WWIRINJ2-vs-time-all-decisions-SIM-1,subfig:OLYMPUS-Exploratory-Analysis-WWIRINJ3-vs-time-all-decisions-SIM-1}. Such observations of two distinct modes of behaviour motivates structured emulation of these outputs within time intervals in \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Hierarchical-Emulation-Exploiting-Known-Simulator-Behaviour}. Note that another characteristic which is observed in these plots is an occasional apparent lag between the new target rate and it being recorded in the simulator output. This is not actually the case and is a consequence of the numerical solver step-sizes which is addressed prior to the first wave of simulations for decision support.

==> Results/Results.tex <==
\section{Results} \label{sec:Results}

The statistical methodology presented in \cref{sec:Hierarchical-Emulators-Exploiting-Known-Simulator-Behaviour} is demonstrated for the motivating \TNOChallengeWC{} introduced in \cref{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge}, which is reformulated as a decision support problem with a focus on the ensemble mean NPV, $\meanNPVd \approx \ENPVd$. This builds on the work published in \cite{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty}. This includes: an exploratory design of simulations and analysis in \cref{subsec:OLYMPUS-Exploratory-Analysis}; subsampling from the OLYMPUS ensemble in \cref{subsec:Subsampling-from-Geological-Multi-Model-Ensemble}; an efficient method for constructing a targeted Bayesian design in \cref{subsec:Bayesian-Design.tex}; application of Bayes linear and the proposed hierarchical emulator to the ensemble mean NPV in \cref{subsec:Bayes-Linear-Emulation-of-the-Expected-NPV,subsec:Hierarchical-Emulation-of-the-Expected-NPV}; with a comparison performed in \cref{subsec:Emulator-Comparison}.


\input{Results/OLYMPUS-Exploratory-Analysis.tex}

\input{Results/Subsampling-from-Geological-Multi-Model-Ensemble.tex}

\input{Results/Design.tex}

\input{Results/Bayes-Linear-Emulation-of-the-Expected-NPV.tex}

\input{Results/Hierarchical-Emulation-of-the-Expected-NPV.tex}

\input{Results/Emulator-Comparison.tex}

==> Results/Subsampling-from-Geological-Multi-Model-Ensemble.tex <==
\subsection{Subsampling from Geological Multi-Model Ensemble} \label{subsec:Subsampling-from-Geological-Multi-Model-Ensemble}

%We first construct a maximum Latin hypercube design and run a wave 0 of $n = 20$ exploratory simulations using all $N = 50$ OLYMPUS models. 
A preliminary graphical investigation is performed using plots of the ensemble mean versus individual model for a range of outputs of interest for the exploratory simulations. Examples are provided in \cref{fig:OLYMPUS-EGES-ensemble-mean-vs-model-outputs} (see \cref{subsec:Extended-Results-Subsampling-from-Geological-Multi-Model-Ensembles}). It is unnecessary to sub-select models exhibiting close individual model output relations with the ensemble mean. Instead we screen for cases where the relationship is easy to model, for example, with a preference for linear associations with small output variation, identifying an initial set of 9 OLYMPUS models for further exploration via linear modelling. Further discussion is found in \cref{subsec:Extended-Results-Subsampling-from-Geological-Multi-Model-Ensembles}, and in \cite[Sec.~4.2]{2022:Owen:PhD-Thesis}.

In order to capture the interacting effects of the different OLYMPUS models, the subsampling technique utilising the linear model in \cref{eq:EGES-ensemble-mean-resp-linear-model-on-individual-model-resp-N_EGES-models-unknown} is implemented. First it is applied to the proposed OLYMPUS subset before extending to all models via both directions stepwise selection starting from the full model and using AIC as the model selection criterion. It is established that a subset of only $\Ntilde = 3$ models is sufficient for a large number of the investigated outputs, yielding high \AdjRsq{} values shown in \cref{fig:OLYMPUS-EGES-LM-all-resp-and-NPV-adj-R-Sq-3-models} in \cref{subsec:Extended-Results-Subsampling-from-Geological-Multi-Model-Ensembles}. The optimal collection for the ensemble mean NPV is OLYMPUS 25, 33, \& 45. The fitted linear model provides an efficient means of prediction and uncertainty quantification by using only 3 ensemble members yielding substantial computational savings. This is a novel application of such multi-model ensemble subsampling techniques in petroleum reservoir engineering.

%An important feature highlighted in the exploratory analysis is the adherence of OLYMPUS simulations to target production and injection rate decision parameters. For one vector of decision parameter settings \cref{fig:OLYMPUS-Exploratory-Analysis-Decision-Output-Rates-vs-time-all-decisions-SIM-1} compares the input target control rates (black dashed lines) with the corresponding outputted achieved rates over the 50 ensemble members (coloured traces). It is immediately evident in all plots that the input targets are not strictly adhered to for duration of control intervals; a consequence of the underlying physics programmed into the OLYMPUS model, including constraints on BHP, resulting in such deviations between the actual and targetted control values. It is this behaviour which motivates our structured emulation approach in \cref{subsec:Emulators-Exploiting-Known-Simulator-Behaviour-for-NPV-Constituents} which is demonstrated in \cref{subsec:Results-Structured-Emulation-of-the-NPV-Constituents}.




%%% Notes %%%
%See PhD Thesis Section 4.2.
%
%Note that we focus on the ensemble mean NPV, $\bar{f}(\boldd) = \meanNPVd$, as this is the primary focus in the \TNOChallengeshort{}, whilst this is linked to the expected NPV, $\Ud = \ENPVd$.%, in \cref{subsec:Ensemble-Uncertainty,subsec:Decision-Support-Implausibility-Measure}.


==> TNO-OLYMPUS-Well-Control-Optimisation-Challenge/TNO-OLYMPUS-Well-Control-Optimisation-Challenge-Bayes-Linear-Emulation.tex <==
\section{TNO OLYMPUS Well Control Optimisation Challenge} \label{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge-Bayes-Linear-Emulation}



==> TNO-OLYMPUS-Well-Control-Optimisation-Challenge/TNO-OLYMPUS-Well-Control-Optimisation-Challenge-V1.tex <==
\section{TNO OLYMPUS Well Control Optimisation Challenge} \label{sec:TNO-OLYMPUS-Well-Control-Optimisation-Challenge}

A major and commercially important challenge in the petroleum industry is field development under uncertainty for a green oil field\footnote{A green oil field is a new subsurface region believed to contain oil or gas which has yet to be exploited meaning that no drilling, production or injection has been performed.}. The Netherlands Organisation for Applied Scientific Research (TNO), as part of Integrated Systems Approach for Petroleum Production (ISAPP) research programme, devised the \TNOChallenge{} \cite{2018:ISAPP:Website} (abbreviated to \TNOChallengeshort{}) to encourage research and technological advancements to address the problem of optimisation under uncertainty. There is a particular emphasis on the uncertainty induced by the unknown underlying geology. The \TNOChallengeshort{} has received much attention across academia and industry with results of the competition phase presented at the EAGE/TNO Workshop on OLYMPUS Field Development Optimization \cite{2018:EAGE-TNO-Workshop-on-OLYMPUS-Field-Development-Optimization}.

The \TNOChallengeshort{} is based around the fictitious oil reservoir named OLYMPUS (inspired by a virgin oil field in the North Sea) and specifically designed by TNO for the challenge. OLYMPUS is a medium complexity model of size 9km by 3km, with a depth of 50m split into 16 layers for modelling purposes. The design was conceived to realistically imitate a real oil field possessing many of the features encountered in actual oil fields including: boundary and minor geological faults; two vertical zones separated by an impermeable shale layer (the top layer contains fluvial channel sands embedded in floodplain shale, whilst the bottom layer consists of alternating layers of coarse, medium and fine sands); as well as multiple types of facies (body of rock of specified characteristics) including channel sands, shale, and multiple types of sand. Geological uncertainty (unknown porosity, permeability, net-to-gross, and initial water saturation) is represented via a multi-model ensemble of $N = 50$ OLYMPUS realisations of a stochastic geology model. These are labelled as OLYMPUS 1 to 50. Full details of the model can be found in \cite{2017:TNO:OLYMPUS-oil-Reservoir-Model}.

The \TNOChallengeshort{} consists of three sub-challenges:
\begin{enumerate*}
	\item Well control optimisation,
	
	\item Field development optimisation,
	
	\item Joint optimisation of well placement and well control.
\end{enumerate*}
In this paper we focus on the first where the aim is to develop an optimal strategy with respect to maximising the expected Net Present Value (NPV) objective function over the 20 year field lifetime (starting January 1, 2016) with accumulation and discounting at 3 month intervals. The NPV for an individual OLYMPUS model is denoted $\NPVjd$ and is defined in \cref{eq:NPV-general-formula-in-decision-parameters} as a function of a vector of decision parameters, $\boldd$, consisting of target production and injection rates for producer and injector wells respectively. The index $i$ refers to the time interval $\Delta t_i = t_i - t_{i - 1}$, total number of time intervals $N_t$, fixed discount factor $d = 0.08$, time interval for discounting $\tau = 365$ days, and $R_j(\boldd, t_i)$ as the difference of all revenue and expenditure during the interval $\Delta t_i$, and $j = 1, \ldots, N = 50$ indexes the particular OLYMPUS realisation of the stochastic geology model. The expected NPV is approximated by the ensemble mean NPV defined in \cref{eq:Expected-NPV-general-formula-in-decision-parameters}.
\begin{align}
	\NPVjd &{} = \sum_{i = 1}^{N_t} \dfrac{R_j(\boldd, t_i)}{(1 + d)^{\frac{t_i}{\tau}}} \label{eq:NPV-general-formula-in-decision-parameters} \\
	\ENPVd &{} \approx \meanNPVd = \dfrac{1}{N} \sum_{j = 1}^{N} \NPVjd \label{eq:Expected-NPV-general-formula-in-decision-parameters}% \text{\nomenclature{$\ENPV(\cdot)$}{Expected NPV, defined in \cref{eq:Expected-NPV-general-formula-in-decision-parameters}}} \text{\nomenclature{$\meanNPV(\cdot)$}{Ensemble mean NPV, defined in \cref{eq:Expected-NPV-general-formula-in-decision-parameters}}}
\end{align}
For the well control optimisation challenge a fixed well configuration is provided by TNO based on oil reservoir engineering principles with $R_j(\boldd, t_i)$ defined in \cref{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)}, where $Q_{j,op}(\boldd, t_i)$, $Q_{j,wp}(\boldd, t_i)$,
and $Q_{j,wi}(\boldd, t_i)$ are the field oil production, water production, and water injection total volumes in time interval $\Delta t_i$ under controls $\boldd$ respectively. TNO also stipulate fixed oil revenue $r_{op} = 45$ \$ per bbl, water production cost $r_{wp} = 6$ \$ per bbl, and water injection cost $r_{wi} = 2$ \$ per bbl.
\begin{align} \label{eq:Well-control-optimisation-challenge-NPV-R(d_t_i)}
	R_j(\boldd, t_i) &{} = Q_{j,op}(\boldd, t_i) \cdot r_{op} - Q_{j,wp}(\boldd, t_i) \cdot r_{wp} - Q_{j,wi}(\boldd, t_i) \cdot r_{wi}
\end{align}
For demonstrative purposes we focus on the control of a subset of the wells enclosed between two partial fault boundaries and in close proximity consisting of two producer wells: 2 \& 10, and two injector wells 2 \& 3, with eight control intervals starting on January 1, 2016, 2018, 2020, 2022, 2024, 2026, 2028 \& 2032; thus a total of $D = 32$ decision parameters. Note that each control interval consists of multiple 3 month discounting periods. Collectively these wells are referred to as the Controlled Wells Group (CWG) which provides a sub-problem of interacting wells on which to illustrate the presented methodology. All remaining wells within OLYMPUS use the fixed controls specified in the TNO reference strategy \cite{2018:ISAPP:Website}. The expected NPV objective function is computed from contributions of wells in the CWG only.

We believe that the \TNOChallengeshort{} setup does not faithfully represent the real world field development under uncertainty problem where ensembles of computer models are used to aid decision makers. Instead, there is an emphasis on developing efficient ensemble optimisation algorithms to identify a single optimal strategy. A full critique and discussion of these limitations is presented in \cite[Sec.~3.1]{2022:Owen:PhD-Thesis} and \cite{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty}. We therefore re-formulate well control optimisation as a decision support problem. The aim of this paper is to develop accurate emulators for the expected NPV objective function by exploiting known simulator behaviour in order to efficiently perform decision support.



%%% Notes %%%
%Present the \TNOChallengeWC{} as motivation for this methodological development.
%
%See PhD Thesis Section 3.1.
%
%A critique of the \TNOChallenge{} is presented in \cite{2020:Owen:A-Bayesian-statistical-approach-to-decision-support-for-TNO-OLYMPUS-well-control-optimisation-under-uncertainty}.
%Further details can be found in \cite[Sec.~3.1]{2022:Owen:PhD-Thesis}
%
%Also see PhD Thesis Section 4.1 and 4.1.1.
